The Power of Two-sided Recruitment in Two-sided Markets

We consider the problem of maximizing the gains from trade (GFT) in two-sided markets. The seminal impossibility result by Myerson and Satterthwaite shows that even for bilateral trade, there is no individually rational (IR), Bayesian incentive compatible (BIC) and budget balanced (BB) mechanism that can achieve the full GFT. Moreover, the optimal BIC, IR and BB mechanism that maximizes the GFT is known to be complex and heavily depends on the prior. In this paper, we pursue a Bulow-Klemperer-style question, i.e., does augmentation allow for prior-independent mechanisms to compete against the optimal mechanism? Our first main result shows that in the double auction setting with $m$ i.i.d. buyers and $n$ i.i.d. sellers, by augmenting $O(1)$ buyers and sellers to the market, the GFT of a simple, dominant strategy incentive compatible (DSIC), and prior-independent mechanism in the augmented market is at least the optimal in the original market, when the buyers' distribution first-order stochastically dominates the sellers' distribution. Next, we go beyond the i.i.d. setting and study the power of two-sided recruitment in more general markets. Our second main result is that for any $\epsilon > 0$ and any set of $O(1/\epsilon)$ buyers and sellers where the buyers' value exceeds the sellers' value with constant probability, if we add these additional agents into any market with arbitrary correlations, the Trade Reduction mechanism obtains a $(1-\epsilon)$-approximation of the GFT of the augmented market. Importantly, the newly recruited agents are agnostic to the original market.

==> app_non_fsd_proof.tex <==
\section{Proof of Theorem~\ref{thm:non_fsd}}
\label{app:non_fsd_proof}
In this section, we prove Theorem~\ref{thm:non_fsd}.
As stated in Section~\ref{sec:non_fsd}, we can no longer use an argument that fixes the quantiles a priori since we could get unlucky with the realization of the quantiles.
For this reason, we consider the following process to assign quantiles.
First, we draw $m$ quantiles $\qbo(1), \ldots, \qbo(m)$ uniformly at random from $[0, 1]$ ordered such that $\qbo(1) \geq \ldots \geq \qbo(m)$.
Similarly, we draw $c$ quantiles $\qbn(1), \ldots, \qbn(c)$ uniformly at random from $[0, 1]$ ordered such that $\qbn(1) \geq \ldots \geq \qbn(c)$.
We repeat this for the sellers except that we order the quantiles such that $\qso(1) \leq \ldots \qso(n)$ and $\qsn(1) \leq \ldots \leq \qsn(c)$.
Finally, we let $\qb(1) \geq \ldots \geq \qb(m+c)$ be all the buyer quantiles
and $\qs(1) \leq \ldots \leq \qs(n+c)$ be all the seller quantiles.
We also let $\Bq$ be a vector with all the quantiles.

We let $\Bold = \{\qbo(1), \ldots, \qbo(m)\}$, $\Bnew = \{\qbn(1), \ldots, \qbn(c)\}$, $\Sold = \{\qso(1), \ldots \qso(n)\}$ and $\Snew = \{\qsn(1), \ldots, \qsn(c)\}$.
We also let $Q = \Bold \cup \Bnew \cup \Sold \cup \Snew$ denote the set of all quantiles.
Let $p = r n / 100 m$.
Next, for $k \geq 1$, we define the intervals
\begin{equation}
    I_k = \left( 1 - kp, 1-(k-1)p \right]
    \quad\text{and}\quad
    J_k = \left[ (k-1)p, kp \right)
\end{equation}
We also define $I_{\leq k} = \cup_{\ell=1}^k I_{\ell}$ and $J_{\leq k} = \cup_{\ell=1}^k J_{\ell}$.
Note that, as in Section~\ref{sec:str}, $I_k$ correspond to high quantile, high value buyers and $J_k$ correspond to low quantile, low value buyers.

% The proof of Theorem~\ref{thm:non_fsd} follows fairly straightforwardly from the following two lemmas.
% \begin{restatable}{lemma}{lemmacontbign}
%     \label{lemma:cont_big_n}
%     Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
%     Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
%     Then
%     \[
%         \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
%     \]
% \end{restatable}

The remainder of this section is structured as follows.
Subsection~\ref{subsec:defining_events} defines the various events we utilize to prove Theorem~\ref{thm:non_fsd}.
Two of the events are nearly identical to the events used in Section~\ref{sec:str} but we require one additional event that shows that each interval
contains roughly the ``right'' number of agents.
Subsection~\ref{subsec:cont_prob} analyzes the increase of GFT by using STR in the augmented market compared with OPT in the original market.
Finally, in Subsection~\ref{subsec:proof_non_fsd}, we summarize the arguments and prove Theorem~\ref{thm:non_fsd}.

\subsection{Constructing the Events}
\label{subsec:defining_events}
In this section, we define and analyze the events that we utilize to prove Theorem~\ref{thm:non_fsd}.

\paragraph{The event $\cE_3$.}
Define the event $\cE_3$ as the event that
\begin{equation}
\label{eqn:contE3def}
\begin{aligned}
    \cE_3 = \{
    & |I_{\leq 2} \cap \Bold| \leq 4pm,
    |(1-r/2, 1] \cap \Bold| \geq r n / 4, \\
    & |J_{\leq 2} \cap \Sold| \leq 4pm,
    |[0, r/2) \cap \Sold| \geq r n / 4
    \}
\end{aligned}
\end{equation}
At a high-level, we should think of $\cE_3$ as the event that each interval contains roughly the right number of original buyers and original sellers.
We require the following fact which will be used repeatedly.
\begin{claim}
    \label{claim:non_fsd_orig_matched}
    Condition on event $\cE_3$.
    In the original first-best matching, every original buyer in $I_{\leq 2}$ is matched
    and every original seller in $J_{\leq 2}$ is matched.
    Furthermore, in the augmented first-best matching, every buyer in $I_{\leq 2}$ is matched and every seller in $J_{\leq 2}$ is matched.
\end{claim}
\begin{proof}
    % \chris{Third line in below proof has a typo I think. Why do we even need that $|(1-r/2, 1] \cap \Bold| \geq r m / 4$ for the buyer case?}
    First, we prove that every original buyer in $I_{\leq 2}$ is matched.
    Let $k = |I_{\leq 2} \cap \Bold|$ be the number of original buyers in $I_{\leq 2}$.
    Note that $k \leq 4pm = 4 r n / 100 < r n / 4$, where the first inequality is by definition of $\cE_3$ (see Eq.~\eqref{eqn:contE3def}).
    % Using the definition of event $\cE_3$ again, since $|(1-r/2, 1] \cap \Bold| \geq r m / 4$ and $|[0, r/2) \cap \Sold| \geq r n / 4$, we must have $\qbo(k) \geq 1 - r/2$ and $\qso(k) \leq r / 2$.
    Using the definition of event $\cE_3$ again, since $|[0, r/2) \cap \Sold| \geq r n / 4$, we must have $\qbo(k) \geq 1 - r/2$ and $\qso(k) \leq r / 2$.
    By Lemma~\ref{lemma:r_fsd}, $b(\qbo(k)) \geq b(1-r/2) \geq s(r/2) \geq s(\qso(k))$ and thus every original buyer in $I_{\leq 2}$ is matched.

    The proof for the sellers is similar.
    Let $t = |J_{\leq 2} \cap \Sold|$ be the number of original sellers in $J_{\leq 2}$.
    When $\cE_3$ happens, we have $t \leq 4pm = 4 r n / 100 < r n / 4$.
    Following the identical logic above, we conclude that $s(\qso(t)) \leq s(r/2)\leq b(1-r/2) \leq b(\qbo(t))$ and thus every original seller in $J_{\leq 2}$ is matched.
    This proves the first assertion.

    The proof for the second assertion is nearly identical and is omitted.
\end{proof}


The following lemma shows that $\cE_3$ happens with high probability.
\begin{lemma}
    \label{lemma:cont_probE3_bound}
    $\prob{\cE_3} \geq 1 - 4\exp\left( -rn/300 \right)$.
\end{lemma}
\begin{proof}
    Since $|I_{\leq 2} \cap \Bold|$ can be written as a sum of i.i.d.~random variables and $\expect{|I_{\leq2} \cap \Bold|} = 2pm$,
    an application of the Chernoff Bound (see Lemma~\ref{lemma:chernoff}) gives
    \[
        \prob{|J_{\leq 2} \cap \Sold| \geq 4pm}
        \leq
        \prob{|I_{\leq 2} \cap \Bold| \geq 4pm} 
        \leq \exp\left( - pm / 3 \right)=\exp(-rn/300).
    \]
    Next, $\expect{|[0, r/2) \cap \Sold|} = rn/2$.
    So
    \[
        \prob{|(1-r/2, 1] \cap \Bold| \leq rn/4}
        \leq \prob{|[0, r/2) \cap \Sold| \leq rn/4}
        \leq \exp\left( - rn / 24 \right).
    \]
    % Similarly,
    % \[
    %     \prob{|[0, r/2) \cap \Sold| \leq rn/4} = \exp\left( -r^2 n / 2 \right).
    % \]
    By union bound we conclude that $\prob{\neg\cE_3} \leq 4 \exp\left( - rn / 300 \right)$.
    %The lemma follows by taking a complement.
\end{proof}
%\mingfei{One minor thing I changed: use $\neg \cE$ for the complement instead of $\overline{\cE}$ as the line connects with the brackets in the prob, e.g. $\prob{\overline{\cE}}$. }
%\chris{Sounds good. We can change it everywhere to be consistent.}

The following lemma bounds the loss on the GFT when the event $\cE_3$ is not satisfied. We denote $q_B\sim I_1$ the random variable $q_B$ drawn uniformly at random from the interval $I_1$. Similarly for $q_S\sim J_1$.
\begin{lemma}\label{lemma:expectation_E3}
    We have that
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq 4m \cdot \exp\left(- rn / 300 \right) \cdot
        \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    In particular, for any $\eta\in (0,1)$, if $n \geq \frac{300 \log(4m / \eta)}{r}$ then
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq \eta \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
    We write
    \begin{align*}
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}}
        & = \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}.
    \end{align*}
    Note that $\OPT(\Bq) - \STR(\Bq) \leq (\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qbo(j))\})_+$.
    {For the proof, we consider the following process to generate random uniform quantiles.
    First, for every agent, we assign them the label $1$ with probability $p$, the label $2$ with probability $p$, the label $3$ with probability $r/2 - 2p > 0$, and the label $4$ with the remaining probability. Note that the event $\neg \cE_3$ is defined via these labels. For example, the event that $|I_{\leq 2} \cap \Bold| \leq 4pm$ is the event that at most $4pm$ original buyers have the label $1$ or $2$.
    For the second step, we assign quantiles as follows.
    \begin{enumerate}[itemsep=0pt, topsep=0pt]
        \item Every buyer with label $1$ is assigned a uniform random quantile from $I_1$.
        \item Every buyer with label $2$ is assigned a uniform random quantile from $I_2$.
        \item Every buyer with label $3$ is assigned a uniform random quantile from $(1-r/2, 1] \setminus I_{\leq 2}$.
        \item Every buyer with label $4$ is assigned a uniform random quantile from $[0, 1-r/2]$.
    \end{enumerate}
    The sellers are assigned quantiles in an analogous manner. Note that each agent receives a uniformly random quantile.}
    
    {We claim that the random variable $\max_{i \in [m]}\{b(\qbo(i))\}$ is first-order stochastically dominated by the random variable $\max_{i \in [m]} \{b(\qb'(i))\}$ where $\qb'(1), \ldots, \qb'(m) \sim I_{1}$ uniformly at random. Indeed, fix any labelling as described above. If $k = 0$ then the stochastic-dominance is trivial. Otherwise, conditioned on $k\geq 1$ original buyers with the label $1$, we know that}
    \[
        \max_{i \in [m]} \{b(\qbo(i))\} \stackrel{d}{=} \max_{i \in [k]} \{b(\qb'(i)\} \stackrel{d}{\leq} \max_{i \in [m]}\{b(\qb'(i))\},
    \]
    {where we used $\stackrel{d}{=}$ to denote equal in distribution and $\stackrel{d}{\leq}$ to denote first-order stochastic dominance. As the stochastic dominance is true for every labelling, it follows that $\max_{i \in [m]} \{b(\qbo(i)\}$, conditioned on $\neg \cE_3$, is first-order stochastically dominated by $\max_{i \in [m]} \{b(\qb'(i))\}$.
    By an analogous argument, and since $m \geq n$, conditioned on $\neg \cE_3$, we can show that $-\min_{j \in [n]} \{s(\qso(j)\}$ is first-order stochastically dominated by $-\max_{j \in [m]} \{s(\qs'(j)\}$ where $\qs'(1), \ldots, \qs'(m) \sim J_{1}$ uniformly at random.}
    
    Thus, we have
    \begin{align*}
        \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3}
        & = \expectg{\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qso(j))\} }{\neg \cE_3} \\
        & \leq \expect{\max_{i \in [m]} \{b(\qb'(i))\} - \min_{j \in [m]} \{s(\qs'(j))\} } \\
        & \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}
    \end{align*}
    % We observe that, conditioned on $\cE_3$, $\OPT(\Bq) - \STR(\Bq)$ is first-order stochastically dominated by the random variable $\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}$ where $\qb'(i) \sim I_1$ (resp.~$\qs'(j) \sim J_1$) i.i.d.~and uniformly at random.
    % Let $\Bq'$ denote these auxiliary quantiles.
    % We thus have
    % \[
    %     \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3} \leq
    %     \expects{\Bq'}{\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}}
    %     \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    % \]
    Combining the inequality with Lemma~\ref{lemma:cont_probE3_bound} completes the proof.
\end{proof}

It remains to lower bound the GFT difference $\STR(\Bq)-\OPT(\Bq)$ when $\cE_3$ is satisfied. Similar to \Cref{sec:str}, we construct the following two events.

\paragraph{The good event $\cE_1$.}
Define $\cE_1$ as
\[
    \cE_1 = \{ \Bq : |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_1 \cap \Snew| \geq 2, |J_2 \cap \Sold| \geq 1 \}.
\]
We prove that $\cE_1\cap \cE_3$ is a sufficient condition for $\STR(\Bq)\geq \STR(\Bq)$. Moreover, we prove a lower bound on the expected GFT increase conditioned on $\cE_1\cap \cE_3$.
%on the event $\cE_1 \cap \cE_3$, we can obtain a strong lower bound on the GFT increase.
\begin{lemma}
    \label{lemma:cont_E1_lb}
    For any $\Bq \in \cE_1\cap \cE_3$, $\STR(\Bq) \geq \OPT(\Bq)$.
    Moreover,
    \[
        \expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_1\cap \cE_3} \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
Let $T$ be the number of trades in the original first-best matching.
We prove in the following claim that when $\cE_1\cap \cE_3$ happens, there are at least $T + 2$ trades in the augmented first-best matching.
% \chris{I think we need that $\Bq \in \cE_1 \cap \cE_3$. Because we use Claim~\ref{claim:non_fsd_orig_matched} which requires $\Bq \in \cE_3$. Also, just intuitively, we need to argue that $\qb'$ is matched and it is event $\cE_3$ that guarantees it is matched.}
% \chris{Also, why is the inequality $b(\qbn(2)) \geq b(\qb(T+2))$ (and similarly for seller) needed?}
\begin{claim}
    Recall that $\qbn(2)$ is the quantile of the second-highest new buyer and $\qsn(2)$ is the quantile of the second-lowest new seller. For any $\Bq\in \cE_1$, $b(\qbn(2)) \geq b(\qb(T+2)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
\end{claim}
\begin{proof}
    Let $\qb' \in I_2 \cap \Bold$ be the index of any original buyer in $I_2$ (by definition of $\cE_1$ there is at least one).
    By Claim~\ref{claim:non_fsd_orig_matched}, we have $\qb' \geq \qbo(T)$ (the buyer corresponding to quantile $\qb'$ is matched).
    On the event $\cE_1$, we have $|I_1 \cap \Bnew| \geq 2$ and thus $\qbn(2) \geq \qb' \geq \qbo(T)$.
    Therefore, $\qbn(2) \geq \qb(T+2) \geq \qbo(T)$ as both the highest and second-highest new buyer have quantile no less than $\qbo(T)$.
    A similar argument shows that $\qsn(2) \leq \qs(T+2) \leq \qso(T)$.
    We conclude that $b(\qbn(2)) \geq b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
    Here the first inequality follows from the fact that there are $T$ trades in the original first-best matching.
\end{proof}
Recall that that $\STR(\Bq) \geq \sum_{t=1}^{T+1} b(\qb(t)) - s(\qs(t))$
and $\OPT(\Bq) = \sum_{t=1}^T b(\qbo(t)) - s(\qso(t))$.
Since $\{\qb(1), \ldots, \qb(T+1)\} \setminus \{\qbn(1)\}$ consists of the top $T$ buyer quantiles except the highest \emph{new} buyer quantile and $\{\qbo(1), \ldots, \qbo(T)\}$ consist only of the top $T$ \emph{original} buyer quantiles, we have $\sum_{t=1}^{T+1} b(\qb(t)) - b(\qbn(1)) \geq \sum_{t=1}^T b(\qbo(t))$.
By a similar argument, we have $\sum_{t=1}^{T+1} s(\qs(t)) - s(\qsn(1)) \leq \sum_{t=1}^T s(\qso(t))$,
whence $\STR(\Bq) - \OPT(\Bq) \geq b(\qbn(1)) - s(\qsn(1))$.

Finally, we check that $\expectg{b(q(\inew_1))}{\cE_1\cap \cE_3} \geq \expects{\qb \sim I_1}{b(\qb)}$ (and analogously for the seller).
Note that if $\qb \sim I_1$ uniformly at random then $\qbn(1)$, conditioned on $|I_1 \cap \Bnew| \geq 2$, FSD $\qb$.
In addition, since the random variables $\qbn(1)$ and $|I_1 \cap \Bnew|$ are independent of the events $\cE_3$ and the random variables $|I_2 \cap \Bold|$, $|J_1 \cap \Snew|$ and $|J_2 \cap \Sold|$, we have
\[
    \expectg{b(\qbn(1))}{\cE_1\cap \cE_3} = \expectg{b(\qbn(1))}{|I_1 \cap \Bnew| \geq 2} \geq \expects{\qb \sim I_1}{b(\qb)}.
\]
A similar argument gives that $\expectg{s(\qsn(1))}{\cE_1\cap \cE_3} \leq \expects{\qs \sim J_1}{s(\qs)}$.
\end{proof}

% \chris{For the following, I think we need one more condition which is that there are at least $n+c$ buyers in the interval $[0, 2n/m]$.}
\paragraph{The bad event $\cE_2$.}
We define the bad event
\[
    \cE_2 = \neg\cE_1 \cap (\{ \Snew \cap (r/2, 1] = \Snew \} \cup \{ |\Bold \cap (1-r/2, 1]| < n + c\})
\]
In other words, the event requires that: (1) $\cE_1$ does not happen; (2) either every new seller has quantile in $(r/2, 1]$, or there are at least $n+c$ old buyers with quantile in $(1-r/2, 1]$. 
%all the new sellers are in the top $\gamma$ quantiles.
\begin{lemma}
    \label{lemma:contNotE2Better}
    % Meant to be a version of Lemma~\ref{lemma:notE2_STR_gt_OPT}.
    For any $\Bq \in \cE_3\cap \neg\cE_2$, we have $\STR(\Bq) \geq \OPT(\Bq)$.
\end{lemma}
\begin{proof}
    If $\Bq \in \cE_3$ but $\Bq \in \cE_1$ then we know from Lemma~\ref{lemma:cont_E1_lb} that $\STR(\Bq) \geq \OPT(\Bq)$.
    It remains to check that if $\Bq \in \cE_3 \cap \{\Snew \cap (1-\gamma, 1] \neq \Snew\} \cap \{|\Bold \cap (1-r/2, 1]| \geq n+c\}$ then $\STR(\Bq) \geq \OPT(\Bq)$.
    Let $\OPT'(\Bq)$ be the first-best matching in the augmented market.
    Suppose that $\OPT(\Bq)$ has $T \leq n$ trades.
    We consider two cases, depending on the number of trades in $\OPT'(\Bq)$.

    \paragraph{Case 1: $\OPT'(\Bq)$ has $T+1$ trades.}
    In this case, $\STR(\Bq)$ trades the top $T$ highest value (original and new) buyers and the bottom $T$ lowest value (original and new) sellers (but it could trade more). In particular, $\STR(\Bq) \geq \OPT(\Bq)$.

    \paragraph{Case 2: $\OPT'(\Bq)$ has $T$ trades.}
    Here, we want to show that $\STR(\Bq) = \OPT'(\Bq)$.
    By definition of STR, it suffices to show that $b(q(T)) \geq s(q(T+1))$.
    We claim that $\qso(T) > r/2$.
    For the sake of contradiction, suppose that $\qso(T) \leq r/2$.
    Since $\Bq \in \{\Snew \cap (r/2, 1] \neq \Snew\}$, this implies that $\qsn(1) \leq r/2$.
    But this means $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} \leq r/2$.
    However, since $|\Bold \cap (1-r/2, 1]| \geq n+c$ and $T \leq n$, it must be that $\qb(T+1) \geq \qbo(T+1) \geq 1-r/2$.
    But then by Lemma~\ref{lemma:r_fsd}, we would have $b(\qb(T+1)) \geq s(\qs(T+1))$ contradicting that $\OPT'(\Bq)$ has $T$ trades.
    We thus conclude that $\qso(T) > r/2$.
    
    To finish the proof, we have
    \[
        b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+1)). 
    \]
    The first inequality is because $\qb(T) \geq \qbo(T)$.
    The second inequality follows from the fact that $\OPT$ has $T$ trades.
    The last inequality holds because $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} = \qso(T)$ since $\qsn(1) \leq r/2 < \qso(T)$.
\end{proof}

\begin{lemma}
\label{lemma:cont_bound_loss_E2}
We have $\expectsg{\Bq}{\OPT(\Bq) - \STR(\Bq)}{\cE_2\cap \cE_3} \leq \expects{\qb \sim I_1, \qs \sim J_1}{b(\qb) - s(\qs)}$.
\end{lemma}
\begin{proof}
    Let $\OPT'(\Bq)$ be the GFT of the first-best matching in the augmented market.
    Let $b^*(\Bq)$ (resp.~$s^*(\Bq)$) denote the lowest (resp.~highest) value among buyers (resp.~sellers) traded in the augmented first-best matching.
    Let $\cF$ be the event that there is no trade in the first-best matching in the augmented market and let $b^*(\Bq) = 0$ and $s^*(\Bq) = 0$ if no trade exists in $\OPT'(\Bq)$.
    By definition of the STR mechanism, we have $\OPT(\Bq) - \STR(\Bq) \leq \OPT'(\Bq) - \STR(\Bq)\leq (b^*(\Bq)-s^*(\Bq)) \cdot \ind{\cF}$.

    We will show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \leq \expects{q_B \sim I_1}{b(\qb)}$. An analogous argument can be used to show that $\expectg{s^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \geq \expects{\Bs \sim J_1}{s(\qs)}$.
    We consider three cases.
    
    {Note that for the proof, we will make use of the following two-stage process to sample $\Bq$, which we describe only for the buyers (the sellers' description is analogous).
    First, we assign original and new buyers with two labels.
    For the first label, we assign them a label in $\{1, \ldots, \lceil 1/p \rceil\}$ where label $\ell \in [\lceil 1/ p \rceil]$
    is assigned with probability equal $\mu(I_\ell \cap [0, 1])$. Here $\mu$ denotes the Lebesgue measure.
    For the second label, if the first label is $\ell$ then we assign the second label $1$ with probability $\mu(I_{\ell} \cap (1-r/2, 1]) / \mu(I_{\ell})$ and $0$ otherwise.
    Note that except for one label $\ell'$ all labels $\ell \neq \ell'$ result in second labels having probability either $1$ or $0$.
    In particular, the label $(1,0)$ occurs with probability $0$ since $I_1 \cap (1-r/2, 1] = I_1$.
    For the second-stage, if a buyer is assigned the label $(\ell, 1)$ then we assign it a uniform random quantile from $(1-r/2, 1] \cap I_{\ell}$ and if it is assigned the label $(\ell, 0)$ then we assign it a uniform random quantile from $[0, 1-r/2) \cap I_{\ell}$.
    Note that with this process, every buyer is assigned a uniform random quantile from $[0, 1]$.}
    
    {Given this process, it is straightforward to maps the events $\cE_2, \cE_3$ to description about labels.
    For example, the event $|I_{\leq 2} \cap \Bold| \leq 4pm$ is equivalent to the event that at most $4pm$ original buyers are assigned a first label of $1$ or $2$ and the event $|(1-r/2, 1] \cap \Bold| \geq rn/4$ is equivalent to the event at least $rn/4$ original buyers are assigned a second label of $1$.}

    \paragraph{Case 1: $|I_1 \cap \Bnew| \geq 1$.}
    Let $\cE' = \{ |I_1 \cap \Bnew| \geq 1 \}$. {This is equivalent to the event that at least one new buyer is assigned a first label of $1$ in the above two-stage sampling process.}
    % To sample $\Bq$ such that $\Bq \in \cE' \cap \cE_2 \cap \cE_3$, we can first sample a quantile $\qb \sim I_1$ for a new buyer and then sample the remainder of $\Bq$.
    Conditioned on $\cE_3$, by Claim~\ref{claim:non_fsd_orig_matched}, we know that every new buyer in $I_1$ is traded (because every buyer in $I_1$ is traded).
    Let $\cG_k$ be the event that there are exactly $k$ new buyers in $I_1$.
    On the event $\cG_k \cap \cE_3 \cap \cE_2$ (provided that this event is non-empty), $b^*(\Bq)\ind{\cF} = b^*(\Bq) \leq \min_{i\in[k]} b(q'(i))$, where $q'(1), \ldots, q'(k)$ are $k$ uniform random quantiles from $I_1$.
    Note that $\min_{i \in [k]} b'(q(i))$ is first-order stochastically dominated by $b(\qb)$ where $\qb \sim I_1$ uniformly at random.
    Thus, $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    This is true for every $k$ such that $\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k \neq \emptyset$ so we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 2: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| \geq 1$.}
    This case is very similar to the above.
    Let $\cE'' = \{|I_1 \cap \Bnew| = 0, |I_1 \cap \Bold| \geq 1\}$.
    In this case, we define $\cG_k$ as the event that there are exactly $k$ \emph{original} buyers in $I_1$.
    Following an identical proof, we can show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    Thus, we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE''} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 3: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| = 0$.}
    This case is fairly trivial.
    Let $\cE''' = \{I_1 \cap \Bnew = I_1 \cap \Bold = \emptyset\}$.
    Then $b^*(\Bq)\ind{\cF} \leq b(1-p)\ind{\cF} \leq \expects{\qb \sim I_1}{b(\qb)} \ind{\cF}$ either because there is no trade or every traded buyer has a quantile outside $I_1$.
    
    Combining the three cases above concludes the proof.
\end{proof}

\subsection{Comparing STR and OPT in different regimes}
\label{subsec:cont_prob}
Let $\alpha \in (0, 1)$ be a constant decided later. We split the analysis into the regime where $n \geq \alpha m$ and $n \leq \alpha m$.
\paragraph{Case 1: $n \geq \alpha m$.}
\begin{lemma}
    \label{lemma:contProbE1}
    $\prob{\cE_1} \geq 1 - 6c(1-p)^c$.
\end{lemma}
\begin{proof}
    We have
    \[
        \prob{|I_1 \cap \Bnew| \leq 1}
        = (1-p)^c + c(1-p)^{c-1} p
        = (1-p)^c \left[ 1 + cp/(1-p) \right]
        < 2c (1-p)^c
    \]
    The inequality uses that $p=\frac{rn}{100m}\leq\frac{1}{100}$. Thus $p(1-p) \leq 1/4$ and $1 + c/4 \leq c + c/4 < 2c$ since $c \geq 1$.
    Identical calculations give
    \[
        \prob{|J_1 \cap \Snew| \leq 1} < 2c(1-p)^c
    \]
    Next, we have $\prob{|I_2 \cap \Bold| = 0} \geq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq (1-p)^c$ since $n\geq c$.
    Taking a union bound gives that $\prob{\neg\cE_1} \leq 6c(1-p)^c$.
\end{proof}
\begin{lemma}
    \label{lemma:cont_big_n}
    Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
    Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
    Then
    \[
        \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
    \]
\end{lemma}
% \lemmacontbign*
\begin{proof}[Proof of Lemma~\ref{lemma:cont_big_n}]
    Note that $\cE_1$ and $\cE_2$ are disjoint, we have
    \begin{align}
        \expect{\STR(\Bq) - \OPT(\Bq)}
        & = \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1\cap\cE_3} \label{eq:contE1E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2\cap\cE_3} \label{eq:contE2E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \cdot \prob{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \label{eq:contNotE1NotE2E3}\\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3} \label{eq:contE3}
    \end{align}
    For Eq.~\eqref{eq:contE1E3}, we use Lemma~\ref{lemma:cont_E1_lb}, Lemma~\ref{lemma:cont_probE3_bound}, and Lemma~\ref{lemma:contProbE1}, along with a union bound to get that
    \begin{multline*}
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1 \cap \cE_3} \\ \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot \left( 1 - 6c(1-p)^c - 4 \exp(-rn/300) \right).
    \end{multline*}
    For Eq.~\eqref{eq:contE2E3}, we use Lemma~\ref{lemma:cont_bound_loss_E2}, Lemma~\ref{lemma:contProbE1}, and the fact that $\prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \prob{\neg\cE_1}$ to get
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2 \cap \cE_3} \geq - \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot 6c(1-p)^c
    \]
    For Eq.~\eqref{eq:contNotE1NotE2E3}, Lemma~\ref{lemma:contNotE2Better} gives
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \geq 0.
    \]
    Finally, for Eq.~\eqref{eq:contE3}, by \Cref{lemma:expectation_E3} we have
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}
        \geq - 4m \cdot \exp(-rn/300) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    Putting everything together, it suffices to check that
    \[
        1 - 6c(1-p)^c - 4\exp(-rn / 300) \geq 6c(1-p)^c + 4m \exp(-rn/300).
    \]
    %A sufficient condition is that 
    The above inequality holds if $12c(1-p)^c \leq 1/2$ and $8m\exp(-rn/300) \leq 1/2$.
    To prove $12c(1-p)^c \leq 1/2$, note that $p = rn/(100 m) \geq r \alpha / 100$ and thus by our choice of $c$, we have
    $c \geq 4\log(24/p) / p$.
    Therefore,
    \[
        12c(1-p)^c \leq 12ce^{-cp} = \frac{12cp e^{-cp}}{p} \leq \frac{12e^{-cp/2}}{p} \leq \frac{12e^{-\log(24/p)}}{p} = \frac{1}{2}.
    \]
    Note that in the second inequality, we used that $cp \geq 4$ and the numeric inequality $xe^{-x} \leq e^{-x/2}$ valid for $x \geq 4$ (see Claim~\ref{claim:xexp_lt_exp}).
    For the inequality $8m \exp(-rn / 300) \leq 1/2$, note that this follows from the assumption that $n \geq \frac{300 \log(16 m)}{r}$.
\end{proof}

\paragraph{Case 2: $n \leq \alpha m$.}
\begin{lemma}
    \label{lemma:cont_small_n_E1}
    Let $\alpha > 0$ and suppose that $n \leq \alpha m$ and $c \geq 2$.
    Then
    \[
        \prob{\cE_1} \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6.
    \]
\end{lemma}
\begin{proof}
    Since $|I_1 \cap \Bnew|$ and $|J_1 \cap \Snew|$ are both distributed as $\Binom(p, c)$, we have that
    \[
        \prob{|J_1 \cap \Bnew| = 2} = \prob{|I_1 \cap \Bnew| = 2} = \binom{c}{2} (1-p)^{c-2} p^2 \geq \frac{c^2}{4} (1-r\alpha / 100)^{c-2} p^2
    \]
    where we used that $p = rn/100m \leq r\alpha / 100$ and $\binom{c}{2} = c(c-1) / 2 \geq c^2 / 4$ since $c \geq 2$.
    Next, since $|I_2 \cap \Bold|$ is distributed as $\Binom(p, m)$ and $|J_2 \cap \Sold|$ is distributed as $\Binom(p, n)$, we have
    \[
        \prob{|I_2 \cap \Bold| = 0} \leq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq 1-p.
    \]
    Therefore, $\prob{|I_2 \cap \Bold| \geq 1} \geq \prob{|J_2 \cap \Sold| \geq 1} \geq p$.
    Since the random variables $|I_1 \cap \Bnew|, |J_1 \cap \Snew|, |I_2 \cap \Bold|, |J_2 \cap \Sold|$ are all independent, the lemma follows by taking a product.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n_E2}
    Suppose that $n \leq mr / 8$.
    Then $\prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3)$.
\end{lemma}
\begin{proof}
    Recall that $\cE_2 \subset (\{\Snew \cap (r/2, 1] = \Snew\} \cup \{|\Bold \cap (1-r/2, 1]| < n+c\})$.
    Since $|\Snew \cap (r/2, 1]|$ is distributed as $\Binom(1-r/2, c)$ we have that
    \[
        \prob{\Snew \cap (r/2, 1] = \Snew} = (1-r/2)^c \leq \exp(-rc/2). 
    \]
    Next, since $\expect{|\Bold \cap (1-r/2, 1]|} = mr/2 \geq 4n$, the Chernoff bound gives (Lemma~\ref{lemma:chernoff})
    \[
        \prob{|\Bold \cap (1-r/2, 1]| < n+c}
        \leq \prob{|\Bold \cap (1-r/2, 1]| < 2n}
        \leq \exp(-n/3).
    \]
    Using a union bound proves the lemma.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n}
    Suppose that $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100m / rn)}{r}$, $n \geq 150c + \frac{300}{r} \log(9m)$, and $n \leq mr/8$.
    Then $\expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0$.
\end{lemma}
\begin{proof}
    The proof is nearly identical to Lemma~\ref{lemma:cont_big_n} except that we replace the bounds on $\prob{\cE_1 \cap \cE_3}$ and $\prob{\cE_2 \cap \cE_3}$
    with Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_small_n_E2}, respectively.
    For the former, using Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_probE3_bound}, where $\alpha = r/8$,
    \[
        \prob{\cE_1 \cap \cE_3}
        = 1 - \prob{\neg\cE_1 \cup \neg\cE_3}
        \geq 1 - \prob{\neg\cE_1} - \prob{\neg\cE_3}
        \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c - 4} p^6 - 4\exp(-rn / 300).
    \]
    and for the latter, using Lemma~\ref{lemma:cont_small_n_E1}, we have
    \[
        \prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3).
    \]
    Continuing as in Lemma~\ref{lemma:cont_big_n}, we now require that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 - 4\exp(-rn/ 300)
        \geq
        \exp(-rc/2) + \exp(-n/3) + 4m \exp(-rn / 300).
    \]
    Rearranging, a sufficient condition is that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 \geq \exp(-rc / 2) + 9m \exp(-rn / 300).
    \]
    Using that $n \geq 150c + \frac{300}{r} \log(9m)$, one can verify that $9m \exp(-rn / 300) \leq \exp(-rc/2)$.
    Also, since $c \geq 2$, we have $c^4/16 \geq 1$.
    Rearranging further, it suffices to show that
    \[
        p^6 \geq \frac{2\exp(-rc/2)}{\left(1 - r\alpha/100 \right)^{2c-4}}.
    \]
    This latter inequality is true since
    \begin{align*}
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c-4}}
        & \leq
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c}} \\
        & \leq 2\exp(-rc / 2 + 4rc\alpha / 100) \\
        & \leq 2\exp(-rc / 4) \\
        & \leq \left( \frac{rn}{100m} \right)^6 = p^6,
    \end{align*}
    where the second inequality used the numeric inequality $1/(1-x) \leq e^{2x}$ valid for $x \in [0, 1/4]$ (see Claim~\ref{claim:one_over_one_minus_x_lt_exp}),
    the third inequality used that $\alpha \leq 1$ and thus, $-rc/2 + 4rc\alpha / 100 \leq -rc / 4$,
    and the last inequality is because $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100 m / rn)}{r}$.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:non_fsd}}
\label{subsec:proof_non_fsd}
Finally, we prove Theorem~\ref{thm:non_fsd}.
\begin{proof}[Proof of Theorem~\ref{thm:non_fsd}]
    Let $\alpha = r/8$.
    We first ``pre-augment'' the market so that we can apply the results from the previous section.
    Let $m \geq n$ be the original number of buyers and sellers.
    First, we add $O(\log(1/r)/r)$ buyers to get $m' = m + O(\log(1/r)/r)$ buyers and so that $m' \geq 300 \log(16m') / r$.
    If $n \leq 300 \log(16m') / r$ we add $300 \log(16m') / r - n = O(\log(m/n) / r)$ buyers \emph{and} sellers get a total of $m''$ buyers $n''$ sellers.
    Note that $m'' \geq 300 \log(16m'') / r$ and $n'' \geq 300 \log(16m'') / r$.
    
    Next, choose
    \[
        c \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m''/rn'')}{r} \right\} = O(\log(m/rn) / r).
    \]
    Let $\Delta_N = 150c + \frac{300}{r} \log(16m'') - n'' \leq 150c$.
    If $\Delta_N > 0$ then it straightforward, albeit somewhat cumbersome, calculation to check that setting $m''' = m'' + 200\cdot C \cdot \Delta_N$, $n''' = n'' + 200\cdot C \cdot \Delta_N$ and $c''' = c + C\cdot \Delta_N$ for a large enough constant $C > 0$, we have
    \begin{itemize}
        \item $m''' \geq n''' \geq 150c + \frac{300}{r} \log(16m''')$;
        \item $c''' \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m'''/rn''')}{r} \right\} = O(\log(m / rn) / r)$.
    \end{itemize}
    
    Finally, applying Lemma~\ref{lemma:cont_big_n} if $n''' \geq \alpha m'''$ and Lemma~\ref{lemma:cont_small_n} if $n''' \leq \alpha m'''$,
    we conclude that $\STR(m''' + c''',n''' + c''') \geq \OPT(m''',n''')$.
    Note that both $m'''+c''' - m$ and $n''' + c''' - n$ are $O(\log(m / rn) / r)$.
\end{proof}



==> app_tr_lb.tex <==
\section{Lower Bound Example for Trade Reduction}
\begin{definition}[$(r, p)$-dominance]
Let $F$ and $G$ denote cumulative density functions.
We say that $F$ $(r,p)$-dominates $G$ if there exists $M$ such that the following holds.
Define $G'(v) = G(v) / G(M)$ for $v \in [0, M]$. Then
\begin{enumerate}
    \item $G(M) \geq p$; and
    \item $1 - F(v) \geq r\cdot (1 - G'(v))$ for all $v \in [0, M]$.
\end{enumerate}
\end{definition}

\textcolor{red}{TODO: We should clarify that trade reduction below means we reduce the last pair and not McAfee's trade reduction mechanism.}
\begin{theorem}
\label{thm:tr_infinite_lb}
Let $c \geq 1, r \in (0, 1)$ be parameters.
There exists a constant $M_{c,r}$, depending only on $c$ and $r$ such that for every $m \geq M_{c,r}$ the following statement holds.
There exists c.d.f.'s $F_B, F_S$ such that $F_B$ $(r,r)$-dominates $F_S$ but $\OPT(m, 1) > \TR(m+c, 1+c)$.
\end{theorem}

\begin{proof}
Fix $\eps \in (0, 1/\sqrt{3})$ and let $N = 1/\eps^2 > 3$.
We consider the following distribution.
\[
    \cD_B = \begin{cases}
        N & \text{with probability $\eps$} \\
        2 & \text{with probability $r-\eps$} \\
        0 & \text{with probability $1-r$}
    \end{cases}
    \quad \text{and} \quad
    \cD_S = \begin{cases}
        3 & \text{with probability $1-r$} \\
        1 & \text{with probability $r$}
    \end{cases}.
\]
Let $F_B, F_S$ denote the corresponding c.d.f.'s.
Observe that $F_B$ $(r,r)$-dominates $F_S$.
Indeed, take $F_S'(v) = F_S(v) / F_S(2.5)$ for $v \in [0, 2.5]$ which simply corresponds to a point mass at the value $1$ with probability $1$.
In this case, $F_S(2.5) = r$.
In addition, for $v < 1$ we have $r = 1 - F_B(v) \geq r \cdot 1 = r \cdot (1 - F_S'(v))$ and for $v \geq 1$, we have $1-F_S'(v) = 0$.

Our goal in the proof is to show that, for sufficiently small $\eps$, using the above distributions, we have $\OPT(m, 1) > \TR(m+c, 1+c)$.

First, we compute a lower bound on $\OPT(m, 1)$.
We use that if there is at least one buyer with value $N$ then the total GFT is at least $N - 3$.
Thus,
\begin{equation}
    \label{eqn:tr_infinite_opt_lb}
    \OPT(m, 1) \geq (N-3) \cdot \left( 1 - (1-\eps)^m \right) \geq N \cdot \left( 1 - (1-\eps)^m \right) - 3.
\end{equation}

Next, we run trade reduction with $m+c$ buyers with value distribution $\cD_B$ and $1+c$ sellers with value distribution $\cD_S$.
We define three events.
Let $\cE_1$ be the event that there is exactly one buyer with value $N$ that participates in a trade in trade reduction.
For event $\cE_1$ to happen it must be that either (i) there are at least two buyers with value $N$ or (ii) there is exactly one buyer with value $N$ and at least two sellers with value $1$.
Note that if there is exactly one buyer with value $N$ and at most one seller with value $1$ then there is only one trade in the optimal matching. In trade reduction, this trade is ``reduced'' and thus, trade reduction has no trades.
Let $\cE_1$ be the event that (i) there are at least two buyers with value $N$ or (ii) there is exactly one buyer with value $N$ and at least two sellers with value $1$.
In addition, note that, on the event $\cE_1$, the total GFT from trade reduction can be upper bounded by $N + (c+1)$; the first term is the GFT contributed from the first buyer and the second term ($c+1$) is a trivial upper bound on the GFT contributed by the remaining buyers.

Next, we define $\cE_2$ as the event that there are more than two buyers with value $N$ that participates in a trade in trade reduction.
Let $X$ be the number of buyers with value $N$. Then it must be that $X \geq 2$.
In this case, an upper bound on the GFT is $N\cdot X + (c+1)$.

The last event is $\cE_3 = \overline{\cE_1} \cup \overline{\cE_2}$. On event $\cE_3$, a trivial upper bound on the GFT is $c+1$.

Combining the above three events, we have that an upper bound on trade reduction is given by
\begin{equation}
    \label{eqn:tr_infinite_ub1}
    \TR(m+c, 1+c)
    \leq N \cdot \prob{\cE_1'} + N \expect{X \ind{X \geq 2}} + (c+1).
\end{equation}
First, we bound the first term in Eq.~\eqref{eqn:tr_infinite_ub1}.
Note that event $\cE_1'$ is composed of two disjoint events. Thus,
\begin{align*}
    \prob{\cE_1'}
    & = \left( 1 - (1-r)^{c+1} - (c+1)r(1-r)^c\right)\cdot (m+c)\eps(1-\eps)^{m+c-1} \\
    & + \left( 1 - (1-\eps)^{m+c} - (m+c)\eps(1-\eps)^{m+c-1} \right).
\end{align*}
The first summand is the probability that there is exactly one buyer with value $N$ and at least two sellers with value $1$ while the second summand is the probability that there are at least buyers with value $N$.
Rearranging, we have that
\begin{align*}
    \prob{\cE_1'}
    & = -\left[ (1-r)^{c+1} + (c+1)r(1-r)^c \right] \cdot (m+c) \eps (1-\eps)^{m+c-1}
      + (1 - (1-\eps)^{m+c}) \\
    & = - A_{c,r} \cdot (m+c) \eps (1-\eps)^{m+c-1}
      + (1 - (1-\eps)^{m+c}),
\end{align*}
where $A_{c,r} = (1-r)^{c+1} + (c+1)r(1-r)^c > 0$ is a constant depending only on $c, r$.

Next, we have
\begin{align*}
    \expect{X \ind{X \geq 2}}
    & \leq (m+c) \cdot \prob{X \geq 2} \\
    & \leq (m+c) \cdot \left(1 - (1-\eps)^{m+c} - (m+c)\eps(1-\eps)^{m+c-1} \right) \\
    & \leq (m+c) \cdot \left(1 - (1 - (m+c)\eps) - (m+c)\eps(1 - (m+c-1)\eps) \right) \\
    & \leq \eps^2(m+c)^3,
\end{align*}
where in the third inequality, we used the inequality $(1-x)^y \geq 1 - xy$, valid for $y \geq 1$ and $x \in [0, 1]$ (see Claim~\ref{claim:power_taylor}).
Thus, we have
\begin{equation}
    \label{eqn:tr_infinite_tr_ub}
    \TR(m+c, 1+c) \leq N\cdot \left[ (1 - (1-\eps)^{m+c}) + \eps^2(m+c)^3 - A_{c,r}(m+c) \eps(1-\eps)^{m+c-1} \right] + (c+1).
\end{equation}
Now we show that $\OPT(m, 1) - \TR(m+c, 1+c) > 0$.
Using Eq.~\eqref{eqn:tr_infinite_opt_lb} and Eq.~\eqref{eqn:tr_infinite_tr_ub}, we have
\begin{align*}
    \frac{1}{N} & \left(\OPT(m, 1) - \TR(m+c, 1+c) \right) \\
    & \geq -(1-\eps)^m + (1-\eps)^{m+c} - \eps^2(m+c)^3 + A_{c,r}(m+c)\eps(1-\eps)^{m+c-1} - \frac{c+4}{N} \\
    & = (1-\eps)^m \cdot \left[ -1 + (1-\eps)^c + A_{c,r}(m+c)\eps(1-\eps)^{c-1} \right] - \eps^2(m+c)^3 - \frac{c+4}{N} \\
    & \geq (1-\eps)^m \cdot \left[ -1 + (1 - c\eps) + A_{c,r}(m+c)\eps(1 - (c-1)\eps) \right] - \eps^2(m+c)^3 - \frac{c+4}{N} \\
    & = (1-\eps)^m \cdot \left[ -c\eps + A_{c,r}(m+c)\eps(1 - (c-1)\eps) \right] - \eps^2(m+c)^3 - \frac{c+4}{N} \\
    & = (1-\eps)^m \cdot \left[ (A_{c,r}(m+c)-c)\eps - A_{c,r}(m+c)(c-1)\eps^2 \right] - \eps^2(m+c)^3 - \frac{c+4}{N},
\end{align*}
where in the second inequality, we used the inequality $(1-x)^y \geq 1 - xy$, valid for $y \geq 1$ and $x \in [0, 1]$ (see Claim~\ref{claim:power_taylor}).
Recall that $N = 1/\eps^2$ and define the constant $M_{c,r}$ to satisfy $A_{c,r}(M_{c,r} + c) > 2c$.
If $m \geq M_{c,r}$ then we have that
\begin{align*}
    \frac{1}{N(1-\eps)^m \eps} & \left(\OPT(m, 1) - \TR(m+c, 1+c) \right) \\
    & \geq (A_{c,r}(m+c) - c) - A_{c,r}(m+c)(c-1) \eps - \eps(m+c)^3 - \eps(c+4) \\
    & \geq c - A_{c,r}(m+c)(c-1) \eps - \eps(m+c)^3 - \eps(c+4).
\end{align*}
As $\eps \to 0$, the RHS tends to $c > 0$.
We thus conclude that for sufficiently small $\eps > 0$ (depending on $c, r, m$), we have $\OPT(m, 1) > \TR(m+c, 1+c)$.
\end{proof}

\begin{remark}
    The proof of Theorem~\ref{thm:tr_infinite_lb} can be easily modified to show that the buyer trade mechanism also has an infinite lower bound.
    In fact, it holds for any mechanism of the following form. Let $u \in [0, 1)$ be a parameter.
    Let $b_1 \geq \ldots \geq b_m$ be the buyer values and $s_1 \leq \ldots \leq s_n$.
    Let $r = \max\{ i \,:\, b_i \geq s_i \}$.
    If $b_r \geq u b_{r+1} + (1-u) s_{r+1} \geq s_r$ then offer a price of $u b_{r+1} + (1-u) s_{r+1}$ to all the agents.
    Otherwise, offer a price of $b_{r}$ to the top $r-1$ value buyers and a price of $s_r$ to the bottom $r-1$ value sellers.
    When $u = 0$, we recover the seller trade reduction mechanism, when $u = 1$, we recover the buyer trade reduction mechanism, and when $u = 1/2$, we recover the trade reduction mechanism due to \citet{McAfee92}.
    The only observation that is needed to extend Theorem~\ref{thm:tr_infinite_lb} to this general setting is that for the event $\cE_1$ (where there is exactly one buyer participating in a trade with value $N$), we still require that at least two buyers with value $N$ or that there is exactly one buyer with value $N$ and at most one seller with value $1$.
    If there is exactly one buyer with value $N$ and one seller with value $1$ then a price of at most $2u + 3(1-u) = 3 - u < 3$ will be offered to the buyers and sellers; this is too low for the only remaining seller (with value $3$) to accept.
\end{remark}

\begin{claim}
    \label{claim:power_taylor}
    Let $x \in [0, 1]$ and $y \geq 1$.
    Then $(1-x)^y \geq 1 - xy$.
\end{claim}
\begin{proof}
    Fix $y \geq 1$ and let $f(x) = (1-x)^y - (1 - xy)$.
    Note that $f(0) = 0$.
    We next check that $f'(x)$ for $x \in (0, 1)$ which proves the claim.
    Indeed, $f'(x) = -y(1-x)^{y-1} + y = y\left[1 - (1-x)^{y-1} \right] \geq 0$ because $(1-x)^{y-1} \leq 1$.
\end{proof}

==> non_fsd.tex <==
%\section{$O(\log(m / rn) / r)$ upper bound for $r$ overlapping distributions}
\section{A Parameterized Upper Bound for General Distributions}
\label{sec:non_fsd}
In this section, we get rid of the stochastic dominance assumption used in \Cref{sec:str} and prove the following theorem.
\begin{theorem}
\label{thm:non_fsd}
Consider the double auction with $m$ i.i.d.~buyers and $n$ i.i.d.~sellers. Suppose $m\geq n$ and that $\probs{b \sim F_B, s \sim F_S}{b \geq s} = r$.
Then there exists $c = O((\log(m/n) + \log(1/r)) / r)$ such that
the GFT of STR with $m+c$ buyers and $n+c$ sellers 
is at least the first-best GFT with $m$ buyers and $n$ sellers.
\end{theorem}

When $m/n = O(1/r)$ (for example, if $m = n$) then \Cref{thm:non_fsd} implies an $O(\log(1/r) / r)$ upper bound. When $F_B$ FSD $F_S$, then the median of the buyer's value exceeds the median of the seller's value. This implies that $r=\prob{b \geq s} \geq 1/4$. However, in this case \Cref{thm:non_fsd} gives an upper bound of $O(\log(m/n))$ which does not fully match \Cref{thm:main_str}. {It remains an interesting open question whether the dependency on $m,n$ can be removed in \Cref{thm:non_fsd} so that the result generalizes the FSD case.}

% The techniques used to prove \Cref{thm:non_fsd} differs from the techniques for \Cref{thm:main_str} in the following way.
% In \Cref{thm:non_fsd} we prove that STR has GFT at least OPT for every fixed set of quantiles,
% with the expectation only taken over the random assignment from the quantiles to the agents.
% However this approach is unlikely to work in this general case since it is possible that we are unlucky with the realization of the quantiles.
% Instead we bound the expected GFT difference over the randomness of the quantiles as well.

To complement \Cref{thm:non_fsd}, we also prove a lower bound that a polynomial dependency on $1/r$ is required, using the result in \cite{BabaioffGG20}.
A proof can be found in Appendix~\ref{subsec:non_fsd_lb}.
\begin{theorem}[{Adapted from \cite[Proposition~3.4]{BabaioffGG20}}]
\label{thm:non_fsd_lb_intro}
For any sufficiently small $r\in (0,1)$, there exists a double auction instance with $\Pr_{b\sim F_B, s\sim F_S}[b\geq s]=r$ such that: For any $c\leq \frac{1}{4}\cdot r^{-1/8}$ and any deterministic, prior-independent, BIC, IR, BB and anonymous mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than the first-best GFT on $m$ buyers and $n$ sellers.
\end{theorem}

% Theorem~\ref{thm:non_fsd},
% %It is known that no finite bound applies to any pair of distributions even at the single seller case~\cite{BabaioffGG20}. Instead 
% a parameterized upper bound on the parameter $r = \probs{b \sim F_B, s \sim F_S}{b \geq s} \in (0,1)$. 
In \Cref{sec:str}, we crucially made use of stochastic dominance in many parts of the proof, i.e. the trade is available as long as the buyer quantile is at least the seller quantile.
%~$b(q) \geq s(q)$ for every $q$. 
While the stochastic dominance is no longer satisfied, the following lemma is useful to prove our result. It indicates that the trade is available if the buyer is at the top $r/2$ quantile and seller is at the bottom $r/2$ quantile.
%we refer to this as the $r$-overlap setting.
% Our main result in this section is the following theorem.
% \begin{theorem}
%     \label{thm:non_fsd}
%     Suppose $m\geq n$ and let $r=\probs{b \sim F_B, s \sim F_S}{b \geq s}$.
%     %For every $m \geq n$, there exists $c = O(\log(m / rn) / r)$ such that
%     There exists $c = O(\frac{\log(m/n)+\log(1/r)}{r})$ such that
%     \[
%         \STR(m+c, n+c) \geq \OPT(m, n). 
%     \]
% \end{theorem}

%\chris{Moved remark to intro.}
% \begin{remark}\label{remark:non_fsd}
% Here are some remarks from \Cref{thm:non_fsd}:

% 1. When $\frac{m}{n}=O(1/r)$ (we notice that $n=m$ belongs to this case), then \Cref{thm:non_fsd} implies an $O(\frac{1}{r}\cdot \log(\frac{1}{r}))$ upper bound.

% 2. We notice that the assumption of $F_B$ FSD $F_S$ implies that $r\geq\frac{1}{4}$ as $b(\frac{1}{2})\geq s(\frac{1}{2})$. However, the upper bound from \Cref{thm:non_fsd} in this case is $O(\log(m/n))$, which does not fully match the result in \Cref{thm:str_main}.
% \end{remark}

%the following observation suggests that we still have a property that has a similar flavor as stochastic dominance.
\begin{lemma}[{\cite[Lemma~3.1]{CaiGMZ21}}]
    \label{lemma:r_fsd}
    For any distribution $F_B$ and $F_S$, let $r=\probs{b \sim F_B, s \sim F_S}{b \geq s}$.
    Then $b(1-r/2) \geq s(r/2)$.
\end{lemma}
Unlike \Cref{sec:str}, an argument for any fixed quantiles does not apply here.
%a priori and then simply consider random assignments of these quantiles.
For example, we could unlucky and draw quantiles such that, in expectation over the random assignments, OPT has positive GFT while STR never trades (and thus, has GFT equal to $0$).
For this reason, we will bound the expected GFT difference over the randomness of the uniform quantiles as well.
%we cannot condition on the realization of the quantiles and must now also take expectation over the uniform quantiles.

In this section, we will only describe the high-level ideas for the proof of Theorem~\ref{thm:non_fsd}.
The proofs are relegated to Appendix~\ref{app:non_fsd_proof}.
%At a high-level, the proof of Theorem~\ref{thm:non_fsd} follows a similar structure to the proof of Theorem~\ref{thm:main_str} in Section~\ref{sec:str}.
We independently draw a uniform quantile from $[0,1]$ for each agent in the augmented market. We denote $\Bq=(q_1,\ldots, q_{m+n+2c})$ the set of quantiles. Here the first $m$ quantiles $q_1,\ldots,q_m$ are the quantiles for the old buyers. The next $n$ quantiles are for the old sellers and so on. Further, $\STR(\Bq)$ denotes the matching obtained by STR with input $\Bq$ and $\OPT(\Bq)$ denote the first-best matching in the original market.
For our proof, we construct \emph{three} events $\cE_1, \cE_2, \cE_3$ over the randomness of the \emph{quantiles} such that for some constant $C > 0$, depending only on $F_B, F_S$, the following statements hold.
\begin{enumerate}[topsep=0pt, itemsep=0pt]
    \item Conditioned on the event $\cE_3$, we have that $\cE_1$ is a sufficient condition for $\STR(\Bq) \geq \OPT(\Bq)$ and $\expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \geq C$.
    \item Conditioned on the event $\cE_3$, we have that $\cE_2$ is a necessary condition for $\OPT(\Bq) > \STR(\Bq)$ and $\expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3}\geq -C$.
    \item On the event $\neg \cE_3$, we have $\expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\neg \cE_3} \geq -m \cdot C$.
    \item $\prob{\cE_1 \cap \cE_3} \geq \prob{\cE_2 \cap \cE_3} + m \cdot \prob{\neg\cE_3}$.
\end{enumerate}
It is instructive to compare these four conditions with the conditions defined in Section~\ref{sec:str} and note that the only difference is the conditioning on a third event.
%As in Section~\ref{sec:str}, these four conditions allow us to prove Theorem~\ref{thm:non_fsd}.
The event $\cE_3$ is defined as the event that the number of high-quantile (i.e.~high-value) buyers is roughly equal to its expectation (and analogously for the low-quantile sellers). Intuitively, $\cE_3$ ensures that there are enough buyers at the top $r/2$ quantiles and enough sellers at the bottom $r/2$ quantiles, so that any high-quantile buyer and any low-quantile seller must trade in the first-best allocation (\Cref{claim:non_fsd_orig_matched}). We prove by concentration that $\cE_3$ does not happen with exponentially small probability, so that the expected loss outside $\cE_3$ is small.

%Having such an event is allows us to define the events 
Conditioned on $\cE_3$, we further construct the ``good event'' $\cE_1$ and the ``bad event'' $\cE_2$ similar to their counterpart in Section~\ref{sec:str}.
However, one notable difference is that we consider ``buckets'' defined via intervals on the real line instead of a fixed number of agents. See \Cref{app:non_fsd_proof} for more details.

\comment{
and instead consider the follow process to assign quantiles.
% we draw quantiles slightly differently than in Section~\ref{sec:str} (although they are still uniform at random).
First, we draw $m$ quantiles $\qbo(1), \ldots, \qbo(m)$ uniformly at random from $[0, 1]$ ordered such that $\qbo(1) \geq \ldots \geq \qbo(m)$.
Similarly, we draw $c$ quantiles $\qbn(1), \ldots, \qbn(c)$ uniformly at random from $[0, 1]$ ordered such that $\qbn(1) \geq \ldots \geq \qbn(c)$.
We repeat this for the sellers except that we order the quantiles such that $\qso(1) \leq \ldots \qso(n)$ and $\qsn(1) \leq \ldots \leq \qsn(c)$.
Finally, we let $\qb(1) \geq \ldots \geq \qb(m+c)$ be all the buyer quantiles
and $\qs(1) \leq \ldots \leq \qs(n+c)$ be all the seller quantiles.
We also let $\Bq$ be a vector with all the quantiles.

We let $\Bold = \{\qbo(1), \ldots, \qbo(m)\}$, $\Bnew = \{\qbn(1), \ldots, \qbn(c)\}$, $\Sold = \{\qso(1), \ldots \qso(n)\}$ and $\Snew = \{\qsn(1), \ldots, \qsn(c)\}$.
We also let $Q = \Bold \cup \Bnew \cup \Sold \cup \Snew$ denote the set of all quantiles.
Let $p = r n / 100 m$.
Next, for $k \geq 1$, we define the intervals
\begin{equation}
    I_k = \left( 1 - kp, 1-(k-1)p \right]
    \quad\text{and}\quad
    J_k = \left[ (k-1)p, kp \right)
\end{equation}
We also define $I_{\leq k} = \cup_{\ell=1}^k I_{\ell}$ and $J_{\leq k} = \cup_{\ell=1}^k J_{\ell}$.
Note that, as in Section~\ref{sec:str}, $I_k$ correspond to high quantile, high value buyers and $J_k$ correspond to low quantile, low value buyers.

% The proof of Theorem~\ref{thm:non_fsd} follows fairly straightforwardly from the following two lemmas.
% \begin{restatable}{lemma}{lemmacontbign}
%     \label{lemma:cont_big_n}
%     Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
%     Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
%     Then
%     \[
%         \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
%     \]
% \end{restatable}

The remainder of this section is structured as follows.
Subsection~\ref{subsec:defining_events} defines the various events we utilize to prove Theorem~\ref{thm:non_fsd}.
Two of the events are nearly identical to the events used in Section~\ref{sec:str} but we require one additional event that shows that each interval
contains roughly the ``right'' number of agents.
Subsection~\ref{subsec:cont_prob} analyzes the increase of GFT by using STR in the augmented market compared with OPT in the original market.
Finally, in Subsection~\ref{subsec:proof_non_fsd}, we summarize the arguments and prove Theorem~\ref{thm:non_fsd}.

\subsection{Constructing the Events}
\label{subsec:defining_events}
In this section, we define and analyze the events that we utilize to prove Theorem~\ref{thm:non_fsd}.

\paragraph{The event $\cE_3$.}
Define the event $\cE_3$ as the event that
\begin{equation}
\label{eqn:contE3def}
\begin{aligned}
    \cE_3 = \{
    & |I_{\leq 2} \cap \Bold| \leq 4pm,
    |(1-r/2, 1] \cap \Bold| \geq r n / 4, \\
    & |J_{\leq 2} \cap \Sold| \leq 4pm,
    |[0, r/2) \cap \Sold| \geq r n / 4
    \}
\end{aligned}
\end{equation}
At a high-level, we should think of $\cE_3$ as the event that each interval contains roughly the right number of original buyers and original sellers.
We require the following fact which will be used repeatedly.
\begin{claim}
    \label{claim:non_fsd_orig_matched}
    Condition on event $\cE_3$.
    In the original first-best matching, every original buyer in $I_{\leq 2}$ is matched
    and every original seller in $J_{\leq 2}$ is matched.
    Furthermore, in the augmented first-best matching, every buyer in $I_{\leq 2}$ is matched and every seller in $J_{\leq 2}$ is matched.
\end{claim}
\begin{proof}
    First, we prove that every original buyer in $I_{\leq 2}$ is matched.
    Let $k = |I_{\leq 2} \cap \Bold|$ be the number of original buyers in $I_{\leq 2}$.
    Note that $k \leq 4pm = 4 r n / 100 < r n / 4$, where the first inequality is by definition of $\cE_3$ (see Eq.~\eqref{eqn:contE3def}).
    Using the definition of event $\cE_3$ again, since $|(1-r/2, 1] \cap \Bold| \geq r m / 4$ and $|[0, r/2) \cap \Sold| \geq r n / 4$, we must have $\qbo(k) \geq 1 - r/2$ and $\qso(k) \leq r / 2$.
    By Lemma~\ref{lemma:r_fsd}, $b(\qbo(k)) \geq b(1-r/2) \geq s(r/2) \geq s(\qso(k))$ and thus every original buyer in $I_{\leq 2}$ is matched.

    The proof for the sellers is similar.
    Let $t = |J_{\leq 2} \cap \Sold|$ be the number of original sellers in $J_{\leq 2}$.
    When $\cE_3$ happens, we have $t \leq 4pm = 4 r n / 100 < r n / 4$.
    Following the identical logic above, we conclude that $s(\qso(t)) \leq s(r/2)\leq b(1-r/2) \leq b(\qbo(t))$ and thus every original seller in $J_{\leq 2}$ is matched.
    This proves the first assertion.

    The proof for the second assertion is nearly identical and is omitted.
\end{proof}


The following lemma shows that $\cE_3$ happens with high probability.
\begin{lemma}
    \label{lemma:cont_probE3_bound}
    $\prob{\cE_3} \geq 1 - 4\exp\left( -rn/300 \right)$.
\end{lemma}
\begin{proof}
    Since $|I_{\leq 2} \cap \Bold|$ can be written as a sum of i.i.d.~random variables and $\expect{|I_{\leq2} \cap \Bold|} = 2pm$,
    an application of the Chernoff Bound (see Lemma~\ref{lemma:chernoff}) gives
    \[
        \prob{|J_{\leq 2} \cap \Sold| \geq 4pm}
        \leq
        \prob{|I_{\leq 2} \cap \Bold| \geq 4pm} 
        \leq \exp\left( - pm / 3 \right)=\exp(-rn/300).
    \]
    Next, $\expect{|[0, r/2) \cap \Sold|} = rn/2$.
    So
    \[
        \prob{|(1-r/2, 1] \cap \Bold| \leq rn/4}
        \leq \prob{|[0, r/2) \cap \Sold| \leq rn/4}
        \leq \exp\left( - rn / 24 \right).
    \]
    % Similarly,
    % \[
    %     \prob{|[0, r/2) \cap \Sold| \leq rn/4} = \exp\left( -r^2 n / 2 \right).
    % \]
    By union bound we conclude that $\prob{\neg\cE_3} \leq 4 \exp\left( - rn / 300 \right)$.
    %The lemma follows by taking a complement.
\end{proof}
%\mingfei{One minor thing I changed: use $\neg \cE$ for the complement instead of $\overline{\cE}$ as the line connects with the brackets in the prob, e.g. $\prob{\overline{\cE}}$. }
%\chris{Sounds good. We can change it everywhere to be consistent.}

The following lemma bounds the loss on the GFT when the event $\cE_3$ is not satisfied. We denote $q_B\sim I_1$ the random variable $q_B$ drawn uniformly at random from the interval $I_1$. Similarly for $q_S\sim J_1$.
\begin{lemma}\label{lemma:expectation_E3}
    We have that
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq 4m \cdot \exp\left(- rn / 300 \right) \cdot
        \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    In particular, for any $\eta\in (0,1)$, if $n \geq \frac{300 \log(4m / \eta)}{r}$ then
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq \eta \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
    We write
    \begin{align*}
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}}
        & = \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}.
    \end{align*}
    Note that $\OPT(\Bq) - \STR(\Bq) \leq (\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qbo(j))\})_+$.
    \chrisnote{For the proof, we consider the following process to generate random uniform quantiles.
    First, for every agent, we assign them the label $1$ with probability $p$, the label $2$ with probability $p$, the label $3$ with probability $r/2 - 2p > 0$, and the label $4$ with the remaining probability. Note that the event $\neg \cE_3$ is defined via these labels. For example, the event that $|I_{\leq 2} \cap \Bold| \leq 4pm$ is the event that at most $4pm$ original buyers have the label $1$ or $2$.
    For the second step, we assign quantiles as follows.
    \begin{enumerate}[itemsep=0pt, topsep=0pt]
        \item Every buyer with label $1$ is assigned a uniform random quantile from $I_1$.
        \item Every buyer with label $2$ is assigned a uniform random quantile from $I_2$.
        \item Every buyer with label $3$ is assigned a uniform random quantile from $(1-r/2, 1] \setminus I_{\leq 2}$.
        \item Every buyer with label $4$ is assigned a uniform random quantile from $[0, 1-r/2]$.
    \end{enumerate}
    The sellers are assigned quantiles in an analogous manner. Note that each agent receives a uniformly random quantile.}
    
    \chrisnote{We claim that the random variable $\max_{i \in [m]}\{b(\qbo(i))\}$ is first-order stochastically dominated by the random variable $\max_{i \in [m]} \{b(\qb'(i))\}$ where $\qb'(1), \ldots, \qb'(m) \sim I_{1}$ uniformly at random. Indeed, fix any labelling as described above. If $k = 0$ then the stochastic-dominance is trivial. Otherwise, conditioned on $k\geq 1$ original buyers with the label $1$, we know that}
    \[
        \max_{i \in [m]} \{b(\qbo(i))\} \stackrel{d}{=} \max_{i \in [k]} \{b(\qb'(i)\} \stackrel{d}{\leq} \max_{i \in [m]}\{b(\qb'(i))\},
    \]
    \chrisnote{where we used $\stackrel{d}{=}$ to denote equal in distribution and $\stackrel{d}{\leq}$ to denote first-order stochastic dominance. As the stochastic dominance is true for every labelling, it follows that $\max_{i \in [m]} \{b(\qbo(i)\}$, conditioned on $\neg \cE_3$, is first-order stochastically dominated by $\max_{i \in [m]} \{b(\qb'(i))\}$.
    By an analogous argument, and since $m \geq n$, conditioned on $\neg \cE_3$, we can show that $-\min_{j \in [n]} \{s(\qso(j)\}$ is first-order stochastically dominated by $-\max_{j \in [m]} \{s(\qs'(j)\}$ where $\qs'(1), \ldots, \qs'(m) \sim J_{1}$ uniformly at random.}
    
    Thus, we have
    \begin{align*}
        \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3}
        & = \expectg{\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qso(j))\} }{\neg \cE_3} \\
        & \leq \expect{\max_{i \in [m]} \{b(\qb'(i))\} - \min_{j \in [m]} \{s(\qs'(j))\} } \\
        & \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}
    \end{align*}
    % We observe that, conditioned on $\cE_3$, $\OPT(\Bq) - \STR(\Bq)$ is first-order stochastically dominated by the random variable $\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}$ where $\qb'(i) \sim I_1$ (resp.~$\qs'(j) \sim J_1$) i.i.d.~and uniformly at random.
    % Let $\Bq'$ denote these auxiliary quantiles.
    % We thus have
    % \[
    %     \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3} \leq
    %     \expects{\Bq'}{\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}}
    %     \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    % \]
    Combining the inequality with Lemma~\ref{lemma:cont_probE3_bound} completes the proof.
\end{proof}

It remains to lower bound the GFT difference $\STR(\Bq)-\OPT(\Bq)$ when $\cE_3$ is satisfied. Similar to \Cref{sec:str}, we construct the following two events.

\paragraph{The good event $\cE_1$.}
Define $\cE_1$ as
\[
    \cE_1 = \{ \Bq : |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_1 \cap \Snew| \geq 2, |J_2 \cap \Sold| \geq 1 \}.
\]
We prove that $\cE_1\cap \cE_3$ is a sufficient condition for $\STR(\Bq)\geq \STR(\Bq)$. Moreover, we prove a lower bound on the expected GFT increase conditioned on $\cE_1\cap \cE_3$.
%on the event $\cE_1 \cap \cE_3$, we can obtain a strong lower bound on the GFT increase.
\begin{lemma}
    \label{lemma:cont_E1_lb}
    For any $\Bq \in \cE_1\cap \cE_3$, $\STR(\Bq) \geq \OPT(\Bq)$.
    Moreover,
    \[
        \expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_1\cap \cE_3} \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
Let $T$ be the number of trades in the original first-best matching.
We prove in the following claim that when $\cE_1\cap \cE_3$ happens, there are at least $T + 2$ trades in the augmented first-best matching.
\begin{claim}
    Recall that $\qbn(2)$ is the quantile of the second-highest new buyer and $\qsn(2)$ is the quantile of the second-lowest new seller. For any $\Bq\in \cE_1$, $b(\qbn(2)) \geq b(\qb(T+2)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
\end{claim}
\begin{proof}
    Let $\qb' \in I_2 \cap \Bold$ be the index of any original buyer in $I_2$ (by definition of $\cE_1$ there is at least one).
    By Claim~\ref{claim:non_fsd_orig_matched}, we have $\qb' \geq \qbo(T)$ (the buyer corresponding to quantile $\qb'$ is matched).
    On the event $\cE_1$, we have $|I_1 \cap \Bnew| \geq 2$ and thus $\qbn(2) \geq \qb' \geq \qbo(T)$.
    Therefore, $\qbn(2) \geq \qb(T+2) \geq \qbo(T)$ as both the highest and second-highest new buyer have quantile no less than $\qbo(T)$.
    A similar argument shows that $\qsn(2) \leq \qs(T+2) \leq \qso(T)$.
    We conclude that $b(\qbn(2)) \geq b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
    Here the first inequality follows from the fact that there are $T$ trades in the original first-best matching.
\end{proof}
Recall that that $\STR(\Bq) \geq \sum_{t=1}^{T+1} b(\qb(t)) - s(\qs(t))$
and $\OPT(\Bq) = \sum_{t=1}^T b(\qbo(t)) - s(\qso(t))$.
Since $\{\qb(1), \ldots, \qb(T+1)\} \setminus \{\qbn(1)\}$ consists of the top $T$ buyer quantiles except the highest \emph{new} buyer quantile and $\{\qbo(1), \ldots, \qbo(T)\}$ consist only of the top $T$ \emph{original} buyer quantiles, we have $\sum_{t=1}^{T+1} b(\qb(t)) - b(\qbn(1)) \geq \sum_{t=1}^T \qbo(t)$.
By a similar argument, we have $\sum_{t=1}^{T+1} s(\qs(t)) - b(\qsn(1)) \leq \sum_{t=1}^T \qso(t)$,
whence $\STR(\Bq) - \OPT(\Bq) \geq b(\qbn(1)) - s(\qsn(1))$.

Finally, we check that $\expectg{b(q(\inew_1))}{\cE_1\cap \cE_3} \geq \expects{\qb \sim I_1}{b(\qb)}$ (and analogously for the seller).
Note that if $\qb \sim I_1$ uniformly at random then $\qbn(1)$, conditioned on $|I_1 \cap \Bnew| \geq 2$, FSD $\qb$.
In addition, since the random variables $\qbn(1)$ and $|I_1 \cap \Bnew|$ are independent of the events $\cE_3$ and the random variables $|I_2 \cap \Bold|$, $|J_1 \cap \Snew|$ and $|J_2 \cap \Sold|$, we have
\[
    \expectg{b(\qbn(1))}{\cE_1\cap \cE_3} = \expectg{b(\qbn(1))}{|I_1 \cap \Bnew| \geq 2} \geq \expects{\qb \sim I_1}{b(\qb)}.
\]
A similar argument gives that $\expectg{s(\qsn(1))}{\cE_1\cap \cE_3} \leq \expects{\qs \sim J_1}{s(\qs)}$.
\end{proof}

% \chris{For the following, I think we need one more condition which is that there are at least $n+c$ buyers in the interval $[0, 2n/m]$.}
\paragraph{The bad event $\cE_2$.}
We define the bad event
\[
    \cE_2 = \neg\cE_1 \cap (\{ \Snew \cap (r/2, 1] = \Snew \} \cup \{ |\Bold \cap (1-r/2, 1]| < n + c\})
\]
In other words, the event requires that: (1) $\cE_1$ does not happen; (2) either every new seller has quantile in $(r/2, 1]$, or there are at least $n+c$ old buyers with quantile in $(1-r/2, 1]$. 
%all the new sellers are in the top $\gamma$ quantiles.
\begin{lemma}
    \label{lemma:contNotE2Better}
    % Meant to be a version of Lemma~\ref{lemma:notE2_STR_gt_OPT}.
    For any $\Bq \in \cE_3\cap \neg\cE_2$, we have $\STR(\Bq) \geq \OPT(\Bq)$.
\end{lemma}
\begin{proof}
    If $\Bq \in \cE_3$ but $\Bq \in \cE_1$ then we know from Lemma~\ref{lemma:cont_E1_lb} that $\STR(\Bq) \geq \OPT(\Bq)$.
    It remains to check that if $\Bq \in \cE_3 \cap \{\Snew \cap (1-\gamma, 1] \neq \Snew\} \cap \{|\Bold \cap (1-r/2, 1]| \geq n+c\}$ then $\STR(\Bq) \geq \OPT(\Bq)$.
    Let $\OPT'(\Bq)$ be the first-best matching in the augmented market.
    Suppose that $\OPT(\Bq)$ has $T \leq n$ trades.
    We consider two cases, depending on the number of trades in $\OPT'(\Bq)$.

    \paragraph{Case 1: $\OPT'(\Bq)$ has $T+1$ trades.}
    In this case, $\STR(\Bq)$ trades the top $T$ highest value (original and new) buyers and the bottom $T$ lowest value (original and new) sellers (but it could trade more). In particular, $\STR(\Bq) \geq \OPT(\Bq)$.

    \paragraph{Case 2: $\OPT'(\Bq)$ has $T$ trades.}
    Here, we want to show that $\STR(\Bq) = \OPT'(\Bq)$.
    By definition of STR, it suffices to show that $b(q(T)) \geq s(q(T+1))$.
    We claim that $\qso(T) > r/2$.
    For the sake of contradiction, suppose that $\qso(T) \leq r/2$.
    Since $\Bq \in \{\Snew \cap (r/2, 1] \neq \Snew\}$, this implies that $\qsn(1) \leq r/2$.
    But this means $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} \leq r/2$.
    However, since $|\Bold \cap (1-r/2, 1]| \geq n+c$ and $T \leq n$, it must be that $\qb(T+1) \geq \qbo(T+1) \geq 1-r/2$.
    But then by Lemma~\ref{lemma:r_fsd}, we would have $b(\qb(T+1)) \geq s(\qs(T+1))$ contradicting that $\OPT'(\Bq)$ has $T$ trades.
    We thus conclude that $\qso(T) > r/2$.
    
    To finish the proof, we have
    \[
        b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+1)). 
    \]
    The first inequality is because $\qb(T) \geq \qbo(T)$.
    The second inequality follows from the fact that $\OPT$ has $T$ trades.
    The last inequality holds because $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} = \qso(T)$ since $\qsn(1) \leq r/2 < \qso(T)$.
\end{proof}

\begin{lemma}
\label{lemma:cont_bound_loss_E2}
We have $\expectsg{\Bq}{\OPT(\Bq) - \STR(\Bq)}{\cE_2\cap \cE_3} \leq \expects{\qb \sim I_1, \qs \sim J_1}{b(\qb) - s(\qs)}$.
\end{lemma}
\begin{proof}
    Let $\OPT'(\Bq)$ be the GFT of the first-best matching in the augmented market.
    Let $b^*(\Bq)$ (resp.~$s^*(\Bq)$) denote the lowest (resp.~highest) value among buyers (resp.~sellers) traded in the augmented first-best matching.
    Let $\cF$ be the event that there is no trade in the first-best matching in the augmented market and let $b^*(\Bq) = 0$ and $s^*(\Bq) = 0$ if no trade exists in $\OPT'(\Bq)$.
    By definition of the STR mechanism, we have $\OPT(\Bq) - \STR(\Bq) \leq \OPT'(\Bq) - \STR(\Bq)\leq (b^*(\Bq)-s^*(\Bq)) \cdot \ind{\cF}$.

    We will show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \leq \expects{q_B \sim I_1}{b(\qb)}$. An analogous argument can be used to show that $\expectg{s^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \geq \expects{\Bs \sim J_1}{s(\qs)}$.
    We consider three cases.
    
    \chrisnote{Note that for the proof, we will make use of the following two-stage process to sample $\Bq$, which we describe only for the buyers (the sellers' description is analogous).
    First, we assign original and new buyers with two labels.
    For the first label, we assign them a label in $\{1, \ldots, \lceil 1/p \rceil\}$ where label $\ell \in [\lceil 1/ p \rceil]$
    is assigned with probability equal $\mu(I_\ell \cap [0, 1])$. Here $\mu$ denotes the Lebesgue measure.
    For the second label, if the first label is $\ell$ then we assign the second label $1$ with probability $\mu(I_{\ell} \cap (1-r/2, 1]) / \mu(I_{\ell})$ and $0$ otherwise.
    Note that except for one label $\ell'$ all labels $\ell \neq \ell'$ result in second labels having probability either $1$ or $0$.
    In particular, the label $(1,0)$ occurs with probability $0$ since $I_1 \cap (1-r/2, 1] = I_1$.
    For the second-stage, if a buyer is assigned the label $(\ell, 1)$ then we assign it a uniform random quantile from $(1-r/2, 1] \cap I_{\ell}$ and if it is assigned the label $(\ell, 0)$ then we assign it a uniform random quantile from $[0, 1-r/2) \cap I_{\ell}$.
    Note that with this process, every buyer is assigned a uniform random quantile from $[0, 1]$.}
    
    \chrisnote{Given this process, it is straightforward to maps the events $\cE_2, \cE_3$ to description about labels.
    For example, the event $|I_{\leq 2} \cap \Bold| \leq 4pm$ is equivalent to the event that at most $4pm$ original buyers are assigned a first label of $1$ or $2$ and the event $|(1-r/2, 1] \cap \Bold| \geq rn/4$ is equivalent to the event at least $rn/4$ original buyers are assigned a second label of $1$.}

    \paragraph{Case 1: $|I_1 \cap \Bnew| \geq 1$.}
    Let $\cE' = \{ |I_1 \cap \Bnew| \geq 1 \}$. \chrisnote{This is equivalent to the event that at least one new buyer is assigned a first label of $1$ in the above two-stage sampling process.}
    % To sample $\Bq$ such that $\Bq \in \cE' \cap \cE_2 \cap \cE_3$, we can first sample a quantile $\qb \sim I_1$ for a new buyer and then sample the remainder of $\Bq$.
    Conditioned on $\cE_3$, by Claim~\ref{claim:non_fsd_orig_matched}, we know that every new buyer in $I_1$ is traded (because every buyer in $I_1$ is traded).
    Let $\cG_k$ be the event that there are exactly $k$ new buyers in $I_1$.
    On the event $\cG_k \cap \cE_3 \cap \cE_2$ (provided that this event is non-empty), $b^*(\Bq)\ind{\cF} = b^*(\Bq) \leq \min_{i\in[k]} b(q'(i))$, where $q'(1), \ldots, q'(k)$ are $k$ uniform random quantiles from $I_1$.
    Note that $\min_{i \in [k]} b'(q(i))$ is first-order stochastically dominated by $b(\qb)$ where $\qb \sim I_1$ uniformly at random.
    Thus, $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    This is true for every $k$ such that $\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k \neq \emptyset$ so we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 2: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| \geq 1$.}
    This case is very similar to the above.
    Let $\cE'' = \{|I_1 \cap \Bnew| = 0, |I_1 \cap \Bold| \geq 1\}$.
    In this case, we define $\cG_k$ as the event that there are exactly $k$ \emph{original} buyers in $I_1$.
    Following an identical proof, we can show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    Thus, we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE''} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 3: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| = 0$.}
    This case is fairly trivial.
    Let $\cE''' = \{I_1 \cap \Bnew = I_1 \cap \Bold = \emptyset\}$.
    Then $b^*(\Bq)\ind{\cF} \leq b(1-p)\ind{\cF} \leq \expects{\qb \sim I_1}{b(\qb)} \ind{\cF}$ either because there is no trade or every traded buyer has a quantile outside $I_1$.
    
    Combining the three cases above concludes the proof.
\end{proof}

\subsection{Comparing STR and OPT in different regimes}
\label{subsec:cont_prob}
Let $\alpha \in (0, 1)$ be a constant decided later. We split the analysis into the regime where $n \geq \alpha m$ and $n \leq \alpha m$.
\paragraph{Case 1: $n \geq \alpha m$.}
\begin{lemma}
    \label{lemma:contProbE1}
    $\prob{\cE_1} \geq 1 - 6c(1-p)^c$.
\end{lemma}
\begin{proof}
    We have
    \[
        \prob{|I_1 \cap \Bnew| \leq 1}
        = (1-p)^c + c(1-p)^{c-1} p
        = (1-p)^c \left[ 1 + cp/(1-p) \right]
        < 2c (1-p)^c
    \]
    The inequality uses that $p=\frac{rn}{100m}\leq\frac{1}{100}$. Thus $p(1-p) \leq 1/4$ and $1 + c/4 \leq c + c/4 < 2c$ since $c \geq 1$.
    Identical calculations give
    \[
        \prob{|J_1 \cap \Snew| \leq 1} < 2c(1-p)^c
    \]
    Next, we have $\prob{|I_2 \cap \Bold| = 0} \geq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq (1-p)^c$ since $n\geq c$.
    Taking a union bound gives that $\prob{\neg\cE_1} \leq 6c(1-p)^c$.
\end{proof}
\begin{lemma}
    \label{lemma:cont_big_n}
    Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
    Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
    Then
    \[
        \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
    \]
\end{lemma}
% \lemmacontbign*
\begin{proof}[Proof of Lemma~\ref{lemma:cont_big_n}]
    Note that $\cE_1$ and $\cE_2$ are disjoint, we have
    \begin{align}
        \expect{\STR(\Bq) - \OPT(\Bq)}
        & = \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1\cap\cE_3} \label{eq:contE1E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2\cap\cE_3} \label{eq:contE2E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \cdot \prob{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \label{eq:contNotE1NotE2E3}\\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3} \label{eq:contE3}
    \end{align}
    For Eq.~\eqref{eq:contE1E3}, we use Lemma~\ref{lemma:cont_E1_lb}, Lemma~\ref{lemma:cont_probE3_bound}, and Lemma~\ref{lemma:contProbE1}, along with a union bound to get that
    \begin{multline*}
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1 \cap \cE_3} \\ \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot \left( 1 - 6c(1-p)^c - 4 \exp(-rn/300) \right).
    \end{multline*}
    For Eq.~\eqref{eq:contE2E3}, we use Lemma~\ref{lemma:cont_bound_loss_E2}, Lemma~\ref{lemma:contProbE1}, and the fact that $\prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \prob{\neg\cE_1}$ to get
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2 \cap \cE_3} \geq - \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot 6c(1-p)^c
    \]
    For Eq.~\eqref{eq:contNotE1NotE2E3}, Lemma~\ref{lemma:contNotE2Better} gives
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \geq 0.
    \]
    Finally, for Eq.~\eqref{eq:contE3}, by \Cref{lemma:expectation_E3} we have
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}
        \geq - 4m \cdot \exp(-rn/300) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    Putting everything together, it suffices to check that
    \[
        1 - 6c(1-p)^c - 4\exp(-rn / 300) \geq 6c(1-p)^c + 4m \exp(-rn/300).
    \]
    %A sufficient condition is that 
    The above inequality holds if $12c(1-p)^c \leq 1/2$ and $8m\exp(-rn/300) \leq 1/2$.
    To prove $12c(1-p)^c \leq 1/2$, note that $p = rn/(100 m) \geq r \alpha / 100$ and thus by our choice of $c$, we have
    $c \geq 4\log(24/p) / p$.
    Therefore,
    \[
        12c(1-p)^c \leq 12ce^{-cp} = \frac{12cp e^{-cp}}{p} \leq \frac{12e^{-cp/2}}{p} \leq \frac{12e^{-\log(24/p)}}{p} = \frac{1}{2}.
    \]
    Note that in the second inequality, we used that $cp \geq 4$ and the numeric inequality $xe^{-x} \leq e^{-x/2}$ valid for $x \geq 4$ (see Claim~\ref{claim:xexp_lt_exp}).
    For the inequality $8m \exp(-rn / 300) \leq 1/2$, note that this follows from the assumption that $r \geq \frac{300 \log(16 m)}{r}$.
\end{proof}

\paragraph{Case 2: $n \leq \alpha m$.}
\begin{lemma}
    \label{lemma:cont_small_n_E1}
    Let $\alpha > 0$ and suppose that $n \leq \alpha m$ and $c \geq 2$.
    Then
    \[
        \prob{\cE_1} \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6.
    \]
\end{lemma}
\begin{proof}
    Since $|I_1 \cap \Bnew|$ and $|J_1 \cap \Snew|$ are both distributed as $\Binom(p, c)$, we have that
    \[
        \prob{|J_1 \cap \Bnew| = 2} = \prob{|I_1 \cap \Bnew| = 2} = \binom{c}{2} (1-p)^{c-2} p^2 \geq \frac{c^2}{4} (1-r\alpha / 100)^{c-2} p^2
    \]
    where we used that $p = rn/100m \leq r\alpha / 100$ and $\binom{c}{2} = c(c-1) / 2 \geq c^2 / 4$ since $c \geq 2$.
    Next, since $|I_2 \cap \Bold|$ is distributed as $\Binom(p, m)$ and $|J_2 \cap \Sold|$ is distributed as $\Binom(p, n)$, we have
    \[
        \prob{|I_2 \cap \Bold| = 0} \leq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq 1-p.
    \]
    Therefore, $\prob{|I_2 \cap \Bold| \geq 1} \geq \prob{|J_2 \cap \Sold| \geq 1} \geq p$.
    Since the random variables $|I_1 \cap \Bnew|, |J_1 \cap \Snew|, |I_2 \cap \Bold|, |J_2 \cap \Sold|$ are all independent, the lemma follows by taking a product.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n_E2}
    Suppose that $n \leq mr / 8$.
    Then $\prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3)$.
\end{lemma}
\begin{proof}
    Recall that $\cE_2 \subset (\{\Snew \cap (r/2, 1] = \Snew\} \cup \{|\Bold \cap (1-r/2, 1]| < n+c\})$.
    Since $|\Snew \cap (r/2, 1]|$ is distributed as $\Binom(1-r/2, c)$ we have that
    \[
        \prob{\Snew \cap (r/2, 1] = \Snew} = (1-r/2)^c \leq \exp(-rc/2). 
    \]
    Next, since $\expect{|\Bold \cap (1-r/2, 1]|} = mr/2 \geq 4n$, the Chernoff bound gives (Lemma~\ref{lemma:chernoff})
    \[
        \prob{|\Bold \cap (1-r/2, 1]| < n+c}
        \leq \prob{|\Bold \cap (1-r/2, 1]| < 2n}
        \leq \exp(-n/3).
    \]
    Using a union bound proves the lemma.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n}
    Suppose that $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100m / rn)}{r}$, $n \geq 150c + \frac{300}{r} \log(9m)$, and $n \leq mr/8$.
    Then $\expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0$.
\end{lemma}
\begin{proof}
    The proof is nearly identical to Lemma~\ref{lemma:cont_big_n} except that we replace the bounds on $\prob{\cE_1 \cap \cE_3}$ and $\prob{\cE_2 \cap \cE_3}$
    with Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_small_n_E2}, respectively.
    For the former, using Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_probE3_bound}, where $\alpha = r/8$,
    \[
        \prob{\cE_1 \cap \cE_3}
        = 1 - \prob{\neg\cE_1 \cup \neg\cE_3}
        \geq 1 - \prob{\neg\cE_1} - \prob{\neg\cE_3}
        \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c - 4} p^6 - 4\exp(-rn / 300).
    \]
    and for the latter, using Lemma~\ref{lemma:cont_small_n_E1}, we have
    \[
        \prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3).
    \]
    Continuing as in Lemma~\ref{lemma:cont_big_n}, we now require that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 - 4\exp(-rn/ 300)
        \geq
        \exp(-rc/2) + \exp(-n/3) + 4m \exp(-rn / 300).
    \]
    Rearranging, a sufficient condition is that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 \geq \exp(-rc / 2) + 9m \exp(-rn / 300).
    \]
    Using that $n \geq 150c + \frac{300}{r} \log(9m)$, one can verify that $9m \exp(-rn / 300) \leq \exp(-rc/2)$.
    Also, since $c \geq 2$, we have $c^4/16 \geq 1$.
    Rearranging further, it suffices to show that
    \[
        p^6 \geq \frac{2\exp(-rc/2)}{\left(1 - r\alpha/100 \right)^{2c-4}}.
    \]
    This latter inequality is true since
    \begin{align*}
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c-4}}
        & \leq
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c}} \\
        & \leq 2\exp(-rc / 2 + 4rc\alpha / 100) \\
        & \leq 2\exp(-rc / 4) \\
        & \leq \left( \frac{rn}{100m} \right)^6 = p^6,
    \end{align*}
    where the second inequality used the numeric inequality $1/(1-x) \leq e^{2x}$ valid for $x \in [0, 1/4]$ (see Claim~\ref{claim:one_over_one_minus_x_lt_exp}),
    the third inequality used that $\alpha \leq 1$ and thus, $-rc/2 + 4rc\alpha / 100 \leq -rc / 4$,
    and the last inequality is because $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100 m / rn)}{r}$.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:non_fsd}}
\label{subsec:proof_non_fsd}
Finally, we prove Theorem~\ref{thm:non_fsd}.
\begin{proof}[Proof of Theorem~\ref{thm:non_fsd}]
    Let $\alpha = r/8$.
    We first ``pre-augment'' the market so that we can apply the results from the previous section.
    Let $m \geq n$ be the original number of buyers and sellers.
    First, we add $O(\log(1/r)/r)$ buyers to get $m' = m + O(\log(1/r)/r)$ buyers and so that $m' \geq 300 \log(16m') / r$.
    If $n \leq 300 \log(16m') / r$ we add $300 \log(16m') / r - n = O(\log(m/n) / r)$ buyers \emph{and} sellers get a total of $m''$ buyers $n''$ sellers.
    Note that $m'' \geq 300 \log(16m'') / r$ and $n'' \geq 300 \log(16m'') / r$.
    
    Next, choose
    \[
        c \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m''/rn'')}{r} \right\} = O(\log(m/rn) / r).
    \]
    Let $\Delta_N = 150c + \frac{300}{r} \log(16m'') - n'' \leq 150c$.
    If $\Delta_N > 0$ then it straightforward, albeit somewhat cumbersome, calculation to check that setting $m''' = m'' + 200\cdot C \cdot \Delta_N$, $n''' = n'' + 200\cdot C \cdot \Delta_N$ and $c''' = c + C\cdot \Delta_N$ for a large enough constant $C > 0$, we have
    \begin{itemize}
        \item $m''' \geq n''' \geq 150c + \frac{300}{r} \log(16m''')$;
        \item $c''' \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m'''/rn''')}{r} \right\} = O(\log(m / rn) / r)$.
    \end{itemize}
    
    Finally, applying Lemma~\ref{lemma:cont_big_n} if $n''' \geq \alpha m'''$ and Lemma~\ref{lemma:cont_small_n} if $n''' \leq \alpha m'''$,
    we conclude that $\STR(m''' + c''',n''' + c''') \geq \OPT(m''',n''')$.
    Note that both $m'''+c''' - m$ and $n''' + c''' - n$ are $O(\log(m / rn) / r)$.
\end{proof}

\mingfeinote{
\subsection{Lower Bound}\label{subsec:non_fsd_lb}

We derive a lower bound on the number of additional agents with result of \cite{BabaioffGG20}.
%required for any deterministic, prior-independent, truthful, BB and anonymous mechanism.

\begin{lemma}\label{lem:bgg_lb}
\cite[Proposition~E.5]{BabaioffGG20} For any $\eps>0$ and any integer $m, n$, there exists a double auction instance with $m$ buyers, $n$ sellers, and distributions $F_B$, $F_S$ such that: (1) $\Pr_{b\sim F_B, s\sim F_S}[b\geq s]\geq \frac{\eps^2}{(m+n+2c)^8}$; (2) For any deterministic, prior-independent, BIC, IR, BB and anonymous\footnote{A mechanism is \emph{anonymous} if the mechanism treats each buyer and seller equally. In other words, swapping the identity of any two buyers (or sellers) will only result in their allocation and payment being swapped.} mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than $\eps$ times the first-best GFT on $m$ buyers and $n$ sellers.
\end{lemma}

\begin{corollary}\label{cor:non_fsd_lb}
For any sufficiently small $r\in (0,1)$, there exists a double auction instance with \\
$\Pr_{b\sim F_B, s\sim F_S}[b\geq s]=r$ such that: For any $c\leq \frac{1}{4}\cdot r^{-1/8}$ and any deterministic, prior-independent, BIC, IR, BB and anonymous mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than the first-best GFT on $m$ buyers and $n$ sellers.
\end{corollary}
\begin{proof}
Applying \Cref{lem:bgg_lb} with any $n\leq m\leq \frac{1}{4}\cdot r^{-1/8}$, we have $\eps\leq \sqrt{r(m+n+2c)^8}\leq 1$. The proof is done by \Cref{lem:bgg_lb}.  
\end{proof}
}
}

==> old_stuff/multiple_sellers.tex <==

\section{Multiple sellers}
\textcolor{red}{WIP.. just jotting down ideas, lemmas, etc.}
\chris{TODO: There is some mix of notation. I propose to use $i$ for buyer indices and $j$ for seller indices. Will change later.}

Assume for now that there are $m$ buyers and $m$ sellers.
Also assume that $m+c$ is even.
Define the sets $\Bold$, $\Bnew$, $\Sold$, $\Snew$ as the subsets of $[2(m+c)]$ that are assigned to
old buyers, new buyers, old sellers, and new sellers, respectively.
So $|\Bold| = |\Sold| = m$ and $|\Bnew| = |\Snew| = c$.
Fix $K \geq 4$ in this argument and assume that $m+c$ is divisible by $K$.
For $k \in [2K]$, define $I_k = \{(m+c) \cdot \frac{k-1}{K} + 1, \ldots, (m+c) \cdot \frac{k}{K}\}$.
Consider the event $\cE_1$ defined as
\begin{itemize}[itemsep=0pt, topsep=0pt]
    \item $|I_1 \cap \Bnew| \geq 2$, i.e.~at least $2$ new buyers are in $I_1$;
    \item $|I_2 \cap \Bold| \geq 1$, i.e.~at least $1$ old buyer is in $I_2$;
    \item $|I_{2K-1} \cap \Sold| \geq 1$, i.e.~at least $1$ old sellers is in $I_{2K-1}$;
    \item $|I_{2K} \cap \Snew| \geq 2$, i.e.~at least $2$ new sellers are in $I_{2K}$.
\end{itemize}
The next claim shows that on the event $\cE_1$, the gain in trade reduction is at least the value of the optimal match among only the new buyers and sellers.
\begin{claim}
    On the event $\cE_1$, we have $\TR - \OPT \geq b(q(i_{b, 1}^n)) - s(q(i_{s, 1}^n))$.
    % Condition on the event $\cE_1$ and let $q_b^*$ be the highest quantile among the new buyers and $q_s^*$ be the lowest quantile among the new sellers.
    % Then $\TR - \OPT \geq b(q_b^*) - s(q_s^*)$.
\end{claim}
\begin{proof}
    Condition on event $\cE_1$ and suppose that initially $\OPT$ had $T$ trades.
    Let $i_{b, 1}^o < \ldots < i_{b, m}^o$ be the indices of the $m$ original buyers
    and $i_{s, 1}^o > \ldots > i_{s, m}^o$ be the indices of the $m$ original sellers. We notice that a smaller index corresponds to a larger quantile and thus a larger value or cost. Similarly, let $i_{b, 1}^n < \ldots < i_{b, c}^n$ be the indices of the $c$ new buyers
    and $i_{s,1}^n > \ldots > i_{s, c}^n$ be the indices of the $c$ new sellers.
    We also let $i_{b, 1} < \ldots < i_{b, m+c}$ be the indices of all $m+c$ buyers
    and $i_{s, 1} < \ldots < i_{s, m+c}$ be the indices of all $m+c$ sellers.

\begin{claim}
    \label{claim:all_I2_trades}
    Suppose $K \geq 4$ and $c \leq m$.
    In the original optimal matching, every original buyer in $I_2$ is matched and every original seller in $I_{2K-1}$ is matched.
\end{claim}
\begin{proof}
    We prove only that every original buyer in $I_2$ is matched since the argument that every seller in $I_{2K-1}$ is matched is identical.

    Let $r$ be the total number of original buyers in $I_1 \cup I_2$.
    Note that $r \leq \frac{2(m+c)}{K}$.
    We prove that there are at least $r$ sellers outside of $I_1 \cup I_2$ which implies the claim (because the top $r$ buyers and bottom $r$ sellers certainly participate in trades).
    The total number of sellers in $I_1 \cup I_2$ is upper bounded by $\frac{2(m+c)}{K}$.
    Since there are $m$ original sellers, there must be at least $m - \frac{2(m+c)}{K}$ original sellers in \mingfeinote{outside of} $I_1 \cup I_2$.
    However,
    \[
        m - \frac{2(m+c)}{K}
        \geq
        \frac{m+c}{2} \cdot \left( 1 - \frac{2}{K} \right)
        \geq \frac{2(m+c)}{K}\mingfeinote{\geq r}
    \]
    where in the first inequality we used that $m \geq \frac{m+c}{2}$
    and in the second inequality we used that $1 - \frac{2}{K} \geq \frac{2}{K}$ when $K \geq 4$.
\end{proof}
    
    \begin{claim}
        \label{claim:T_plus_2_trades}
        $b(q(i_{b, T+2})) \geq s(q(i_{s, T+2}))$.
    \end{claim}
    \begin{proof}
        Let $i_b^o \in I_2 \cap \Bold$ be the index of any original buyer in $I_2$.
        By Claim~\ref{claim:all_I2_trades}, $q(i_b^o) \geq q(i_{b, T}^o)$ since $i_b^o$ must be matched.
        Recall that $i_{b, 1}^n < i_{b, 2}^n$ are the indices of the top $2$ new buyers.
        By the assumption that $|I_1 \cap \Bnew| \geq 2$, we know that $q(i_{b, 2}^n) \geq q(i_b^o) \geq q(i_{b, T}^o)$.
        Therefore, $q(i_{b, T+2}) \geq q(i_{b, T}^o)$.
        A similar argument shows that $q(i_{s, T+2}) \leq q(i_{s, T}^o)$.
        We conclude that $b(q(i_{b, T+2})) \geq b(q(i_{b, T}^o)) \geq s(q(i_{s, T}^o)) \geq s(q(i_{s, T+2}))$. \mingfeinote{Here the second inequality follows from the fact that there are $T$ trades in original setting.}
    \end{proof}
    
    We are now ready to show that $\TR - \OPT \geq b(q(i_{b, 1}^n)) - s(q(i_{s, 1}^n))$.
    Let $i_{b, 1}' < \ldots < i_{b, T+1}' = i_{b, T+2}$ be the smallest indices in $B' \coloneqq \Bold \cup \Bnew \setminus \{i_{b, 1}^n\}$
    and $i_{s, 1}' > \ldots > i_{s, T+1}' = i_{s, T+2}$ be the largest indices in $S' \coloneqq \Sold \cup \Snew \setminus \{i_{s, 1}^n\}$.
    Since $B' \supset \Sold$, we have $i_{b, t}' \leq i_{b, t}^o$ for all $t \in [T]$.
    Similarly, since $S' \supset \Bold$, we have $i_{s, t}' \geq i_{s, t}^o$ for all $t \in [T]$.
    Therefore,
    \begin{equation}
        \label{eqn:OPT_UB}
        \OPT \leq \sum_{t=1}^{T} b(q(i_{b, t}')) - s(q(i_{s, t}')).
    \end{equation}
    Next, we give a lower bound on $\TR$.
    By Claim~\ref{claim:T_plus_2_trades}, the top $T+1$ buyers and bottom $T+1$ sellers participate in trades in trade reduction.
    Moreover, Claim~\ref{claim:all_I2_trades} shows that $i_{b, 1}^n < i_{b, T+1}'$ and $i_{s, 1}^n > i_{s, T+1}'$.
    Thus, both $i_{b, 1}^n$ and $i_{s, 1}^n$ participate in a trade in trade reduction.
    Therefore, we have
    \begin{equation}
        \label{eqn:TR_LB}
        \TR \geq \left( b(q(i_{b,1}^n)) - s(q(i_{s,1}^n)) \right) + \sum_{t=1}^T b(q(i_{b, T}')) - s(q(i_{s, T}')).
    \end{equation}
    Combining Eq.~\eqref{eqn:OPT_UB} and Eq.~\eqref{eqn:TR_LB}, we conclude that $\OPT - \TR \geq b(q(i_{b, 1}^n)) - s(q(i_{s, 1}^n))$.
\end{proof}


Following claim is for the augmented setting.
\chris{As far as I can tell right now, we only need the claim for $L = 1$.}
\begin{claim}
    \label{claim:all_high_trades}
    Let $L \leq 2K$.
    If there are $r$ buyers in $\cup_{\ell=1}^L I_{\ell}$ then the size of the augmented optimal matching is at least $r$.
    Similarly, if there are $r$ sellers in $\cup_{\ell=1}^L I_{2K + 1 - \ell}$ then the size of the augmented optimal matching is at least $r$.
\end{claim}
\begin{proof}
    We prove only the first assertion since the second assertion is nearly identical.

    First, we prove that there are at least $r$ sellers \emph{not} in $I \coloneqq \cup_{\ell=1} I_{\ell}$.
    Indeed, the total number of sellers is $m+c$.
    There can be at most $(m+c) \cdot \frac{L}{K}$ sellers in $I$ and so there are at least $(m+c) \cdot \left( 1 - \frac{L}{K} \right) \geq (m+c) \cdot \frac{L}{K} \geq r$ sellers not in $I_1$.
    (The second last inequality used that $K \geq 2L$.)
    Since there are $r$ buyers in $I$ and $r$ sellers not in $I$, there must be at least $r$ trades in the optimal matching.
\end{proof}

Let $\cE_2$ be the event that $|I_1 \cap \Bnew| \leq 1$ \emph{and} $|I_{2K} \cap \Snew| \leq 1$,
i.e.~there is at most $1$ new buyer in $I_1$ and at most $1$ new seller in $I_{2K}$.
Note that this event is slightly larger than \mingfeinote{smaller than} the complement of the event $\cE_1$.
\newcommand{\OPTnew}{\OPT_{\textsc{New}}}
Let $\OPTnew$ be the optimal GFT with the augmented sellers and buyers.
\begin{lemma}
    $\expectg{\OPT - \TR}{\cE_2} \leq \expectg{\OPTnew - \TR}{\cE_2} \leq \expects{i, j}{b(q(i)) - s(q(j))}$
    where $i \sim I_1, j \sim I_{2K}$ uniformly at random.
\end{lemma}
\begin{proof}
    The first inequality is trivial. We prove only the second inequality.

    Let $B = \Bold \cup \Bnew$ be all the buyer indices and let $S = \Sold \cup \Snew$ be all the seller indices.
    Let $\cF_r$ be the event that $|I_1 \cap B| = r$.
    By Claim~\ref{claim:all_high_trades}, there are at least $r$ trades.
    Let $i_1 < \ldots < i_{m+c}$ be the indices of the buyers sorted in decreasing values
    and let $j_1 > \ldots > j_{m+c}$ be the indices of the sellers sorted in increasing values.
    We further partition $\cF_r$ into two events $\cF_{r, 1}, \cF_{r, 2}$
    where $\cF_{r, 1} = \cF_r \cap \{j_r \in I_{2K}\}$ and $\cF_{r, 2} = \cF_r \cap \{j_r \notin I_{2K}\}$.
    Note that, on the event $\cF_r$, we have $\OPT - \TR \leq b(q(i_r)) - s(q(i_r))$.

    Now observe that
    \[
        \expectg{b(q(i_r)) - s(q(j_r))}{\cE_2 \cap \cF_{r, 1}}
        \leq \expects{i, j}{b(q(i)) - s(q(j))},
    \]
    where $i \in I_1, j \in I_{2K}$ uniformly at random.
    This is because on the event $\cE_2 \cap \cF_{r,1}$ there are exactly $r$ buyer quantiles in $I_1$
    \chris{Fix here since if $i_r \in I_{2K}$ there could be more than $r$ sellers in $I_{2K}$.}
    and $i_r$ is the maximum of $r$ uniform random indices drawn from $I_1$ without replacement.
    Similarly, $j_r$ is the minimum of $r$ uniform random indices drawn from $I_{2K}$ without replacement.
    
    Next, we also have that
    \[
        \expectg{b(q(i_r)) - s(q(j_r))}{\cE_2 \cap \cF_{r, 2}}
        \leq \expects{i, j}{b(q(i)) - s(q(j))}.
    \]
    The argument for $i_r$ is as above.
    Note that $j_r \notin I_{2K}$ on the event $\cF_{r, 2}$ so it is clearly upper bounded by a uniform random index from $I_{2K}$.
\end{proof}

We now bound the probabilities.
\begin{lemma}
    $\prob{\cE_1} \geq ???$
\end{lemma}
\begin{proof}
    Let
    \begin{itemize}[itemsep=0pt, topsep=0pt]
        \item $\cE_{1, 1} = \{ |I_1 \cap \Bnew| \geq 2 \}$;
        \item $\cE_{1, 2} = \{ |I_2 \cap \Bold| \geq 1 \}$;
        \item $\cE_{1, 3} = \{ |I_3 \cap \Sold| \geq 1 \}$;
        \item $\cE_{1, 4} = \{ |I_4 \cap \Snew| \geq 2\}$;
    \end{itemize}
    
\mingfeinote{
$$\Pr[\neg\cE_{1, 1}] = \Pr[\neg\cE_{1, 4}] = \frac{\binom{2m+c}{2(m+c)/K}+\binom{c}{1}\binom{2m+c}{2(m+c)/K-1}}{\binom{2(m+c)}{2(m+c)/K}}$$

$$\Pr[\neg\cE_{1, 2}] = \Pr[\neg\cE_{1, 3}] = \frac{\binom{m+2c}{2(m+c)/K}}{\binom{2(m+c)}{2(m+c)/K}}$$

}
\end{proof}

\begin{lemma}
    $\prob{\cE_2} \leq ???$
\end{lemma}

\subsection{General Case ($m_B\not=m_S$)}

\mingfeinote{Some random thoughts:

Ideally we want a small probability event which is a necessary condition for $\OPT>\TR$.

One observation: Suppose $\OPT$ trades $r$ pairs. If $\TR$ trades $\geq r$ pairs, or equivalently the opt in the augmented setting has one more trade, then $\TR\geq\OPT$.

Let $m_B=m, m_S=m'$, $m>m'$. When $m'=o(m^{0.5})$, we can try to use the argument for the single seller case. Let $\cE_1$ be the event that at most $m'$ buyers are in the top $m'+c$ quantile. When $\cE_1$ does not happen, there are at least $m'+1$ buyers in the top $m'+c$ and at least $m'+1$ sellers outside. So there are at least $m'$ trades in $\TR$ and so $\TR\geq\OPT$. $\cE_1$ should be a low prob event since in expectation there are only $(m'+c)\cdot m'/m=o(1)$ sellers in the top $m'+c$ quantile.  

When $m'$ is large, it feels like $\cE_1$ is too ambitious: the complement of $\cE_1$ results in a trade size of $m'$ in $\TR$ while as $m'$ increase, the efficient trade size $r$ becomes less than $m'$. 

}

==> old_stuff/old_stuff.tex <==
\clearpage
\textbf{\textcolor{red}{Below is buggy!!!}}


\paragraph{Notation.}
Let us assume there are $m_B \geq 1$ buyers and $m_S \geq 1$ sellers.
Each buyer has a value drawn i.i.d.~from some distribution $F_B$ and each seller has a distribution drawn i.i.d.~from some distribution $F_S$.
We assume that $F_B$ stochastically dominates $F_S$, i.e.~for every $v \geq 0$, we have $\probs{b \sim F_B}{b \geq v} \geq \probs{s \sim F_S}{s \geq v}$.

\paragraph{Trade Reduction.}
We consider the following version of trade reduction.
Let $b_1 \geq \ldots \geq b_{m_B}$ be the values of the buyers and let $s_1 \leq \ldots \leq s_{m_S}$ be the values of the sellers.
If $b_1 < s_1$ then do not trade.
Otherwise, let $i^* \in \max \setst{i \leq \min\{m_S, m_B\}}{b_i \geq s_i}$.
We then trade buyers $1, \ldots, i^*-1$ with sellers $1, \ldots, i^*-1$; each buyer pays $b_{i^*}$ and each seller receives $s_{i^*}$.
The welfare is $\sum_{i=1}^{i^*-1}(b_i - s_i)$.
We let $\TR(m_B, m_S)$ denote the \emph{expected} welfare obtained by trade reduction when there are $m_B$ buyers and $m_S$ sellers.

\paragraph{First Best.}
As above, let $b_1 \geq \ldots \geq b_{m_B}$ be the values of the buyers and let $s_1 \leq \ldots \leq s_{m_S}$ be the values of the sellers.
If $b_1 < s_1$ then no trade is possible.
Otherwise, let $i^* \in \max \setst{i \leq \min\{m_S, m_B\}}{b_i \geq s_i}$.
The optimal welfare is $\sum_{i=1}^{i^*} (b_i - s_i)$
We let $\OPT(m_B, m_S)$ denote the expected first best welfare when there are $m_B$ buyers and $m_S$ sellers.

Our main theorem is the following.
\begin{theorem}
    There is a constant $c \geq 1$ such that $\TR(m_B+c,m_S+c) \geq \OPT(m_B,m_S)$ for all $m_B, m_S$.
\end{theorem}
For $q \in [0,1]$, we define $b(q) \coloneqq \inf F_B^{-1}(q)$ and $s(q) \coloneqq \inf F_S^{-1}(q)$.
Observe that, by stochastic dominance, we have $b(q) \geq s(q)$ for every $q \in [0, 1]$.
Our proof is via a coupling argument.
Let $q_1, \ldots, q_{m_B+m_S+2c} \in [0,1]$ be $m_B+m_S+2c$ quantiles drawn uniformly at random.
In addition, let us sort the quantiles so that $q_1 \geq \ldots \geq q_{m_B+m_S+2c}$.
We then assign the quantiles uniformly at random amongst all the buyers and sellers;
if a buyer (resp.~seller) receives quantile $q_i$ then its value is $b(q_i)$ (resp.~$s(q_i)$).
Let us use $B_{orig}, B_{new}, S_{orig}, S_{new}$ to denote the set of \emph{indices} of the quantiles
received by the original buyers, new buyers, original sellers, and new sellers respectively.

For the analysis, let $W_{\OPT}$ be the random variable that gives the first best welfare
and let $W_{\TR}$ be the random variable that gives the welfare under trade reduction.

We split the analysis into two cases based on the ratio $m_S / m_B$
\textcolor{red}{(although the analysis is similar enough that we may be able to unify the two cases)}.

We first consider the case when $m_S \leq r \cdot m_B$ for some constant $r \leq 1/2$ to be determined.

Let $\cE_1$ be the event that all $c$ of the new sellers are in the top $2m_S+c$ quantiles.
Note that $\cE_1$ is a necessary event for the optimal allocation to have more welfare than trade reduction.
Indeed, if there is a single new seller outside the top $2m_S+c$ quantiles then there must be at least $m_S+1$
buyers in the top $2m_S + c$ quantiles and one new seller in the bottom $c$ quantiles.
At least one of the buyers in the top $2m_S+c$ quantiles must be unmathced
(either because it is an original buyer that is unmatched or it is a new buyer)
and such a buyer can be matched to the new seller that is in one of the bottom $c$ quantiles.
\begin{lemma}
    \LemmaName{cE_1}
    We have that $\expect{(W_{\OPT} - W_{\TR})\ind{\cE_1}} \leq \expect{b(q_i) - s(q_j)} \cdot \prob{\cE_1}$
    where $i \sim [m_S]$ u.a.r.~and $j \sim [m_B+m_S+2c] \setminus [m_S + 2c]$ u.a.r.
\end{lemma}
\begin{proof}
    Let $q_o(1) \geq \ldots \geq q_o(m_B+m_S)$ denote the quantiles assigned to the original buyers and sellers.
    For $k \geq 1$, let $\cF_k$ be the event that amongst the original buyers and sellers,
    exactly $k$ of the buyers received the top $m_S$ quantiles that were assigned to the original buyers and sellers.
    Thus, there are exactly $k$ sellers who received the bottom $m_B$ quantiles
    (amongst the quantiles assigned to the original buyers and sellers).
    
    Let $i_1 < \ldots < i_k \leq m_S$ denote the indices of the original quantiles assigned to the top $k$ buyers
    and $j_1 > \ldots > j_k \geq m_S + 1$ denote the indices of the original quantiles assigned to the bottom $k$ sellers.
    Note that, on the event $\cF_k$, we have $W_{\OPT} - W_{\TR} \leq b(q_o(i_k)) - s(q_o(j_k))$.
    This is because the optimal allocation matches the buyer that is assigned quantile $q_o(i_k)$ and the seller that is assigned
    quantile $q_o(j_k)$.
    Therefore, the trade removed by trade reduction has value at most $b(q_o(i_k)) - s(q_o(j_k))$.
    We thus have that
    \begin{align*}
        \expect{(W_{\OPT} - W_{\TR}) \cdot \ind{\cE_1 \wedge \cF_k}}
        & ~\leq~ \expect{(b(q_o(i_k)) - s(q_o(j_k))) \cdot \ind{\cE_1 \wedge \cF_k}} \\
        & ~=~ \expectg{(b(q_o(i_k)) - s(q_o(j_k)))}{\cE_1 \wedge \cF_k} \cdot \prob{\cE_1 \wedge \cF_k} \\
        & ~=~ \expect{(b(q_o(i_k)) - s(q_o(j_k)))} \cdot \prob{\cE_1 \wedge \cF_k} \\
        & ~\leq~ \expect{(b(q_o(i)) - s(q_o(j-2c)))} \cdot \prob{\cE_1 \wedge \cF_k} \\
        & ~\leq~ \expect{(b(q(i)) - s(q(j)))} \cdot \prob{\cE_1 \wedge \cF_k}.
    \end{align*}
    The second equality is because $i_k, j_k$ is independent of the event $\cE_1 \wedge \cF_k$.
    For $k = 0$, we have
    \begin{align*}
        0 ~=~ \expect{(W_{\OPT} - W_{\TR}) \cdot \ind{\cE_1 \wedge \cF_0}}
        & ~\leq~ \expect{(b(q(i)) - s(q(j)))} \cdot \prob{\cE_1 \wedge \cF_0},
    \end{align*}
    where the inequality is simply because the RHS is non-negative (as $q(i) < q(j)$).
    The claim now follows from summing over $k = 0, \ldots, m_S$.
\end{proof}
Next, let $\cE_2$ be the event that at least two new buyers are in the top $m_S$ quantiles
and at least two new sellers are in the bottom $m_B$ quantiles.
Clearly, on the event $\cE_2$, trade reduction with the new participants obtains more welfare than the optimal allocation
with only the original participants.
\begin{lemma}
    \LemmaName{cE_2}
    Let $i \sim [m_S]$ and $j \sim [m_B+m_S+2c] \setminus [m_S+2c]$.
    Then
    \[
        \expect{(W_{\TR} - W_{\OPT})\ind{\cE_2}}  \geq \expect{b(q_i) - s(q_j)} \cdot \prob{\cE_2}.
    \]
\end{lemma}
\begin{proof}
    Let $i_1, i_2 \sim [m_S]$ uniformly at random without replacement and $j_1, j_2 \sim [m_B+m_S+2c] \setminus [m_S+2c]$ uniformly at random without replacement.
    On the event $\cE_2$, we have that $W_{\OPT} - W_{\TR} \geq b(q(\max(i_1, i_2))) - s(q(\min(j_1, j_2)))$.
    Taking expectations and using that $b(q(\max(i_1, i_2))) \leq b(q(i_1))$ and $s(q(\min(j_1, j_2))) \geq s(q(j_1))$ proves the lemma.
\end{proof}

We also have the following simple observation.
\begin{lemma}
    \LemmaName{TR_OPT_LB}
    Let $i \sim [m_S]$ and $j \sim [m_B+m_S+2c] \setminus [m_S + 2c]$.
    Then $\expect{W_{\TR} - W_{\OPT}} \geq \expect{b(q_i) - s(q_j)} \cdot (\prob{\cE_2} - \prob{\cE_1})$.
\end{lemma}
\begin{proof}
    This follows directly from \Lemma{cE_1} and \Lemma{cE_2}.
    More specifically, let $\cE_3 = \cE_1^c \wedge \cE_2^c$.
    Then
    \begin{align*}
        \expect{W_{\TR} - W_{\OPT}}
        & ~=~ \expect{(W_{\TR} - W_{\OPT})\ind{\cE_1}} + \expect{(W_{\TR} - W_{\OPT})\ind{\cE_2}} + \expect{(W_{\TR} - W_{\OPT})\ind{\cE_3}} \\
        & ~\geq~ \expect{(W_{\TR} - W_{\OPT})\ind{\cE_1}} + \expect{(W_{\TR} - W_{\OPT})\ind{\cE_2}} \\
        & ~\geq~  \expect{b(q_i) - s(q_j)} \cdot (\prob{\cE_2} - \prob{\cE_1}),
    \end{align*}
    where the first inequality is because $W_{\TR} - W_{\OPT} \geq 0$ on the event $\cE_1^c \supset \cE_3$
    and the last inquality is \Lemma{cE_1} and \Lemma{cE_2}.
\end{proof}
From \Lemma{TR_OPT_LB}, it suffices to show that $\prob{\cE_2} \geq \prob{\cE_1}$.
\begin{lemma}
    $\prob{\cE_1} \leq \left( \frac{2m_S}{m_B+m_S+c} \right)^c$.
\end{lemma}
\begin{proof}
    Recall that $\cE_1$ is the event that all of the $c$ new sellers are in the top $2m_S + c$ quantiles.
    The probability of this happening is
    \begin{equation*}
    \begin{aligned}
        \prob{\cE_1} = \frac{\binom{2m_S + c}{c}}{\binom{m_B + m_S + 2c}{c}}
        & = \frac{(2m_S+c)!}{c!(2m_S)!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
        & = \frac{(2m_S+c) \ldots (2m_S+1)}{(m_B+m_S+2c)\ldots(m_B+m_S+c+1)} \\
        & \leq \left( \frac{2m_S}{m_B+m_S+c} \right)^c,
    \end{aligned}
    \end{equation*}
    as required.
\end{proof}

Next, we lower bound the probability of event $\cE_2$.
To do this, we define two random variables.
Let $X_B$ be the random variable counting the number of new buyers in the top $m_S$ quantiles.
Let $X_S$ be the random variable counting the number of new sellers in the bottom $m_B$ quantiles.
Then $\cE_2 = \{ X_B \geq 2 \} \wedge \{ X_S \geq 2 \}$.
Let $p_B = \frac{m_B+2c}{m_B + m_S+2c}$.
\begin{lemma}
    \LemmaName{XS_and_XB_LB}
    Suppose that $m_S \geq \max\{4, c\}$.
    Then $\prob{X_S \geq 2} \geq \prob{X_B \geq 2} \geq \frac{1}{2} \binom{c}{2} (1-p_B)^2 p_B^{c-2}$.
\end{lemma}
\begin{proof}
    The inequality $\prob{X_S \geq 2} \geq \prob{X_B \geq 2}$ should be trivial since $m_B \geq m_S$.
    Therefore, we only prove the second inequality.

    First, we have that
    \begin{align*}
        \prob{X_B = 0}
        & = \frac{\binom{m_B+2c}{c}}{\binom{m_B+m_S+2c}{c}} \\
        & = \frac{(m_B+2c)!}{(m_B+c)!c!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
        & = \frac{(m_B+2c)\ldots (m_B+c+1)}{(m_B+m_S+2c) \ldots (m_B+m_S+c+1)} \\
        & \leq p_B^c
    \end{align*}
    Next,
    \begin{align*}
        \prob{X_B = 1}
        & = \frac{m_S \cdot \binom{m_B+2c}{c-1}}{\binom{m_B+m_S+2c}{c}} \\
        & = m_S \cdot \frac{(m_B+2c)!}{(m_B+c+1)!(c-1)!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
        & = c \cdot \frac{m_S}{m_B+m_S+c+1} \cdot \frac{(m_B+2c)\ldots(m_B+c+2)}{(m_B+m_S+2c)\cdot(m_B+m_S+c+2)} \\
        & \leq c \cdot (1-p_B) \cdot p_B^{c-1} \cdot \left( 1 + \frac{c-1}{m_B+m_S+c+1} \right).
    \end{align*}
    Now, for any $p \in [0,1]$ we have that $p^c + cp^{c-1}(1-p) + \binom{c}{2} p^{c-2} (1-p)^2 \leq 1$ (LHS is truncated Binomial expansion of $1$), hence
    \begin{align*}
        \prob{X_B \geq 2}
        = 1 - \prob{X_B \leq 1}
        \geq \binom{c}{2} p_B^{c-2} \cdot (1-p_B)^2 - c\cdot(1-p_B)\cdot p_B^{c-1} \cdot \frac{c-1}{m_B+m_S+c+1}.
    \end{align*}
    We now need to verify that
    \[
        \binom{c}{2} p_B^{c-2} \cdot (1-p_B)^2 \geq 2(1-p_B) p_B^{c-1} \frac{c(c-1)}{m_B+m_S+c+1}. 
    \]
    Rearranging, this is equivalent to
    \[
        (1-p_B) \geq 4 \frac{p_B}{m_B+m_S+c+1}.
    \]
    Recall that $p_B = \frac{m_B+2c}{m_B+m_S+2c}$.
    Plugging this in and cancelling common terms gives the equivalent inequality
    \[
        m_S \geq 4 \cdot \frac{m_B+2c}{m_B+m_S+c+1}. 
    \]
    Since $m_S \geq c$, we have $4\cdot\frac{m_B+2c}{m_B+m_S+c+1} \leq 4\cdot\frac{m_B+2c}{m_B+2c} = 4 \leq m_S$ by assumption on $m_S$.
\end{proof}

\begin{lemma}
    $\prob{\cE_2} \geq \frac{1}{16} c^2(c-1)^2 (1-p_B)^4 p_B^{2c-4}$.
\end{lemma}
\begin{proof}
    \textcolor{red}{Check that $\probg{X_B \geq 2}{X_s \geq 2} \geq \prob{X_B \geq 2}$.}
    Thus, $\prob{\cE_2} = \prob{X_S \geq 2} \probg{X_B \geq 2}{X_s \geq 2} \geq \prob{X_S \geq 2}\cdot\prob{X_B \geq 2}$
    and apply \Lemma{XS_and_XB_LB}.
\end{proof}





We prove the theorem in two parts although the proofs are similar and it may be possible to merge the two parts.

\paragraph{Part 1: $m_S \leq m_B / 4$.}
Let $c \geq 1$ be a constant that we choose at the end of the proof.
First, we define two events.
\begin{itemize}
    \item \textbf{Event $\cE_1$.}
    Let $\cE_1$ be the event that all $c$ of the new sellers receive the top $2m_S+c$ quantiles.
    
    \item \textbf{Event $\cE_2$.}
    Let $\cE_2$ be the event that at least two \emph{new} buyers receive the top $m_S+c$ quantiles
    and at least two \emph{new} sellers receive the top $m_B$ quantiles.
    
    \item \textbf{Event $\cE_3$.}
    We let $\cE_3 = $
\end{itemize}

\begin{lemma}
    \LemmaName{cE_1}
    The event $\cE_1$ is \emph{necessary}
\end{lemma}

Let $\cE_1$ be the event that all $c$ of the new sellers receive 



\paragraph{General case.}
We now turn to the general case.


Here is an attempt for the general case.
First, we \emph{order} the original $m_B$ buyers and $m_S$ sellers;
we do not assign quantiles just yet.

Now let us condition on the trade size $q$ of the optimal matching amongst the original $m_B$ buyers and $m_S$ sellers.
We now add in the new buyers and sellers.
A \emph{necessary} condition for $\OPT$ to have higher value than $\TR$ is the following:
\begin{enumerate}
    \item Amongst the top $m_S$ of the original buyers and sellers, exactly $q$ are buyers;
    \item all $c$ of the new buyers that we add in is ranked strictly above the ($m_s+q$)th slot amongst the original.
\end{enumerate}
For the second item, there are $\binom{m_S + q + c}{c}$ such assignments,
whereas there are $\binom{m_B+m_S+c}{c}$ total possible assignments.


Now let us assume the general case with $m_B$ buyers and $m_S$ sellers.
The case where $m_B \approx m_S$ should be fairly straightforward by concentration.

Jotting down some quick general ideas.
\begin{itemize}
\item A necessary condition for $\OPT$ to strictly win is that at most $m_S$ sellers outside of top $m_S + c$.
If $m_S+1$ sellers outside of top $m_S+c$ then can construct a matching of size $m_S+1$ and $\TR$ gets at least as much as $\OPT$.
\item A sufficient condition for $\TR$ to do as well as $\OPT$ is that at least $2$ new buyers in top $m_S + c$ and at least $2$ sellers outside.
\end{itemize}
Are these enough?

\input{scratchpad.tex}

==> old_stuff/one_seller.tex <==
\section{Single seller}
\paragraph{Notation.}
We use $\OPT(m_B, m_S)$ to denote the optimal GFT with $m_B$ buyers and $m_S$ sellers.
Similarly, we use $\TR(m_B, m_S)$ to denote the value of GFT of trade reduction with $m_B$ buyers and $m_S$ sellers.

As a warmup, we begin with the single seller case and prove the following theorem.

\begin{theorem}
    There is a constant $c \geq 1$ such that $\TR(m + c, 1 + c) \geq \OPT(m, 1)$.
\end{theorem}

The proof uses a coupling argument.
For $q \in (0, 1)$, we get $b(q) = F_B^{-1}(q)$ and $s(q) = F_S^{-1}(q)$, where $F_B, F_S$ are the c.d.f.'s of the buyer, seller distributions.
For simplicity, we assume that $F_B, F_S$ are continuous so that their inverses are well-defined.
\chris{Figure out if there are any subtleties with non-continuous CDF.}
Let $q_1, \ldots, q_{m+1+2c}$ be $m+1+2c$ uniform quantiles from $[0,1]$;
we assume these are sorted so that $q_1 \geq \ldots \geq q_{m+1+2c}$.
We then uniformly assign these quantiles to the new and old buyers and sellers.

\begin{lemma}
    \label{lem:one_seller_necessary}
    A necessary condition for $\OPT$ to obtain strictly more GFT
    %\mingfeinote{Mingfei: It's equivalent but maybe better to stick with GFT everywhere?}
    than $\TR$ is that at most one of the top $c+1$ quantiles belong to a buyer.
    Denote this event by $\cE_1$.
    Conditioned on $\cE_1$, we have
    \[
        \expectg{\OPT - \TR}{\cE_1}
        \leq \expects{i, j}{b(q_i) - s(q_j)},
    \]
    where $i \sim [c+1]$ uniformly at random and $j \sim [m+1+2c] \setminus [c+1]$ uniformly at random.
\end{lemma}
\begin{proof}
    Suppose that at least $2$ of the top $c+1$ quantiles belong to buyers.
    Then there are also at least two sellers outside of the top $c+1$ quantiles.
    % In particular, this implies that $\TR$ has at least one trade and the GFT from this trade is at least the GFT of $\OPT$.
    This implies that $\TR$ has at least one trade. The GFT of $\TR$ is thus at least the highest value among all buyers subtracting the highest cost among sellers, which is at least the GFT of $\OPT$ since there is only 1 seller before augmentation.

    For an integer $k \geq 0$, let $\cF_k$ be the event that there are exactly $k$ buyers in the top $c+1$ quantiles.
    Note that $\cE_1 = \cF_0 \cup \cF_1$.
    Let $q_b$ be the quantile of the highest value buyer and $q_s$ be the quantile of the lowest value seller.
    Note that $b(q_b) - s(q_s)$ is an upper bound on the GFT from $\OPT$ since $q_b, q_s$ may not belong to the original buyer and/or seller.
    In other words, $\OPT - \TR \leq b(q_b) - s(q_s)$.
    Finally, let $i \sim [c+1]$ be drawn uniformly at random and let $j \sim [m+2c+1] \setminus [c+1]$ be drawn uniformly at random.
    
    On the event $\cF_0$, note that $q_b < q_i$ since $q_i$ is in the top $c+1$ quantiles but $q_b$ is not.
    Similarly, $q_s > q_j$ because $q_s$ is in the top $c+1$ quantiles but $q_j$ is not.
    Hence, $\expectg{b(q_b) - s(q_s)}{\cF_0} \leq \expect{b(q_i) - s(q_j)}$.
    Next, on the event $\cF_1$, we have exactly $1$ buyer in the top $c+1$ quantiles and so $q_b = q_i$ in distribution. Similarly, $q_s = q_j$ in distribution.
    So $\expectg{b(q_b) - s(q_s)}{\cF_1} = \expect{b(q_i) - s(q_j)}$.
    
    We conclude that $\expectg{\OPT - \TR}{\cE_1} \leq \expect{b(q_i) - s(q_j)}$.
\end{proof}

Next, we define an event which is sufficient for trade reduction with the additional buyers and sellers to have GFT at least
the optimal GFT with the original buyers and sellers.
\begin{enumerate}[itemsep=0pt, topsep=0pt]
    \item Let $\cE_{2, 1}$ be the event that at least $2$ buyers are in the top $c+1$ quantiles.
    \item Let $\cE_{2, 2}$ be the event that the top $2$ buyers are new buyers.
    % \item Let $\cE_{2, 3}$ be the event that at least $2$ sellers are outside the top $c+1$ quantiles.
    \item Let $\cE_{2, 3}$ be the event that the bottom $2$ sellers are new sellers.
\end{enumerate}

%\mingfeinote{Mingfei: Should we remove $\cE_{2,3}$ since it's always true conditioned on $\cE_{2,1}$?}
%\chris{Sounds good. I think I removed it now.}

Note that the event $\cE_{2,1}$ also implies that at least $2$ sellers are outside the top $c+1$ quantiles since there are exactly $c+1$ sellers.
Finally, let $\cE_2$ be the event that all $4$ of the above events happen, i.e.~$\cE_2 = \cap_{k=1}^3 \cE_{2, k}$.

Observe that $\cE_2$ implies that trade reduction with the augmented bidders has a GFT at least that of the optimal GFT before augmentation.
To see this, let $b$ be the highest value among all buyers and $s$ be the lowest value among all sellers.
Then, on the event $\cE_{2,1}$ trade reduction with augmentation has GFT at least $b - s$ while the optimal GFT without augmentation is upper bounded by $b - s$.
However, our goal now is to show that trade reduction with augmentation has significantly higher GFT than the optimal GFT before augmentation in the event $\cE_2$.
{To verify $\cE_2$ is sufficient condition, denote $b$ the highest value among all buyers and $s$ the lowest cost among all sellers. Then conditioned on $\cE_2$, $\TR$ has at least one trade (because of $\cE_{2,1}$) and has GFT at least $b-s$. Before augmentation, $\OPT$ has GFT at most the highest value among all original buyers subtracting the lowest cost among all original sellers, which is at most $b-s$.}
\begin{claim}
    \label{claim:one_seller_tr_lb}
    Let $q_b$ be the quantile of the top buyer and $q_s$ be the quantile of the lowest seller.
    On the event $\cE_2$, we have $\TR - \OPT \geq b(q_b) - s(q_s)$.
\end{claim}
\begin{proof}
    Let $q_{b,1} \geq q_{b, 2} \geq \ldots \geq q_{b,m+c}$ be the quantiles of the buyers and let $q_{s,1} \leq q_{s, 2} \leq \ldots \leq q_{s,c+1}$ be the quantiles of the sellers.
    If there was no trade in $\OPT$ then the claim is trivial since $q_{b,2} \geq q_{s,2}$ (because of $\cE_{2,1}$)
    so the GFT of trade reduction is at least $b(q_{b,1}) - s(q_{s,1})$.
    % so the top buyer and lowest seller trades in trade reduction. \mingfeinote{Mingfei: I think it might be better to write ``So the GFT of TR is at least $b(q_{b,1})-s(q_{s,1})$", since if there are more than one trades, the top buyer not necessary ``trades'' with the lowest seller it can trade with any seller within the opt trade size. } 
    
    Now, we assume that there was a single trade in $\OPT$.
    Let $q_{b}^{o}$ be the largest quantile of the original buyer and $q_{s}^{o}$ be the lowest quantile of the original seller.
    Note that $q_{b,3} \geq q_{b}^{o}$ and $q_{s}^{o} \geq q_{s,3}$.
    Thus, we have $b(q_{b,3}) \geq b(q_{b}^{o}) \geq s(q_{s}^{o}) \geq s(q_{s,3})$.
    The GFT of $\TR$ is thus lower bounded by $(b(q_{b,1}) - s(q_{s,1})) + (b(q_{b,2}) - s(q_{s,2}))$.
    On the other hand, the GFT of $\OPT$ is $b(q_{b}^o) - s(q_{s}^o) \leq b(q_{b,3}) - s(q_{s,3}) \leq b(q_{b,2}) - s(q_{s,2})$.
    Therefore, $\TR - \OPT \geq b(q_{b,1}) - s(q_{s,1})$ as claimed.
\end{proof}

\begin{lemma}
    $\expectg{\TR - \OPT}{\cE_2} \geq \expects{i, j}{b(q_i) - s(q_j)}$
    where $i \sim [c+1]$ uniformly at random and $j \sim [m+1+2c] \setminus [c+1]$ uniformly at random.
\end{lemma}
\begin{proof}
    Let $\cF_{k}$ be the event that there are exactly $k$ buyer quantiles in the top $c+1$ quantiles.
    Note that this implies that there are also exactly $k$ seller quantiles outside the top $c+1$ quantiles.
    Then
    \[
        \expectg{\TR - \OPT}{\cE_2}
        \geq \sum_{k} \expectg{b(q_b) - s(q_s)}{\cE_2 \cap \cF_{k}}
        \cdot \prob{\cF_{k}}.
    \]
    Note that $\cE_2 \cap \cF_{k} = \emptyset$ for $k < 2$.
    Henceforth, we assume $k \geq 2$.

    Let us condition on the event $\cE_2 \cap \cF_k$.
    Recalling the definition of $\cE_2$, observe that $\cE_2 \cap \cF_k = \cF_k \cap \cE_{2,2} \cap \cE_{2,3}$.
    Let $i_1 < i_2 < \ldots < i_k$ be the indices of the $k$ quantiles amongst the top $c+1$ quantiles that belong to buyers.
    Then $q_b \ind{\cF_k} = q(\min(i_1, \ldots, i_{k})) \ind{\cF_{k}}$ is independent of $\cE_{2,2}, \cE_{2,3}$ and so
    \[
        \expectg{b(q_b)}{\cE_2 \cap \cF_{k}}
        = \expectg{b(q_b)}{\cF_{k}}
        = \expects{i_1, \ldots, i_{k}}{\max_j b(q_{i_j})}
        \geq \expects{i}{b(q_i)}.
    \]
    In the third expression, the $i_{k_1}, \ldots, i_{k}$ are drawn uniformly from $[c+1]$ without replacement
    and in the last expression, $i$ is drawn uniformly from $[c+1]$.
    A similar argument would give that
    \[
        \expectg{s(q_s)}{\cE_2 \cap \cF_{k}}
        \leq \expects{j}{s(q_j)}
    \]
    where $j$ is drawn uniformly from $[m+2c+1] \setminus [c+1]$.
\end{proof}

\begin{lemma}
    \label{lemma:E1_prob}
    If $m \geq 1, c \geq 3$ then $\prob{\cE_1} < \frac{1}{10} \cdot \frac{\binom{c}{2}}{\binom{m+c}{2}} < \frac{1}{10}$.
\end{lemma}
\begin{proof}
    We only prove the first inequality since the second inequality is trivial.
    Recall that $\cE_1$ is the event that at most $1$ of the top $c+1$ quantiles belong to a buyer.
    Thus, $\prob{\cE_1} = \frac{1 + (m+c+1)}{\binom{m+2c+1}{c+1}}$ \mingfeinote{$\frac{1 + (m+c)(c+1)}{\binom{m+2c+1}{c+1}}$} \chris{I will fix. This should only affect constants right?}.
    So we just need to check the numeric inequality
    \[
        \frac{m+c+2}{\binom{m+2c+1}{c+1}} \cdot \frac{\binom{m+c}{2}}{\binom{c}{2}} < \frac{1}{10}. 
    \]
    Expanding and simplifying, we have
    \begin{align*}
        \frac{m+c+2}{\binom{m+2c+1}{c+1}} \cdot \frac{\binom{m+c}{2}}{\binom{c}{2}}
        & ~=~
        \frac{(m+c+2) \cdot (m+c)! \cdot (c+1)!}{(m+2c+1)!} \cdot
        \frac{(m+c)! \cdot (c-2)!}{c! \cdot (m+c-2)!} \\
        & ~=~
        \frac{(m+c+2) \cdot (m+c)! \cdot (c+1)!}{(m+2c+1)!} \cdot
        \frac{(m+c) \cdot (m+c-1)}{c \cdot (c-1)} \\
        & ~\leq~
        \frac{(m+c+2)!}{(m+2c+1)!} \cdot \frac{(c+1)!}{c\cdot(c-1)} \\
        & ~=~
        \frac{c+1}{m+2c+1} \cdot \prod_{k=1}^{c-2} \frac{k}{m+c+k+2} \\
        & ~\leq~ \frac{c+1}{m+2c+1} \cdot \frac{1}{m+c+3} \\
        & ~<~ \frac{1}{10},
    \end{align*}
    where in the last inequality we used that the second-last line is decreasing in $c$ and $m$ so we plugged in $c = 3$ and $m = 1$.
\end{proof}

\begin{lemma}
    \label{lemma:E2_prob}
    $\prob{\cE_2} = \left(1 - \prob{\cE_1} \right) \cdot \frac{\binom{c}{2}}{\binom{m+c}{2}} \cdot \frac{c-1}{c+1}$.
\end{lemma}
\begin{proof}
    We use the fact that $\cE_{2,1}, \cE_{2,2}, \cE_{2,3}$ are all independent events.
    Note that $\cE_{2,1}$ is the complement of $\cE_{1}$ so $\prob{\cE_{2,1}} = 1 - \prob{\cE_1}$.
    Next, $\prob{\cE_{2,2}} = \frac{\binom{c}{2}}{\binom{m+c}{2}}$ because there are $\binom{c}{2}$ to choose the top $2$ buyer quantiles such that both belong to new buyers.
    Finally, $\prob{\cE_{2,3}} = \frac{c-1}{c+1}$ because there is only one old seller quantile and $\frac{c-1}{c+1}$ is the probability that it is \emph{not} in the top $2$ quantiles.
    The lemma follows by taking the product.
\end{proof}

\begin{lemma}
    If $m \geq 1, c \geq 3$ then $\prob{\cE_1} < \prob{\cE_2}$.
\end{lemma}
\begin{proof}
    By Lemma~\ref{lemma:E1_prob}, $\prob{\cE_1} < \frac{1}{10} \cdot \frac{\binom{c}{2}}{\binom{m+c}{2}}$.
    By Lemma~\ref{lemma:E2_prob}, $\prob{\cE_2} > \frac{9}{10} \cdot \frac{\binom{c}{2}}{\binom{m+c}{2}} \cdot \frac{1}{4} > \frac{2}{10} \cdot \frac{\binom{c}{2}}{\binom{m+c}{2}}$.
    We conclude that $\prob{\cE_2} > \prob{\cE_1}$.
\end{proof}

==> old_stuff/one_seller_with_fix.tex <==
\paragraph{One seller with fix.}
\begin{lemma}
    % \label{lem:one_seller_necessary}
    A necessary condition for $\OPT$ to obtain strictly more welfare than $\TR$ is that exactly one of the top $c+2$ quantiles belong to a buyer.
    Denote this event by $\cE_1$.
    Conditioned on $\cE_1$, we have
    \[
        \expectg{\OPT - \TR}{\cE_1}
        \leq \expects{i, j}{b(q_i) - s(q_j)},
    \]
    where $i \sim [c+2]$ uniformly at random and $j \sim [m+1+2c] \setminus [c+2]$ uniformly at random.
\end{lemma}
\begin{proof}
    Suppose that there is \emph{not} exactly one buyer in the top $c+2$ quantiles.
    Since there are at most $c+1$ sellers, there cannot be $0$ buyers in the top $c+2$ quantiles.
    Hence, there are at least two buyers in the top $c+2$ quantiles.
    Consequently, there must be at least two sellers outside of the top $c+1$ quantiles. \mingfeinote{Mingfei: Replace the previous sentence by ``Thus there must be some seller outside of the top $c+2$ quantiles."?}
    This implies that $\TR$ must have at least one trade and this trade has value at least that of $\OPT$.
    \mingfeinote{Mingfei: In this case if the two buyers are (c+1)-th and (c+2)-th and the top c quantiles are all on the seller side, $\TR$ doesn't have a trade.}
    \chris{Thanks! Good catch. Actually, I think the $c+2$ should be $c+1$ and that the ``exactly $1$ buyer'' should be ``at most $1$ buyer''. Now if there are $2$ buyers in the top $c+1$ quantiles there must be two sellers outside so should fix your counter-example. I don't think the stuff below depends on the $c+2$ (as opposed to $c+1$) but we can discuss later.} \mingfeinote{I agree with the ``at most 1 buyer out of $c+1$". Thanks!}

    Now let us condition on $\cE_1$.
    Then there is exactly one buyer in the top $c+2$ quantiles and its quantile rank is uniformly random amongst the top $c+2$.
    Similarly, there is exactly one seller outside the top $c+2$ quantiles and its quantile rank is uniformly random amongst the bottom
    $m+c-1$ quantiles.
    So the value of the highest value match is $\expects{i, j}{b(q_i) - s(q_j)}$ where $i \sim [c+2]$ u.a.r.~and $j \sim [m+1+2c] \setminus [c+2]$ u.a.r.
    Finally, observe that the value of the highest value match is an upper bound on $\OPT$.
\end{proof}

Consider the event $\cE_2$ that satisfies the following condition:
\begin{itemize}
    \item at least $2$ buyers are in the top $c+2$ quantiles;
    \item the top $2$ buyers are new;
    \item at least $2$ sellers are outside the top $c+2$ quantiles;
    \item the bottom $2$ sellers are new.
\end{itemize}

\begin{claim}
    % \label{claim:one_seller_tr_lb}
    Condition on $\cE_2$.
    Let $q_b$ be the quantile of the top buyer and $q_s$ be the quantile of the lowest seller.
    Then $\TR - \OPT \geq b(q_b) - s(q_s)$.
\end{claim}
\begin{proof}
    Let $q_{b,1} > q_{b, 2} > \ldots$ be the quantiles of the buyers and let $q_{s, 1} < q_{s, 2} < \ldots$ be the quantiles of the sellers.
    If there was no trade in $\OPT$ then the claim is trivial since $q_{b,2} > q_{s,2}$ so the top buyer and lowest seller trades in trade reduction. 
    
    Now, we assume that there was a single trade in $\OPT$.
    Let $q_{b}^{o}$ be the quantile of the original buyer and $q_{s}^{o}$ be the quantile of the original seller.
    Note that $q_{b,3} \geq q_{b}^{o}$ and $q_{s}^{o} \geq q_{s,3}$.
    Thus, we have $b(q_{b,3}) \geq b(q_{b}^{o}) \geq s(q_{s}^{o}) \geq s(q_{s,3})$.
    The revenue $\TR$ is thus lower bounded by $(b(q_{b,1}) - s(q_{s,1})) + (b(q_{b,2}) - s(q_{s,2}))$.
    On the other hand, the revenue of $\OPT$ is $b(q_{b}^o) - s(q_{s}^o) \leq b(q_{b,3}) - s(q_{s,3}) \leq b(q_{b,2}) - s(q_{s,2})$.
    Therefore, $\TR - \OPT \geq b(q_{b,1}) - s(q_{s,1})$ as claimed.
\end{proof}

\begin{lemma}
    $\expectg{\TR - \OPT}{\cE_2} \geq \expects{i, j}{b(q_i) - s(q_j)}$
    where $i \sim [c+2]$ uniformly at random and $j \sim [m+1+2c] \setminus [c+2]$ uniformly at random.
\end{lemma}
\begin{proof}
    Let $\cF_{b, k}$ be the event that there are exactly $k$ buyer quantiles in the top $c+2$ quantiles and let $\cF_{s,k}$ be the event that there are exactly $k$ seller quantiles outside the top $c+2$ quantiles.
    Then
    \[
        \expectg{\TR - \OPT}{\cE_2}
        \geq \sum_{k_b, k_s} \expectg{b(q_b) - s(q_s)}{\cE_2 \wedge \cF_{b, k_b} \wedge \cF_{s, k_s}}
        \cdot \prob{\cF_{b, k_b} \wedge \cF_{s, k_s}}.
    \]
    Note that $\cE_2 \wedge \cF_{b, k_b} \wedge \cF_{s, k_s} = \emptyset$ for $k_b < 2$ or $k_s < 2$.
    Henceforth, we assume that $k_b \geq 2$ and $k_s \geq 2$.
    
    Let us condition on the event $\cE_2 \wedge \cF_{b, k_b} \wedge \cF_{s, k_s}$.
    \textcolor{red}{(Check!)} Conditioned on the event $\cF_{b, k_b}$, $q_b$ is independent of $\cE_2 \wedge \cF_{s, k_s}$ and thus
    \[
        \expectg{b(q_b)}{\cE_2 \wedge \cF_{b, k_b} \wedge \cF_{s, k_s}}
        = \expectg{b(q_b)}{\cF_{b, k_b}}
        = \expects{i_1, \ldots, i_{k_b}}{\max_j b(q_{i_j})}
        \geq \expects{i}{b(q_i)}.
    \]
    In the third expression, the $i_{k_1}, \ldots, i_{k_b}$ are drawn uniformly from $[c+2]$ without replacement
    and in the last expression, $i$ is drawn uniformly from $[c+2]$.
    A similar argument would give that
    \[
        \expectg{s(q_s)}{\cE_2 \wedge \cF_{b, k_b} \wedge \cF_{s, k_s}}
        \leq \expects{j}{s(q_j)}
    \]
    where $j$ is drawn uniformly from $[m+2c+1] \setminus [c+2]$.
\end{proof}

Next, we give estimates on $\prob{\cE_1}$ and $\prob{\cE_2}$.

\paragraph{Estimate on $\prob{\cE_1}$.}
Recall that $\cE_1$ is the event that exactly one of the $c+2$ quantiles is a buyer.
Thus, we can choose one of the top $c+2$ quantiles and one of the buyers for $(c+2) \cdot (m+c)$ choices.
For the rest of the $c+1$ quantiles in the top $c+1$, we randomly permute for $(c+1)!$ choices and also permute the $[m+2c+1] \setminus [c+2]$ remaining quantiles for the buyers for $(m+c-1)!$.
Total is $(m+2c+1)!$ permutations.
So
\[
    \prob{\cE_1} = \frac{(c+2)!(m+c)!}{(m+2c+1)!} = O\left( m^{-(c+1)} \right),
\]
where the $O(\cdot)$ is hiding dependence on $c$.

\paragraph{Estimate on $\prob{\cE_2}$.}
Recall the event $\cE_2$ that satisfies the following condition:
\begin{itemize}
    \item at least $2$ buyers are in the top $c+2$ quantiles;
    \item the top $2$ buyers are new;
    \item at least $2$ sellers are outside the top $c+2$ quantiles;
    \item the bottom $2$ sellers are new.
\end{itemize}
We pick such an assignment of quantiles to buyers as follows.
\begin{enumerate}
    \item from the top $c+2$ quantiles, pick $2$ to be buyers ($\binom{c+2}{2}$ choices);
    \item from the bottom $m+c-1$ quantiles, pick $2$ be sellers ($\binom{m+c-1}{2}$ choices);
    \item from the remaining $m+2c-3$ quantiles, pick $m+c-2$ to be buyers ($\binom{m+2c-3}{m+c-2}$ choices);
    \item permute the buyers; $c \cdot (c-1)$ choices for the first two slots and $(m+c-2)!$ choices for the remaining $m+c-2$ slots
    \item permute the sellers; $c \cdot (c-1)$ choices for the last two slots and $(c-1)!$ choices for the remaining $c-1$ slots.
\end{enumerate}
Total is $(m+2c+1)!$ permutations.
Very roughly, we get $\prob{\cE_2} \sim m^{-2}$ so may be much larger than $\prob{\cE_1}$.

==> old_stuff/scratchpad.tex <==
\paragraph{Scratchpad.}
Suppose there are $m_B$ buyers and $m_S$ sellers, originally.
Throughout, we assume $m_B \geq m_S$ (otherwise, we could probably make some reduction like the other paper does).
\textbf{For this first part, we must assume $m_S \leq m_B / 2$ (or something like that, not sure about the constant yet).}
A necessary condition for $\OPT$ to perform better than $\TR$ is for all $c$ of the new sellers to be in the top $2m_S + c$ quantiles.
If there is even a single seller outside the top $2m_S + c$ quantiles then there must be at least $m_S + 1$ buyers in the top $2m_S + c$ quantiles.
Thus, there is at least one buyer that was not originally matched (may be either new or original).
And so $\TR$ does at least as well as $\OPT$.
\chris{Not correct. Here is counter-example. First $c-1$ belong to new sellers. Next $m_S-1$ belong to original new sellers. Followed by an original buyer $(B)$ and then an original seller $(S)$. Remaining buyers (original and new) follow and then the final new seller $(S')$. In OPT, $B$ trades with $S$ and that could be the only trade. With the new buyers and sellers, $B$ trades with $S'$ and that is the optimal GFT. TR has no trades.}

On the other hand, a sufficient condition for $\TR$ to do at least as well as $\OPT$ is if at least $2$ new buyers are in the top $m_S+c$ quantiles and at least $2$ new sellers are in the bottom $m_B$ quantiles.

Let $\cE_1$ be the event that all $c$ of the new sellers are in the top $2m_S + c$ quantiles.
Let us further refine this event.
For $k \in \{0, 1, \ldots, m_s\}$, let $\cF_k$ be the event that exactly $k$ original buyers are in the original top $m_S$ quantiles.
This implies that there are exactly $k$ original sellers in the original bottom $m_B$ quantiles.
Let $q_o(1) \geq \ldots \geq q_o(m_B + m_S)$ be the quantiles for the original buyers and sellers
(obtained by picking $m_B + m_S$ quantiles out of the $m_B + m_S + 2c$ quantiles uniformly at random).
Then, for $k \geq 1$, we have
\begin{align*}
    \expect{(\OPT - \TR) \ind{\cE_1 \wedge \cF_k}}
    & \leq \expect{(b(q_{o}(\max\{i_1, \ldots, i_k\})) - s(q_{o}(\min\{j_1, \ldots, j_k\}))) \cdot \ind{\cE_1 \wedge \cF_k}} \\
    & = \expectg{b(q_{o}(\max\{i_1, \ldots, i_k\})) - s(q_{o}(\min\{j_1, \ldots, j_k\}))}{\cE_1 \wedge \cF_k} \cdot \prob{\cF_k \wedge \cE_1} \\
    & \leq \expectg{b(q_{o}(i)) - s(q_{o}(j))}{\cE_1 \wedge \cF_k} \cdot \prob{\cE_1 \wedge \cF_k} \\
    & \leq \expectg{b(q(i)) - s(q(j))}{\cE_1 \wedge \cF_k} \cdot \prob{\cE_1 \wedge \cF_k} \\
    & = \expect{b(q(i)) - s(q(j))} \cdot \prob{\cE_1 \wedge \cF_k}.
\end{align*}
In the first line, $i_1, \ldots, i_k$ are $k$ uniformly random indices from $[m_S]$ drawn without replacement
and $j_1, \ldots, j_k$ are $k$ uniformly random indieces from $[m_B + m_S] \setminus [m_S]$ drawn without replacement.
In the third line, $i$ is drawn from $[m_S]$ uniformly at random and $j$ is drawn from $[m_B + m_S] \setminus [m_S]$ uniformly at random.
It is clearly an upper bound because a uniformly random draw will have higher (resp.~lower) rank than the max (resp.~min) of $k$ uniformly random draws.
In the fourth line, $i$ is again uniform on $[m_S]$ but $j$ is uniform on $[m_B + m_S + 2c] \setminus [m_S + 2c]$ (i.e.~the bottom $m_B$ quantiles).
The inequality is because the quantile for the buyer can only go up and the quantile for the seller can only go down when we switch to the original.
The last equality is because the term $b(q(i)) - s(q(j))$ is now independent of $\cE_1 \wedge \cF_k$.
For $k = 0$, we can use that the RHS of the first line is an upper bound on $\OPT - \TR$.

Summing over all $k$, we have that
\begin{equation}
    \expect{(\OPT - \TR) \ind{\cE_1}} \leq \expect{b(q(i)) - s(q(j))} \cdot \prob{\cE_1},
\end{equation}
where $i$ is in top $m_S$ quantiles u.a.r.~and $j$ is in bottom $m_B$ quantiles u.a.r.

Now let $\cE_2$ be the event that at least two new buyers are in the top $m_S$ quantiles and at least two new sellers are in the bottom $m_B$ quantiles.
Conditioned on $\cE_2$, we have that
\begin{equation}
    \expect{(\OPT - TR) \ind{\cE_2}} \geq \expect{b(q(i)) - s(q(j))} \cdot \prob{\cE_2}
\end{equation}
Suffice to find when $\prob{\cE_2} \geq \prob{\cE_1}$.

Look at $\cE_1$ first.
We require all new $c$ sellers to be in the top $2m_S + c$.
Probability of this happening is
\begin{align*}
    \prob{\cE_1} = \frac{\binom{2m_S + c}{c}}{\binom{m_B + m_S + 2c}{c}}
    & = \frac{(2m_S+c)!}{c!(2m_S)!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
    & = \frac{(2m_S+c) \ldots (2m_S+1)}{(m_B+m_S+2c)\ldots(m_B+m_S+c+1)} \\
    & \leq \left( \frac{2m_S}{m_B+m_S} \right)^c
\end{align*}

Now let us look at $\cE_2$.
Let $X_B$ be the random variable counting the number of buyers in the top $m_S$ quantiles.
Let $X_S$ be the random variable counting the number of sellers in the bottom $m_B$ quantiles.
Then $\cE_2 = \{ X_B \geq 2 \} \wedge \{ X_S \geq 2 \}$.

Let $p_B = \frac{m_B+2c}{m_B + m_S+2c}$.
\begin{lemma}
    Suppose that $m_S \geq \max\{4, c\}$.
    Then $\prob{X_B \geq 2} \geq \frac{1}{2} \binom{c}{2} (1-p_B)^2 p_B^{c-2}$.
\end{lemma}
\begin{proof}
    First, we have that
    \begin{align*}
        \prob{X_B = 0}
        & = \frac{\binom{m_B+2c}{c}}{\binom{m_B+m_S+2c}{c}} \\
        & = \frac{(m_B+2c)!}{(m_B+c)!c!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
        & = \frac{(m_B+2c)\ldots (m_B+c+1)}{(m_B+m_S+2c) \ldots (m_B+m_S+c+1)} \\
        & \leq p_B^c
    \end{align*}
    Next,
    \begin{align*}
        \prob{X_B = 1}
        & = \frac{m_S \cdot \binom{m_B+2c}{c-1}}{\binom{m_B+m_S+2c}{c}} \\
        & = m_S \cdot \frac{(m_B+2c)!}{(m_B+c+1)!(c-1)!} \cdot \frac{c!(m_B+m_S+c)!}{(m_B+m_S+2c)!} \\
        & = c \cdot \frac{m_S}{m_B+m_S+c+1} \cdot \frac{(m_B+2c)\ldots(m_B+c+2)}{(m_B+m_S+2c)\cdot(m_B+m_S+c+2)} \\
        & \leq c \cdot (1-p_B) \cdot p_B^{c-1} \cdot \left( 1 + \frac{c-1}{m_B+m_S+c+1} \right).
    \end{align*}
    Now, for any $p \in [0,1]$ we have that $p^c + cp^{c-1}(1-p) + \binom{c}{2} p^{c-2} (1-p)^2 \leq 1$ (LHS is truncated Binomial expansion of $1$), hence
    \begin{align*}
        \prob{X_B \geq 2}
        = 1 - \prob{X_B \leq 1}
        \geq \binom{c}{2} p_B^{c-2} \cdot (1-p_B)^2 - c\cdot(1-p_B)\cdot p_B^{c-1} \cdot \frac{c-1}{m_B+m_S+c+1}.
    \end{align*}
    We now need to verify that
    \[
        \binom{c}{2} p_B^{c-2} \cdot (1-p_B)^2 \geq 2(1-p_B) p_B^{c-1} \frac{c(c-1)}{m_B+m_S+c+1}. 
    \]
    Rearranging, this is equivalent to
    \[
        (1-p_B) \geq 4 \frac{p_B}{m_B+m_S+c+1}.
    \]
    Recall that $p_B = \frac{m_B+2c}{m_B+m_S+2c}$.
    Plugging this in and cancelling common terms gives the equivalent inequality
    \[
        m_S \geq 4 \cdot \frac{m_B+2c}{m_B+m_S+c+1}. 
    \]
    Since $m_S \geq c$, we have $4\cdot\frac{m_B+2c}{m_B+m_S+c+1} \leq 4\cdot\frac{m_B+2c}{m_B+2c} = 4 \leq m_S$ by assumption on $m_S$.
\end{proof}
Observe that we have $\prob{X_S \geq 2} \geq \prob{X_B \geq 2}$ because $m_B \geq m_S$.
Note that we also have $\probg{X_B \geq 2}{X_S \geq 2} \geq \prob{X_B \geq 2}$ \textcolor{red}{(prove, but simple)}.
Thus, $\prob{\cE_2} \geq \frac{1}{16} c^2(c-1)^2 (1-p_B)^4 p_B^{2c-4}$.

The above analysis was assuming $m_S \leq m_B / 2$ or so.
We now consider the case where $m_S \geq m_B / 10$.
In this case, the events we consider are of the form $\cE_1$ where at most $1$ new buyers are in the top $m_S / 100$ \textbf{OR} at most $1$ new sellers are in the bottom $m_S / 100$.
$\cE_2$ will be the complement, i.e.~at least $2$ new buyers are in the top $m_S / 100$ \textbf{AND} at least 2 new buyers in the top $m_S / 100$ \textbf{AND} at least $2$ new sellers in the bottom $m_S / 100$.
Since $m_S = \Omega(m_B)$, these are very high probability events

==> r_dominance.tex <==
\section{A Parameterized Upper Bound for General Distributions via Dominance}
\begin{definition}[$(r,p)$-stochastic dominance]
We say that $F_B$ $(r,p)$-stochastically dominates $F_S$ if the following two statements hold.
\begin{enumerate}[itemsep=0pt, topsep=0pt]
    \item Let $M = \inf\{x\,:\, \probs{X \sim F_B}{X > x} > 0 \}$. Then $\probs{X \sim F_S}{X \geq M} \leq p$.
    \item For $v \leq M$, define $F_S'(v) = F_S(v) / F_S(M)$ for $v \in [0, M]$ and $F_S'(v) = 0$ for $v \notin [0, M]$. Then $1 - F_B(v) \geq r \cdot (1 - F_S'(v))$.
\end{enumerate}
\end{definition}
\begin{remark}
    Note that $F_B$ first-order stochastically dominates $F_S$ if and only if $F_B$ $(1, 1)$-stochastically dominates $F_S$.
\end{remark}

For now, we focus on the case of $(r, 1)$-stochastic dominance and then discuss how to extend to $(r, p)$-stochastic dominance for arbitrary $p \in (0, 1]$.
For convenience, we refer to $(r, 1)$-stochastic dominance as $r$-stochastic dominance when it is clear from context that $p = 1$.

% In this section, we define $b(q) = \inf\{ x\,:\, \probs{X \sim F_B}{X \leq x} \geq 1 - q\}$ and similarly for $s(q)$.
In this section, we define $b(q) = F_{B}^{-1}(1-q)$ and $s(q) = F_{S}^{-1}(1-q)$.
\chris{We should update the $r$ overlap case for this.}
\begin{claim}
    \label{claim:r_stochastic_quantiles}
    If $F_B$ $r$-stochastically dominates $F_S$ then
    for all $q \leq r$, we have $b(q) \geq s(q/r)$.
\end{claim}
\begin{proof}
    Let $x$ be such that $\probs{X \sim F_B}{X \leq x} \geq 1 - q$.
    This is equivalent to $1 - F_B(x) \leq q$.
    Since $F_B$ $r$-stochasically dominates $F_S$, we have that $1 - F_S(x) \leq (1 - F_B(x)) / r \leq q/r$.
    Thus, $s(q/r) \leq x$.
    Since this is true for $x$ satisfying $\probs{X \sim F_B}{X \leq x} \geq 1 - q$, we conclude that $s(q/r) \leq b(q)$.
\end{proof}

% \textcolor{red}{(Chris: increased the constant $10$ to $100$. Below calculations need to be modified)}
Define the intervals
\[
    I_1 = \left[0, \frac{nr}{100m}\right), I_2 = \left[\frac{nr}{100m}, \frac{2nr}{100m}\right), J_1 = \left(1 - \frac{nr}{100m}, 1\right], J_2 = \left(1 - \frac{2nr}{100m}, 1 - \frac{nr}{100m} \right].
\]
Define the event
\begin{align*}
    \cE_3 = \{ \Bq \,:\,
    & |I_{\leq 2} \cap \Bold| \leq nr/2, |[n / 50m, 1] \cap \Sold| \geq nr/2, \\
    & |J_{\leq 2} \cap \Sold| \leq mr / 10, |[0, r - nr^2 / 50m] \cap \Bold| \geq mr / 10
    \}.
\end{align*}
\begin{claim}
    \label{claim:r_dominance_E3_matched}
    Condition on event $\cE_3$.
    In the original first-best matching, every original buyer in $I_{\leq 2}$ is matched and every original seller in $J_{\leq 2}$ is matched.
\end{claim}
\begin{proof}
    Let $k = |I_{\leq 2} \cap \Bold| \leq nr/2$ be the number of original buyers in $I_{\leq 2}$. By definition, we have $\qbo(k) \leq nr / 50m$. On the event $\cE_3$, we have $|[n/5m, 1] \cap \Sold| \geq nr/2$ and thus, $\qso(k) \geq n / 5m$. Thus, by Claim~\ref{claim:r_stochastic_quantiles} we have
    \[
        \oldb_k = b(\qbo(k)) \geq b(nr/50m) \geq s(n/50m) \geq s(\qso(k)) = \olds_k.
    \]
    Thus, the top $k$ buyers are matched.

    The argument for the seller is completely analogous.
    Let $k = |J_{\leq 2} \cap \Sold| \leq mr/10$ be the number of original buyers in $J_{\leq 2}$.
    By definition, we have $\qso(k) \geq 1-nr/50m$.
    On the event $\cE_3$, we have $|[0, r - nr^2/50m] \cap \Bold| \geq mr/10$ and thus $\qbo(k) \leq r - nr^2 / 50m$.
    Again, by Claim~\ref{claim:r_stochastic_quantiles} we have
    \[
        \oldb_k = b(\qbo(k)) \geq b(r - nr^2 / 50m) \geq s(1 - nr/50m) \geq s(\qso(k)) = \olds_k.
    \]
    Thus, the bottom $k$ sellers are matched.
\end{proof}

\begin{lemma}
    We have that
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\neg \cE_3}} \leq e^{-\Omega(nr)} \cdot
        \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
% \textcolor{red}{I don't think the above is sufficient.}
\begin{proof}
    Let $\cF_1 = \{|I_{\leq 2} \cap \Bold| > nr / 2\}$, $\cF_2 = \{|[n/5m, 1] \cap \Sold| < nr/2\}$, $\cF_3 = \{|J_{\leq 2} \cap \Sold| > mr / 10\}$, and $\cF_4 = \{|[0, r - nr^2 / 2m] \cap \Bold| < mr / 10\}$.
    Note that $\neg \cE_3 = \cup_{i \in [4]} \cF_i$.

    In the proof, we use the following trivial observation.
    Let $\qb'(i) = \min\{\qbo(i), nr / 5m\}$ and $\qs'(j) = \max\{\qso(j), 1 - nr / 5m\}$.
    A trivial bound is that
    \begin{align*}
        \OPT(\Bq) - \STR(\Bq)
        & \leq \left(\max_{i \in [m]} b(\qbo(i)) - \min_{j \in [n]} s(\qso(j)) \right)_+ \\
        & \leq \max_{i \in [m]} b(\qb'(i)) - \min_{j \in [n]} s(\qs'(j)),
    \end{align*}
    where the last inequality uses \Cref{claim:r_dominance_E3_matched}.
    \begin{claim}
        We have that
        \[
            \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\cF_1}} \leq O(nr) e^{-\Omega(nr)} \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
        \]
    \end{claim}
    \begin{proof}
        First, we bound $\expect{\max_{i \in [m]} b(\qb'(i)) \cdot \ind{\cF_1}}$.
        We have that
        \[
            \expectg{\max_{i \in [m]} b(\qb'(i))}{|I_{\leq 2} \cap \Bold| = k}
            \leq k \cdot \expects{\qb \sim I_1}{b(\qb)}.
        \]
        Observe that $\expect{|I_{\leq 2} \cap \Bold|} = nr / 5$.
        Thus, using \Cref{lemma:chernoff}, we have
        \begin{align*}
            \expect{\max_{i \in [m]} b(\qb'(i)) \cdot \ind{\cF}}
            & \leq \expects{\qb \sim I_1}{b(\qb)} \cdot \sum_{k > nr/2} k \cdot \prob{|I_{\leq 2} \cap \Bold| \geq k} \\
            & \leq \expects{\qb \sim I_1}{b(\qb)} \cdot \sum_{k > nr/2} k \cdot \exp\left( (5k/nr-1)nr / 15 \right) \\
            & \leq \expects{\qb \sim I_1}{b(\qb)} \cdot \sum_{k > nr/2} k \cdot \exp\left( -k/5 \right) \\
            & \leq \expects{\qb \sim I_1}{b(\qb)} \cdot \int_{nr/2 - 1}^{\infty} x e^{-x/5} \, \dd x \\
            & \leq \expects{\qb \sim I_1}{b(\qb)} \cdot \int_{nr/4}^{\infty} x e^{-x/5} \, \dd x \\
            & = 25 e^{-nr/20} (nr / 20 + 1) \leq 3nr \cdot e^{-nr/20},
        \end{align*}
        where the third, fifth, and final inequalities use that $n \geq 20 / r$. \textcolor{red}{(Chris: explain why the third uses the inequality.)}

        Next, note that $-\min_{j \in [n]} s(\qs'(j))$ is independent of $\cF_1$.
        Some calculations give
        \begin{align*}
            \expect{-\min_{j \in [n]} s(\qs'(j))}
            & = \sum_{k=0}^n \expectg{-\min_{j \in [n]} s(\qs'(j))}{|J_{\leq 1} \cap \Sold| = k} \\
            & \geq \sum_{k=0}^n -\max(1, k) \expects{\qs \sim J_1}{s(\qs)} \prob{|J_{\leq 1} \cap \Sold| = k} \\
            & \geq -\expects{\qs \sim J_1}{s(\qs)} \cdot \left( \frac{n^2 r}{m} + \sum_{k > n^2r / m} k \prob{|J_{\leq 1} \cap \Sold| \geq k} \right) \\
            & \geq -\expects{\qs \sim J_1}{s(\qs)} \cdot \left( \frac{n^2 r}{m} + \sum_{k > n^2r / m} k \exp(-(k - n^2 r / 10m) / 3)\right) \\
            & \geq -\expects{\qs \sim J_1}{s(\qs)} \cdot \left( \frac{n^2 r}{m} + \sum_{k > n^2r / m} k \exp(-k / 10)\right).
        \end{align*}
        For the final summation, we have \textcolor{red}{(Chris: the 10 is so that we are in the range where the integral is actually an upper bound.)}
        \begin{align*}
            \sum_{k > n^2r / m} k \exp(-k/10)
            & \leq 10 + \frac{n^2r}{m} \exp(-n^2 r / 10m) + \int_{n^2r / m}^{\infty} x e^{-x/10} \, \dd x \\
            & \leq 10 + \frac{n^2r}{m} \exp(-n^2 r / 10m) + 100\exp(-n^2 r / 10m)(n^2r / 10 m + 1) \\
            & \leq 10 + nr + 100(nr/10 + 1) \leq 22nr,
        \end{align*}
        with the last equality using $n \geq 10 / r$.
        We thus have that
        \[
            \expect{-\min_{j \in [n]} s(\qs'(j))} \geq -23nr \cdot \expects{\qs \sim J_1}{s(\qs)}
        \]
        and so since $\prob{\cF_1} \leq \exp(-nr/10)$ by a Chernoff bound, we have
        \[
            \expect{-\min_{j \in [n]} s(\qs'(j)) \cdot \ind{\cF}} \geq -23nr \cdot \expects{\qs \sim J_1}{s(\qs)} \cdot \exp(-nr / 10).
        \]
        We conclude that
        \[
            \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\cF_1}}
            \leq 23nr e^{-nr/20} \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}. \qedhere
        \]
    \end{proof}
    \begin{claim}
        We have that
        \[
            \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\cF_2}} \leq O(nr) e^{-\Omega(n)} \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
        \]
    \end{claim}
    \begin{proof}
        A similar argument as above would show that $\expect{\max_{i \in [m]} b(\qb'(i))} \leq O(nr) \cdot \expects{\qb \sim I_1}{b(\qb)}$.
        We also have a trivial bound of $\expectg{-\min_{j \in [n]} s(\qs'(j))}{\cF_2} \geq -nr \cdot \expects{\qs \sim J_1}{s(\qs)}$.
        In addition, a standard Chernoff bound gives $\prob{\cF_2} \leq e^{-\Omega(n)}$.
    \end{proof}
    \begin{claim}
        We have that
        \[
            \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\cF_3}} \leq O(mr) \cdot \exp(-\Omega(mr)) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
        \]
    \end{claim}
    \begin{proof}
        First, observe that $\expect{|J_{\leq 2} \cap \Sold|} = n^2r/5m \leq m / 50$ so $\prob{\cF_3} \leq \exp(-\Omega(m))$.
        By the same calculations from above, we have that $\expect{\max_{i \in [m]} b(\qb'(i))} \leq O(nr) \cdot \expect{\qb \sim I_1}{b(\qb)}$.
        Thus, we have $\expect{\max_{j \in [m]} b(\qb'(i)) \cdot \ind{\cF_3}} \leq O(nr) e^{-\Omega(m)} \cdot \expect{\qb \sim I_1}{b(\qb)}$.

        Next, we have
        \begin{align*}
            \expect{-\min_{j \in [n]} s(\qs'(j)) \cdot \ind{\cF_3}}
            & \geq \sum_{k > mr / 10} \expectg{-\min_{j \in [m]} s(\qs'(j))}{\ind{|J_{\leq 2} \cap \Sold| = k}} \prob{|J_{\leq 2} \cap \Sold| \geq k} \\
            & \geq \sum_{k > mr/10} -k \expects{\qs \sim J_1}{s(\qs)} \prob{|J_{\leq 2} \cap \Sold| \geq k} \\
            & \geq \sum_{k > mr / 10} -k \expects{\qs \sim J_1}{s(\qs)} \exp\left( -\Omega(k) \right) \\
            & = O(mr) \exp(-\Omega(mr)).
        \end{align*}
    \end{proof}
    \begin{claim}
        We have that
        \[
            \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\cF_4}} \leq O(mr) \cdot \exp(-\Omega(mr)) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
        \]
    \end{claim}
    \begin{proof}
        Note that $\expectg{\max_{i \in [m]} b(\qb'(i))}{\cF_4} \leq \frac{mr}{10} \expects{\qb \sim I_1}{b(\qb)}$.
        Also, since $[0, r/2] \subseteq [0, r - nr^2 /2m]$, we have that $\expect{|[0, r - nr^2/2m] \cap \Bold|} \geq mr / 2$.
        By a standard Chernoff bound, we have $\prob{\cF_4} \leq \exp(-\Omega(mr))$.

        Next, we have $\expect{-\min_{j \in [n]} s(\qs'(j))} \geq - O(nr) \expects{\qs \sim J_1}{s(\qs)}$ as calculated above.
        The claim follows.
    \end{proof}
    Combining the four claims above gives the lemma.
\end{proof}

\paragraph{The good event $\cE_1$.}
We define $\cE_1$ as
\[
    \cE_1 = \{
        \Bq \,:\, |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_1 \cap \Snew| \geq 2, |J_2 \cap \Sold| \geq 1
    \}.
\]
\begin{lemma}
    \label{lemma:r_dominance_good}
    For any $\Bq \in \cE_1 \cap \cE_3$, we have $\STR(\Bq) \geq \OPT(\Bq)$.
    Moreover, we have
    \[
        \expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
    Let $T$ be the number of trades in the original first-best matching.
    First, we prove that when $\cE_1 \cap \cE_3$ happens, there are at least $T + 2$ trades in the augmented first-best matching.
    \begin{claim}
        Recall that $\qbn(2)$ is the quantile of the second-highest new buyer and $\qsn(2)$ is the quantiles of the second-lowest new seller.
        For any $\Bq \in \cE_1 \cap \cE_3$, we have $b(\qb(T+2)) \geq s(\qs(T+2))$.
    \end{claim}
    \begin{proof}
        Let $\qb' \in I_2 \cap \Bold$ be the quantile of any original buyer in $I_2$.
        Note that such an element exists by the definition of $\cE_1$.
        In addition, by Claim~\ref{claim:r_dominance_E3_matched}, since $\Bq \in \cE_3$, we have that every original buyer in $I_2$ is matched in the optimal first-best matching.
        In particular, $\qb' \geq \qbo(T)$.
        Since $\qbn(1), \qbn(2) \in I_1$, by definition of $\cE_1$, we have $\qb(T+2) \geq \min\{\qbn(1), \qbn(2), \qbo(T)\} = \qbo(T)$ and therefore $b_{T+2} \geq \oldb_T$.
        A similar argument shows that $s_{T+2} \leq \olds_T$.
        We conclude that $b_{T+2} \geq \oldb_T \geq \olds_T \geq s_{T+2}$.
    \end{proof}
    Recall that that $\STR(\Bq) \geq \sum_{t=1}^{T+1} b(\qb(t)) - s(\qs(t))$
    and $\OPT(\Bq) = \sum_{t=1}^T b(\qbo(t)) - s(\qso(t))$.
    Since $\{\qb(1), \ldots, \qb(T+1)\} \setminus \{\qbn(1)\}$ consists of the top $T$ buyer quantiles except the highest \emph{new} buyer quantile and $\{\qbo(1), \ldots, \qbo(T)\}$ consist only of the top $T$ \emph{original} buyer quantiles, we have $\sum_{t=1}^{T+1} b(\qb(t)) - b(\qbn(1)) \geq \sum_{t=1}^T b(\qbo(t))$.
    By a similar argument, we have $\sum_{t=1}^{T+1} s(\qs(t)) - s(\qsn(1)) \leq \sum_{t=1}^T s(\qso(t))$,
    whence $\STR(\Bq) - \OPT(\Bq) \geq b(\qbn(1)) - s(\qsn(1))$.

    It remains to prove the final assertion.
    From the argument above, we know that $\STR(\Bq) - \OPT(\Bq) \geq b(\qbn(1)) - s(\qsn(1))$ whenever $\Bq \in \cE_1 \cap \cE_3$.
    So it suffices to show that $\expectsg{\Bq}{b(\qbn(1))}{\cE_1 \cap \cE_3} \geq \expects{\qb \sim I_1}{b(\qb)}$ and $\expectsg{\Bq}{s(\qsn(1))}{\cE_1 \cap \cE_3} \leq \expects{\qs \sim J_1}{s(\qs)}$.
    We prove only the first inequality since the second inequality is analogous.
    The event $\cE_1 \cap \cE_3$ guarantees that $I_1 \cap \Bnew \neq \emptyset$.
    If $\qb$ is a uniformly random quantile from $I_1 \cap \Bnew$ then $\qb$ is distributed uniformly from $I_1$. \textcolor{red}{(Chris: explain why?)}
    Note that $\qb$ FSD $\qbn(1)$ whence $\expectsg{\Bq}{b(\qbn(1))}{\cE_1 \cap \cE_3} \geq \expects{\qb \sim I_1}{b(\qb)}$.
\end{proof}

\paragraph{The bad event $\cE_2$.}
We define $\cE_2$ as
\[
    \cE_2 = \neg \cE_1 \cap (\{ \Snew \cap [0, 3rn/m] = \Snew \} \cup \{|\Bold \cap [0, 3n/m]| < n + 1\}).
\]
\textcolor{red}{Chris: updated.. change below!!}
\begin{lemma}
    For any $\Bq \in \cE_3 \cap \neg \cE_2$, we have $\STR(\Bq) \geq \OPT(\Bq)$.
    \textcolor{red}{(Chris: Following needs a proof. Can check if the existing proof carries here.)}
    Moreover,
    \[
        \expectsg{\Bq}{\OPT(\Bq) - \STR(\Bq)}{\cE_2 \cap \cE_3} \leq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
   If $\Bq \in \cE_3 \cap \cE_1$ then Lemma~\ref{lemma:r_dominance_good} asserts that $\STR(\Bq) \geq \OPT(\Bq)$.
   It remains to check that if $\Bq \in \cE_3 \cap \{ \Snew \cap [0, r] \neq \Snew \} \cap \{ |\Bold \cap [0, r^2]| \geq n + 1 \}$ then $\STR(\Bq) \geq \OPT(\Bq)$.
   Let $\OPT'(\Bq)$ be the first-best matching in the augmented market.
   Suppose that $\OPT(\Bq)$ has $T \leq n$ trades.
   We consider two cases, depending on the number of trades in $\OPT'(\Bq)$.
   
   \paragraph{Case 1: $\OPT'(\Bq)$ has at least $T + 1$ trades.}
   In this case, $\STR(\Bq)$ trades the top $T$ highest value (original and new) buyers and the bottom $T$ lowest value (original and new) sellers.
   Note that $\STR$ may trade more than this many.
   Thus, $\STR(\Bq) \geq \OPT(\Bq)$.
   
   \paragraph{Case 2: $\OPT'(\Bq)$ as $T$ trades.}
   Here, we want to show that $\STR(\Bq) = \OPT'(\Bq)$.
   By definition of STR, it suffices to show that $b(\qb(T)) \geq s(\qs(T+1))$.
   First, we claim that $\qso(T) \leq r$.
   For the sake of contradiction, let us assume that $\qso(T) > r$.
   Since $\Bq \in \{\Snew \cap [0, r] \neq \Snew\}$, we have $\qsn(1) > r$.
   Thus, $\qs(T+1) \geq \min\{\qso(T), \qsn(1)\} > r$.
   However, since $|\Bold \cap [0, r^2]| \geq n+1$ and $T \leq n$, we have that $\qb(T+1) \leq r^2$.
   Since $\qs(T+1) > r$ and $\qb(T+1) \leq r^2$, we conclude, using Claim~\ref{claim:r_stochastic_quantiles}, that $\OPT'(\Bq)$ has at least $T+1$ trades contradicting our assumption that $\OPT'(\Bq)$ has $T$ trades.
   We thus conclude that $\qso(T) \leq r$.
   
   To finish the proof, we have
   \[
        b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+1)). 
   \]
   The first inequality is because $\qb(T) \leq \qbo(T)$.
   The second inequality follows from the fact that $\OPT$ has $T$ trades.
   The last inequality is because $\qs(T+1) \geq \min\{\qso(T), \qsn(1)\} = \qso(T)$.
\end{proof}

\subsection{Comparing \STR~and \OPT~in different regimes}
Let $\alpha \in (0,1)$ be a constant to be decided later.

\paragraph{Case 1: $n \geq \alpha m$.}
Let $p = rn / 100m$.
\begin{lemma}
    \label{lemma:rdomProbE1}
    $\prob{\cE_1} \geq 1 - 6c(1-p)^c$.
\end{lemma}
\begin{proof}
    We have
    \[
        \prob{|I_1 \cap \Bnew| \leq 1}
        = (1-p)^c + c(1-p)^{c-1} p
        = (1-p)^c \left[ 1 + cp/(1-p) \right]
        < 2c (1-p)^c
    \]
    The inequality uses that $p=\frac{rn}{100m}\leq\frac{1}{100}$. Thus $p(1-p) \leq 1/4$ and $1 + c/4 \leq c + c/4 < 2c$ since $c \geq 1$.
    Identical calculations give
    \[
        \prob{|J_1 \cap \Snew| \leq 1} < 2c(1-p)^c
    \]
    Next, we have $\prob{|I_2 \cap \Bold| = 0} \geq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq (1-p)^c$ since $n\geq c$.
    Taking a union bound gives that $\prob{\neg\cE_1} \leq 6c(1-p)^c$.
\end{proof}
\textcolor{red}{BELOW NEEDS UPDATED REFERENCES}
\begin{lemma}
    \label{lemma:rdom_big_n}
    Let $\alpha > 0$ and suppose that $m \geq n \geq c \geq \Omega(\log(1/r)/r)$.
    Then
    \[
        \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0.
    \]
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:rdom_big_n}]
    Note that $\cE_1$ and $\cE_2$ are disjoint, we have
    \begin{align}
        \expect{\STR(\Bq) - \OPT(\Bq)}
        & = \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1\cap\cE_3} \label{eq:rdomE1E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2\cap\cE_3} \label{eq:rdomE2E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \cdot \prob{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \label{eq:rdomNotE1NotE2E3}\\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3} \label{eq:rdomE3}
    \end{align}
    \textcolor{red}{Update references.}
    For Eq.~\eqref{eq:rdomE1E3}, we use Lemma~\ref{lemma:cont_E1_lb}, Lemma~\ref{lemma:cont_probE3_bound}, and Lemma~\ref{lemma:contProbE1}, along with a union bound to get that
    \textcolor{red}{(Chris: add the $e^{-\Omega(rn)}$ somewhere as a claim.)}
    \begin{align*}
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot & \prob{\cE_1 \cap \cE_3} \\
        & \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot \left( 1 - 6c(1-p)^c - 4e^{-\Omega(rn)} \right).
    \end{align*}
    For Eq.~\eqref{eq:contE2E3}, we use Lemma~\ref{lemma:cont_bound_loss_E2}, Lemma~\ref{lemma:contProbE1}, and the fact that $\prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \prob{\neg\cE_1}$ to get
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2 \cap \cE_3} \geq - \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot 6c(1-p)^c
    \]
    For Eq.~\eqref{eq:rdomNotE1NotE2E3}, Lemma~\ref{lemma:contNotE2Better} gives
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \geq 0.
    \]
    Finally, for Eq.~\eqref{eq:rdomE3}, by \Cref{lemma:expectation_E3} we have
    \begin{multline*}
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}
        \\ \geq -\left( O(rn) \cdot \exp(-\Omega(rn)) + O(rm) \cdot \exp(-\Omega(rm)) \right) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \end{multline*}
    Putting everything together, it suffices to check that
    \[
        1 - 6c(1-p)^c - 4e^{-\Omega(rn)} \geq 6c(1-p)^c + O(rm) e^{-\Omega(rm)} + O(rn) e^{-\Omega(rn)}.
    \]
    Thus, as long as $m \geq n \geq \Omega(1/r)$, it suffices to choose $c$ such that $12c(1-p)^c \leq 1/2$.
    Since $12c (1-p)^c \leq 12c e^{-pc}$, a sufficient condition is $12c e^{-pc} \leq 1/2$.
    \textcolor{red}{(Chris: come back to this and check because we might need $1/r^2$ here.)}
    Taking $c \geq 4\log(24/p) / p = \Omega(\log(1/r) / r)$, we have
    %A sufficient condition is that 
    % The above inequality holds if $12c(1-p)^c \leq 1/2$ and $8m\exp(-rn/300) \leq 1/2$.
    % To prove $12c(1-p)^c \leq 1/2$, note that $p = rn/(100 m) \geq r \alpha / 100$ and thus by our choice of $c$, we have
    % $c \geq 4\log(24/p) / p$.
    % Therefore,
    \[
        12c(1-p)^c \leq 12ce^{-cp} = \frac{12cp e^{-cp}}{p} \leq \frac{12e^{-cp/2}}{p} \leq \frac{12e^{-\log(24/p)}}{p} = \frac{1}{2}.
    \]
    Note that in the second inequality, we used that $cp \geq 4$ and the numeric inequality $xe^{-x} \leq e^{-x/2}$ valid for $x \geq 4$ (see Claim~\ref{claim:xexp_lt_exp}).
    % For the inequality $8m \exp(-rn / 300) \leq 1/2$, note that this follows from the assumption that $r \geq \frac{300 \log(16 m)}{r}$.
\end{proof}

\paragraph{Case 2: $n \leq \alpha m$.}
\begin{lemma}
    \label{lemma;rdom_small_n_E1E3}
    Let $\alpha > 0$ and suppose that $n \leq \alpha m$ and $c \geq ???$.
    Then
    \[
        \prob{\cE_1 \cap \cE_3} \geq \frac{0.99 c^4}{16} \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^4.
    \]
\end{lemma}
\begin{proof}
    Recall that
    \[
        \cE_1 = \{ \Bq \,:\, |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_1 \cap \Snew| \geq 2, |J_2 \cap \Sold| \geq 1 \}
    \]
    and
    \begin{align*}
        \cE_3 = \{ \Bq \,:\,
        & |I_{\leq 2} \cap \Bold| \leq nr/2, |[n / 5m, 1] \cap \Sold| \geq nr/2, \\
        & |J_{\leq 2} \cap \Sold| \leq mr / 10, |[0, r - nr^2 / 2m] \cap \Bold| \geq mr / 10
        \}.
    \end{align*}
    Define $\cF_1 = \{I_1 \cap \Bnew| \geq 2, |J_1 \cap \Snew| \geq 2\}$.
    Since $|I_1 \cap \Bnew|$ and $|J_1 \cap \Snew|$ are both distributed as $\Binom(p, c)$, we have that
    \[
        \prob{|J_1 \cap \Bnew| = 2} = \prob{|I_1 \cap \Bnew| = 2} = \binom{c}{2} (1-p)^{c-2} p^2 \geq \frac{c^2}{4} (1-r\alpha / 100)^{c-2} p^2
    \]
    where we used that $p = rn/100m \leq r\alpha / 100$ and $\binom{c}{2} = c(c-1) / 2 \geq c^2 / 4$ since $c \geq 2$.
    Thus,
    \[
        \prob{\cF_1} \geq \frac{c^4}{16} \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^4.
    \]

    Next, let $\cF_2 = \{|I_2 \cap \Bold| \geq 1, |I_{\leq 2} \cap \Bold| \leq nr/2, |[0, r-nr^2 / 2m] \cap \Bold| \geq mr / 10\}$.
    First, we have
    \[
        \prob{|I_2 \cap \Bold| = 0} = (1-rn/100m)^m \leq e^{-rn/100}.
    \]
    Since $\expect{|I_{\leq 2} \cap \Bold|} = nr / 50$, a standard Chernoff bound gives that
    \[
        \prob{|I_{\leq 2} \cap \Bold| > nr / 2} \leq e^{-\Omega(nr)}.
    \]
    In addition, since $r - nr^2 / 2m \geq r/2$ and $\expect{|[0, r/2] \cap \Bold|} = mr/2$, we have that
    \[
        \prob{|[0, r - nr^2 / 2m] \cap \Bold| \geq mr/10} \leq e^{-\Omega(mr)}.
    \]
    Thus a union bound gives
    \[
        \prob{|I_2 \cap \Bold| \geq 1, |I_{\leq 2} \cap \Bold| \leq nr/2, |[0, r-nr^2 / 2m]} \leq 1 - e^{-\Omega(nr)}.
    \]
    Using a union bound, we conclude that
    \[
        \prob{\cF_2} \geq 1 - e^{-\Omega(nr)}.
    \]
    In particular, if $n \geq \Omega(1/r)$ then $\prob{\cF_2} \geq 0.999$.

    Finally, we define $\cF_3 = \{ |J_2 \cap \Sold| \geq 1, |J_{\leq 2} \cap \Sold| \leq mr / 10, |[n/5m, 1] \cap \Sold| \geq nr/2 \}$.
    Since $\expect{|J_{\leq 2} \cap \Sold|} = n^2 r / 100m$, a standard Chernoff bound gives
    \[
        \prob{|J_{\leq 2} \cap \Sold| > mr / 10} \leq e^{-\Omega(mr)}.
    \]
    Next, since $\expect{|[n/5m,1] \cap \Sold|} \geq \expect{|[1/5, 1] \cap \Sold|} = 4n/5$, we have
    \[
        \prob{|[n/5m, 1] \cap \Sold| < nr/2} \leq e^{-\Omega(n)}.
    \]
    We need to take some care in dealing with the event $|J_2 \cap \Sold| \geq 1$.
    Let $k \geq nr / 2$.
    Then
    \begin{align*}
        \probg{|J_2 \cap \Sold| = 0}{|[n/5m, 1] \cap \Sold| = k}
        & = \left(1 - \frac{rn/100m}{1-n/5m} \right)^k \\
        & \leq \left(1 - rn/100m \right)^k \\
        & \leq e^{-rnk / 100m} \\
        & \leq e^{-\Omega(r^2 n^2)}.
    \end{align*}
    Thus, we have
    \[
        \prob{|J_2 \cap \Sold| = 0, |[n/5m, 1] \cap \Sold| \geq nr/2} \geq (1 - e^{-\Omega(r^2 n^2)})(1 - e^{-\Omega(n)}).
    \]
    Finally, a union bound gives that
    \[
        \prob{\cF_3} \geq (1 - e^{-\Omega(r^2 n^2)})(1 - e^{-\Omega(n)}) - e^{-\Omega(mr)}.
    \]
    In particular, if $m \geq n \geq \Omega(1/r)$ then $\prob{\cF_3} \geq 0.999$.
    Note that $\cF_1, \cF_2, \cF_3$ are defined so that the events are mutually independent. The claim thus follows by taking a product.
\end{proof}


% \begin{lemma}
%     \label{lemma:rdom_small_n_E1}
%     Let $\alpha > 0$ and suppose that $n \leq \alpha m$ and $c \geq 2$.
%     Then
%     \[
%         \prob{\cE_1} \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6.
%     \]
% \end{lemma}
% \begin{proof}
%     Since $|I_1 \cap \Bnew|$ and $|J_1 \cap \Snew|$ are both distributed as $\Binom(p, c)$, we have that
%     \[
%         \prob{|J_1 \cap \Bnew| = 2} = \prob{|I_1 \cap \Bnew| = 2} = \binom{c}{2} (1-p)^{c-2} p^2 \geq \frac{c^2}{4} (1-r\alpha / 100)^{c-2} p^2
%     \]
%     where we used that $p = rn/100m \leq r\alpha / 100$ and $\binom{c}{2} = c(c-1) / 2 \geq c^2 / 4$ since $c \geq 2$.
%     Next, since $|I_2 \cap \Bold|$ is distributed as $\Binom(p, m)$ and $|J_2 \cap \Sold|$ is distributed as $\Binom(p, n)$, we have
%     \[
%         \prob{|I_2 \cap \Bold| = 0} \leq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq 1-p.
%     \]
%     Therefore, $\prob{|I_2 \cap \Bold| \geq 1} \geq \prob{|J_2 \cap \Sold| \geq 1} \geq p$.
%     Since the random variables $|I_1 \cap \Bnew|, |J_1 \cap \Snew|, |I_2 \cap \Bold|, |J_2 \cap \Sold|$ are all independent, the lemma follows by taking a product.
% \end{proof}
\begin{lemma}
    \label{lemma:rdom_small_n_E2}
    Suppose that $n \leq mr^2 / 8$.
    Then $\prob{\cE_2} \leq r^c + e^{-\Omega(n)}$.
\end{lemma}
\begin{proof}
    Recall that $\cE_2 \subset \{\Snew \cap [0,3rn/m] = \Snew\} \cup \{|\Bold \cap [0, 3n/m]| < n+1|\}$.
    In addition, recall that each new seller is assigned a uniformly random quantile.
    Thus, we have
    \[
        \prob{\Snew \cap [0, r] = \Snew} = (3rn/m)^c.
    \]
    Next, since $\expect{|\Bold \cap [0, 3n/m]|} = 3n$, we have $\prob{|\Bold \cap [0, 3n/m]| < n+1} \leq e^{-\Omega(n)}$.
\end{proof}

% \textcolor{red}{(Chris: In the above, the $n$ appears again. This is an attempt to check what happens if we slightly redefine $\cE_2$.}
% \textcolor{red}{START NEW}

% Let us define
% \[
%     \cE_2 = \neg \cE_1 \cap (\{\Snew \cap [0, \max\{3n/m, 1/\sqrt{m}\} / r] = \Snew\} \cup \{|\Bold \cap [0, \max\{3n/m, 1/\sqrt{m}\}]| < n+1\}.
% \]
% \begin{lemma}
%     We have that
%     \[
%         \prob{\cE_2} \leq
%         \begin{cases}
%             (3n/rm)^c + e^{-\Omega(\sqrt{m})} & n \geq \sqrt{m} / 3 \\
%             (1/r\sqrt{m})^c + e^{-\Omega(\sqrt{m})} & n < \sqrt{m} / 3
%         \end{cases}.
%     \]
% \end{lemma}
% \begin{proof}
%     Suppose that $3n / m \geq 1/\sqrt{m}$, i.e.~$n \geq \sqrt{m} / 3$.
%     In this case $\max\{3n/m, 1/\sqrt{m}\} = 3n/m$.
%     Then
%     \[
%         \prob{\Snew \cap [0, 3n/rm] = \Snew}
%         = (3n/rm)^c
%     \]
%     and
%     \[
%         \prob{|\Bold \cap [0, 3n/m]| < n+1} \leq e^{-\Omega(n)} \leq e^{-\Omega(\sqrt{m})}.
%     \]

%     Now suppose that $3n/m < 1 / \sqrt{m}$ so that $\max\{3n/m, 1/\sqrt{m}\} = \sqrt{m}$. In particular $n < \sqrt{m} / 3$.
%     In this case
%     \[
%         \prob{\Snew \cap [0, 1/r\sqrt{m}] = \Snew}
%         = (1/r\sqrt{m})^c
%     \]
%     and
%     \[
%         \prob{|\Bold \cap [0, 1/\sqrt{m}]| < \sqrt{m}+1} \leq e^{-\Omega(\sqrt{m})}.
%     \]
% \end{proof}

% \textcolor{red}{END NEW}

\begin{lemma}
    If $m \geq n \geq c \geq ???$ and $n \leq mr^2 / 8$ then $\expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0$.
\end{lemma}
\begin{proof}
    First, we have
    \[
        \prob{\cE_1 \cap \cE_3}
        \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6 - 4 e^{-\Omega(rn)}.
    \]
    Next, we have
    \[
        \prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq r^c + e^{-\Omega(n)}.
    \]
    We thus require that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6 \geq r^c + e^{-\Omega(rn)}
    \]
    If $c \geq 2$ then $c^4 / 16 \geq 1$.
    So we only need to check that
    \[
        p^6 = \left( \frac{rn}{100m} \right)^6 \geq \frac{r^c + e^{-\Omega(rn)}}{\left(1 - r\alpha/100\right)^{2c}}
    \]
\end{proof}

==> r_overlap_bad_example.tex <==
\section{Bad example for $r$ overlap case}
Here we construct a bad example for $r$ overlap.
We begin by proving that it is a bad example for trade reduction where we are forced to lose a pair.

The distribution is as follows. Let $N \gg 3$.
\[
    F_B = \begin{cases}
        N & \text{w.p.~$\eps$} \\
        2 & \text{w.p.~$r-\eps$} \\
        0 & \text{w.p.~$1-r$}
    \end{cases}
    \quad \text{and} \quad
    F_S = \begin{cases}
        3 & \text{w.p.~$1-r$} \\
        1 & \text{w.p.~$r$}
    \end{cases}.
\]
Suppose we have $m$ buyers and $1$ seller.
Then we can lower bound $\OPT$ by $N-3$ when at least one buyer has value $N$, i.e.~$\OPT \geq (N-3) \cdot \left[ 1 - (1-\eps)^m \right]$.

For trade reduction, suppose we add $c$ additional buyers and sellers.
If there is exactly one buyer with value $N$ then the GFT of trade reduction is upper bounded by $N + c$ when there are at least $2$ sellers with value $1$.
Note that if there is only a single seller with value $1$ then the only possible trade is the buyer with value $N$ and the seller with value $1$.
This trade is then reduced and trade reduction has a GFT of $0$.
The GFT contributed from this event is upper bounded by
\[
    (N + c) \cdot \underbrace{\left[(m+c) \cdot (1-\eps)^{m+c-1} \cdot \eps\right]}_{\text{exactly $1$ buyer with value $N$}}
    \underbrace{\left[1 - (1-r)^{c+1} - (c+1)r(1-r)^{c}\right]}_{\text{at least $2$ sellers with value $1$}}.
\]
Next, if there are at least two buyers with value $N$, a trivial upper bound is $X \cdot N + c$ where $X$ is the number of buyers with value $N$.
We have that $\prob{X \geq 2} = 1 - (1-\eps)^{m+c} - (m+c) \cdot (1-\eps)^{m+c-1} \cdot \eps$.
Thus, an upper bound on the value of trade reduction is given by
\begin{align*}
    N \cdot & \left[(m+c) \cdot (1-\eps)^{m+c-1} \cdot \eps\right]
    \left[1 - (1-r)^{c+1} - (c+1)r(1-r)^{c}\right] \\
    & +
    N \cdot \left[1 - (1-\eps)^{m+c} - (m+c) \cdot (1-\eps)^{m+c-1} \cdot \eps\right]
    + c
\end{align*}

==> zz_fsd_noniid_approx_oct23.tex <==
\section{Approximation and Augmentation for FSD but Non-i.i.d.~Distributions}
\label{sec:fsd_noniid_approx}
In this section, we consider the following setting.
Let us assume that we have $m$ buyers whose value distributions are given by $F_1, \ldots, F_m$ and $n$ sellers whose cost distributions are given by $G_1, \ldots, G_n$.

\begin{definition}
    We say that a market is $(c,\gamma)$-dominant if there exists sets $B \subseteq [m]$ and $S \subseteq [n]$ such that $|B| = |S| = c$ and $F_i^{-1}(1-\gamma) \geq G_j^{-1}(\gamma)$ for all $i \in B, j \in S$.
\end{definition}

\begin{theorem}
    \label{thm:fsd_noniid_approx}
    If a market is $(c, \gamma)$-dominant then Trade Reduction obtains a $(1-O(1/\gamma^2 c))$-approximation to the first-best GFT.
\end{theorem}

For the proof, we need to define a bit of notation.
We fix $\gamma \in (0, 1/2]$ and let $\alpha, N, T, f$ be as given by \Cref{lemma:combinatorial_fsd_approx}.
For a set of quantiles $\qb(1), \ldots, \qb(c)$ and $\qs(1), \ldots, \qs(c)$, define the random sets $B_+ = \{i \,:\, \qb(i) \geq 1-\gamma$ and $S_+ = \{i \,:\, \qs(i) \leq \gamma\}$.
We also define the following four events.
\begin{align*}
    & \cE(1,1) = \{|B_+| \geq \alpha c, |S_+| \geq \alpha c\},
    &&
    \cE(1,0) = \{|B_+| \geq \alpha c, |S_+| < \alpha c\}, \\
    & \cE(0,1) = \{|B_+| < \alpha c, |S_+| \geq \alpha c\}, 
    &&
    \cE(0,0) = \{|B_+| < \alpha c, |S_+| < \alpha c\}.
\end{align*}
Also define the events
\[
    \cE(B_+, S_+) = \{\qb(i) \geq 1-\gamma \text{ if and only if } i \in B_+, \qs(j) \geq 1-\gamma \text{ if and only if } j \in S_+\}.
\]
Finally, we write
\[
    \OPT(B_+, S_+) = \expectg{\OPT(\Bq_B, \Bq_S)}{\cE(B_+, S_+)}.
\]

\begin{lemma}
    \label{lemma:opt_monotone}
    If $B_+' \supseteq B_+$ and $S_+' \supseteq S_+$ then $\OPT(B_+', S_+') \geq \OPT(B_+, S_+)$.
\end{lemma}

\begin{lemma}
    \label{lemma:tr_lose_one_trade}
    Let $k = \min\{|B_+|, |S_+|\}$.
    Then $\TR(B_+, S_+) \geq \left( 1 - \frac{1}{k} \right) \OPT(B_+, S_+)$.
\end{lemma}

\begin{lemma}
    \label{lemma:opt_approx}
    If $n \geq N$ then $\OPT(\cE(1,1)) \geq (1-3/n) \cdot \OPT$.
\end{lemma}
\begin{proof}
    Note that $\prob{\cE(B_+, S_+)} = \gamma^{|B_+|}(1-\gamma)^{n-|B_+|} \gamma^{|S_+|} (1-\gamma)^{n-|S_+|}$.
    We now consider three cases.

    \textbf{Case 1: $|B_+| < \alpha n$ and $|S_+| < \alpha n$.~~} We have
    \begin{align*}
        \sum_{t_1, t_2 \in [T]} \OPT(f_{t_1}(B_+), & f_{t_2}(S_+)) \cdot \prob{\cE(f_{t_1}(B_+), f_{t_2}(S_+))} \\
        & \geq 
        n \cdot \sum_{t_1 \in [T]} \OPT(f_{t_1}(B_+), S_+) \cdot \prob{\cE(f_{t_1}(B_+), S_+)} \\
        & \geq
        n^2 \cdot \OPT(B_+, S_+) \cdot \prob{\cE(B_+, S_+)}.
    \end{align*}
    We conclude that $\OPT(\cE(1, 1)) \geq n^2 \cdot \OPT(\cE(0, 0))$.
    
    \textbf{Case 2: $|B_+| < \alpha n$ and $|S_+| \geq \alpha n$.~~} We have
    \begin{align*}
        \sum_{t \in [T]} \OPT(f_{t}(B_+), S_+) \cdot \prob{\cE(f_{t}(B_+), S_+)}
        \geq
        n \cdot \OPT(B_+, S_+) \cdot \prob{\cE(B_+, S_+)}.
    \end{align*}
    We conclude that $\OPT(\cE(1, 1)) \geq n \cdot \OPT(\cE(0, 1))$.

    \textbf{Case 3: $|B_+| \geq \alpha n$ and $|S_+| < \alpha n$.~~}
    This is analogous to the previous case and we get that $\OPT(\cE(1, 1)) \geq n \cdot \OPT(\cE(1, 0))$.
\end{proof}

\begin{proof}[Proof of \Cref{thm:fsd_noniid_approx}]
    By \Cref{lemma:tr_lose_one_trade}, we have $\TR \geq \TR(\cE(1, 1)) \geq \left(1 - 1/\alpha n \right) \OPT(\cE(1, 1))$.
    By \Cref{lemma:opt_approx}, we have $\OPT(\cE(1, 1)) \geq (1 - 3 / n) \cdot \OPT$.
    We conclude that $\TR \geq (1 - (1/\alpha + 3) / n) \cdot \OPT$.
\end{proof}

\begin{lemma}
    \label{lemma:combinatorial_fsd_approx}
    There are functions $\alpha(\gamma) = \Theta(\gamma^2)$ and $N(\gamma) = \Theta(1/\gamma^2)$ such that the following holds.
    For any $\gamma \in (0, 1/2]$, if $n \geq N(\gamma)$ then there exists $T$ and a function $f \colon \binom{[n]}{\leq \alpha(\gamma) \cdot n} \to (2^{[n]})^T$ satisfying the following properties.
    \begin{enumerate}[topsep=0pt, itemsep=0pt]
        \item For every $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha(\gamma) n}$ we have $|f_t(S)| \geq \gamma n$.
        % \item For every $t_1, t_2 \in [T]$ and $S_1, S_2 \in \binom{[n]}{\leq \alpha(\gamma) n}$, we have $f_{t_1}(S_1) \neq f_{t_2}(S_2)$ whenever $(t_1, S_1) \neq (t_2, S_2)$.
        \item For every $S \in \binom{[n]}{\leq \alpha(\gamma) n}$, we have $n \cdot \gamma^{|S|} (1-\gamma)^{n - |S|} \leq \frac{1}{Z_S} \sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|}$ where $Z_S = \max_Y |\{ t \,:\, f_t(S) = Y\}|$.
    \end{enumerate}
\end{lemma}

\subsection{Proof of \Cref{lemma:combinatorial_fsd_approx}}
\begin{proof}[Proof of \Cref{lemma:combinatorial_fsd_approx}]
    We consider the following probabilistic construction of $f$.
    For each $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$, we set $f_t(S)$ to be the set which chooses a uniformly random subset from $[n] \setminus S$ of size $\gamma n$. Note that the first item is trivial by construction so we only need to check the second item.

    To that end, fix $S \in \binom{[n]}{\leq \alpha n}$.
    We have that $\sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|} = T \gamma^{|S| + \gamma n} (1-\gamma)^{n - |S| - \gamma n}$
    so we need to check that $Z_S \leq \frac{T \gamma^{\gamma n}(1-\gamma)^{-\gamma n}}{n}$.
    
    If $S \setminus Y \neq \emptyset$ then $\prob{f_t(S) = Y} = 0$.
    So now suppose that $S \subseteq Y$.
    Since $|Y| - |S| = \gamma n$, we have
    \[
        \prob{f_t(S) = Y} \leq \binom{n-|S|}{\gamma n}^{-1} \leq \binom{n(1-\alpha)}{\gamma n}^{-1} \leq \left(\frac{1-\alpha}{\gamma} \right)^{\gamma n}.
    \]
    Let $Z_S(Y) = |\{t \,:\, f_t(S) = Y\}|$.
    Then $\expect{Z_S(Y)} \leq \left( \frac{1-\alpha}{\gamma} \right)^{\gamma n} T$.

    % \begin{claim}
    %     \label{claim:combinatorial2}
    %     With probability at least $1-T^2 (e/\alpha)^{2\alpha n} \left( \frac{\gamma}{1-\alpha} \right)^{\gamma n}$, we have $f_{t_1}(S_1) \neq f_{t_2}(S_2)$ for all $t_1, t_2 \in [T]$ and $S_1, S_2 \in \binom{[n]}{\leq \alpha n}$ provided $(t_1, S_1) \neq (t_2, S_2)$.
    % \end{claim}
    % \begin{proof}
    %     Note that we only need to compare $S_1, S_2 \in \binom{[n]}{\leq \alpha n}$ with $|S_1| = |S_2|$ since $|f_t(S_1)| = \alpha n + |S_1|$.
    %     Let us condition on $f_{t_1}(S_1)$. If $S_2 \setminus f_{t_1}(S_1) \neq \emptyset$ then $\probg{f_{t_2}(S_2) = f_{t_1}(S_1)}{f_{t_1}(S_1)} = 0$. Otherwise, we have $\probg{f_{t_2}(S_2) = f_{t_1}(S_1)}{f_{t_1}(S_1)} = \binom{n-|S_1|}{\gamma n}^{-1} \leq \binom{n(1-\alpha)}{\gamma n}^{-1}$.
    %     We conclude that
    %     \[
    %         \prob{f_{t_1}(S_1) = f_{t_2}(S_2)} \leq \binom{n(1-\alpha)}{\gamma n}^{-1} \leq \left( \frac{\gamma}{1-\alpha} \right)^{\gamma n}.
    %     \]
    %     Taking a union bound over all pairs of $(t_1,S_1)$ and $(t_2, S_2)$ gives that
    %     \begin{align*}
    %         \prob{\exists (t_1, S_1), (t_2, S_2) \text{ such that }f_{t_1}(S_1) = f_{t_2}(S_2)}
    %         \leq T^2 (e/\alpha)^{2\alpha n} \left( \frac{\gamma}{1-\alpha} \right)^{\gamma n},
    %     \end{align*}
    %     where in the last inequality we used that $|\binom{[n]}{\leq \alpha n}| \leq (e/\alpha)^{\alpha n}$ (see \Cref{fact:binom_bounds}).
    % \end{proof}
    \begin{claim}
        \label{claim:combinatorial3}
        Suppose that $T \geq n \cdot \left( \frac{1-\gamma}{\gamma} \right)^{\gamma n}$.
        Then
        \[
            n \cdot \gamma^{|S|} (1-\gamma)^{n - |S|} \leq \sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|}
        \]
        for every $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$.
    \end{claim}
    \begin{proof}
        Since $|f_t(S)| = \gamma n + |S|$, we have
        \[
            \gamma^{|f_t(S)|} (1-\gamma)^{n - |f_t(S)|}
            = \gamma^{|S| + \gamma n} (1-\gamma)^{n - |S| - \gamma n}.
        \]
        Thus, so long as $T \geq n \cdot \left( \frac{1-\gamma}{\gamma} \right)^{\gamma n}$, we have
        \begin{align*}
            \sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|}
            & = n \cdot (1-\gamma)^{\gamma n} \gamma^{-\gamma n} \gamma^{|S| + \gamma n} (1-\gamma)^{n - |S| - \gamma n} \\
            & = n \cdot \gamma^{|S|} (1-\gamma)^{n-|S|}. \qedhere
        \end{align*}
    \end{proof}
    The only remaining step is to choose parameters so that the probability in \Cref{claim:combinatorial2} is strictly positive.
\end{proof}
\begin{fact}[{\cite[Exercise~2.14]{boucheron2013concentration}}]
    \label{fact:binom_bounds}
    For all $n \geq 1$ and $1 \leq k \leq n$, we have $\sum_{j = 0}^k \binom{n}{k} \leq \left( \frac{en}{k} \right)^k$.
\end{fact}

\begin{claim}
    \label{claim:alpha_log_e_alpha}
    Fix $x \in (0, 1)$.
    Suppose that $0 <\alpha \leq \frac{x}{1 + 2\log(1/x)}$.
    Then $\alpha \log(e/\alpha) \leq x$.
    Equivalently, $(e/\alpha)^{\alpha} \leq e^x$.
\end{claim}
\begin{proof}
    First we check that $\frac{x}{1 + 2 \log(1/x)} < 1$ whence $\alpha < 1$.
    Let $f(x) = \frac{x}{1+2\log(1/x)}$.
    Then $f'(x) = \frac{2\log(1/x) + 3}{(1+2\log(1/x))^2} > 0$ when $x \in (0, 1)$.
    Thus, $f(x) \leq f(1) = 1$ when $x \in (0, 1)$.
    Now let $g(\alpha) = \alpha \log(e/\alpha)$.
    Then $g'(\alpha) = - \log(\alpha) > 0$ when $\alpha < 1$ so it suffices to check the claim only when $\alpha = \frac{x}{1 + 2\log(1/x)}$.
    In this case, we have
    \begin{align*}
        \alpha \log(e/\alpha)
        & = \frac{x}{1 + 2\log(1/x)} \left[1 + \log\left( \frac{1 + 2\log(1/x)}{x} \right) \right] \leq x \\
        & \leq \frac{x}{1 + 2\log(1/x)} \cdot [1 + 2\log(1/x)] = x,
    \end{align*}
    where the inequality is from \Cref{claim:alpha_log_e_alpha_aux}.
\end{proof}
\begin{claim}
    \label{claim:alpha_log_e_alpha_aux}
    If $x \in (0,1)$ then $\log((1+2\log(1/x))/x) \leq 1 + 2\log(1/x)$.
\end{claim}
\begin{proof}
    By exponentiating, the inequality is equivalent to $1 + 2 \log(1/x) \leq 1/x^3$.
    Taking $u = 1/x$ the inequality is equivalent to $1 + 2\log u \leq u^3$ for $u > 1$.
    Let $f(u) = u^3 - 2 \log u - 1$.
    Then $f(1) = 0$ and $f'(u) = 3u^2 - 2 / u > 0$ when $u \geq 1$.
    We conclude that $f(u) \geq 0$ for all $u \geq 1$.
\end{proof}

\begin{claim}
    \label{claim:log_ineq1}
    Let $a, b > 0$.
    If $x \geq 2 \max\{a, 5(b+1)(1 + \log(b+1))\}$ then $x \geq a + b\log x$.
    Equivalently, $e^x / x^b \geq e^a$.
\end{claim}
\begin{proof}
    We have $x - b\log x \geq x/2 \geq a$ where the first inequality follows from \Cref{claim:log_ineq2} and the second inequality is because $x \geq 2a$.
\end{proof}
\begin{claim}
    \label{claim:log_ineq2}
    Fix $b > 0$.
    If $x \geq 10(b+1)(1 + \log(b+1))$ then $x - b \log x \geq x / 2$.
\end{claim}
\begin{proof}
    The last inequality is equivalent to $x/2 - b \log x \geq 0$.
    Let $f(x) = x/2 - b\log x$.
    Note that $f'(x) = 1/2 - b / x$ so $f$ is increasing on $(2b, \infty)$.
    Thus it suffices to prove that $f(x) \geq 0$ when $x= 10(b+1)(1 + \log(b+1))$.
    Let
    \begin{align*}
        g(b)
        & = f(2(b+1)(1 + \log(b+1))) \\
        & = 5(b+1) + 5(b+1) \log(b+1) - b \log(2) - b \log(b+1) - b\log(1 + \log(b+1)).
    \end{align*}
    Some calculations give that
    \begin{align*}
        g'(b) & = 5 + 5(\log(b+1) + 1) - \log(2) - \frac{b}{b+1} - \log(b+1) \\
        & - \frac{b}{(b+1)(1 + \log(b+1))} - \log(1+\log(b+1)).
    \end{align*}
    Differentiating again gives
    \begin{align*}
        g''(b) & = \frac{5}{b+1} + \frac{1}{(b+1)^2} - \frac{1}{b+1} + \frac{b - \log(b+1) + 1}{(b+1)^2(1+\log(b+1))^2} - \frac{1}{(b+1)(1+\log(b+1))} \\
        & = \frac{4}{b+1} + \frac{1}{(b+1)^2} - \frac{(b+2) \log(b+1)}{(b+1)^2(1 + \log(b+1))^2} \\
        & = \frac{4(b+1)(1 + 2 \log(b+1) + \log^2(b+1)) - (b+2) \log(b+1)}{(b+1)^2(1 + \log(b+1))^2} + \frac{1}{(b+1)^2} > 0.
    \end{align*}
    Note that $g(0) = 5$ and $g'(0) = 10 - \log 2 > 0$ and $g'(b) > 0$ for all $b > 0$.
    We conclude that $g(b) \geq g(0) > 0$ for all $b > 0$.
\end{proof}

==> zz_intro_nov07_2023.tex <==
\section{Introduction}
In this paper, we study the problem of maximizing the gains from trade (GFT) in two-sided markets.
Two-sided markets are ubiquitous and have many practical applications;
some major examples include the FCC spectrum auction and online marketplaces such as Uber, Lyft, and Airbnb.
For example, in ride-sharing platforms like Uber and Lyft, passengers (as the role of buyers) have some private value for obtaining transportation services and drivers (as the role of sellers) have some private cost for providing the necessary services.
Mechanism design for two-sided markets poses additional challenges over its one-sided counterpart.
In a one-sided market, the mechanism designer aims to maximize some objective (e.g.~welfare or revenue) subject to a one-sided incentive-compatibility constraint.
The seminal papers of \citet{Vickrey61} and \citet{Myerson81} described how to design mechanisms that achieve the optimal welfare and revenue for one-sided markets, respectively.
However, in a two-sided market, one needs to ensure incentive compatibility for \emph{both} sides of the market as well as to ensure that the mechanism itself does not run a deficit (called \emph{budget balance}). The seminal impossibility result of \citet{MyersonS83} show that these additional constraints make the mechanism design problem much more challenging.
In particular, even in the simplest setting with  a single seller selling a single item to a single buyer (known as bilateral trade), no mechanism can achieve full efficiency while being Bayesian incentive-compatible (BIC), individually rational (IR), and budget balanced (BB). \citet{MyersonS83} also described the best BIC, IR and BB mechanism that maximizes efficiency in bilateral trade. However, the optimal mechanism is complex and heavily depends on the prior.

Motivated by the aforementioned challenges, there has been extensive research efforts and substantial progress in recent years investigating the two-sided market in the ``simple versus optimal'' perspective, i.e. to show that a simple mechanism can approximate the performance of the optimal mechanism.
A non-exhaustive list includes \cite{BabaioffCGZ18, CaiGMZ21, BrustleCWZ17, DengMSW22, KangPV22, MaoPW22, Fei22, CaiW23,BlumrosenD21,BlumrosenM16,colini2017fixed, Colini-Baldeschi16, colini2020approximately, DuttingRT14}. However, in many of these results, the mechanism designer requires a priori knowledge of both the buyers' and the sellers' distribution. Alternatively, the designer can increase the competition and thus her objective by recruiting more agents to the market.
In single-item one-sided markets, the seminal work by \citet{BulowK94} showed that the revenue of a second price auction with only a \emph{single} additional participant from the same population is at least that of the optimal mechanism with the original set of participants.
More recently, this result has been generalized to other one-sided market settings \cite{HartlineR09, EdenFFTW17, FeldmanFR18, FuLR19, BeyhagiW19, SivanS13, DughmiRS09, LiuP18}.
Such results showcase how additional competition, coupled with a simple mechanism
can be used to overcome the requirement of having precise knowledge of the underlying distribution and using the optimal-yet-complex mechanism. A natural question is whether such Bulow-Klemperer-type results also hold in the two-sided market settings.

In a recent paper, \citet{BabaioffGG20} initiated this line of work to develop Bulow-Klemperer-type results for a fundamental single-parameter two-sided market setting called a \emph{double auction}.
In this problem there are $n$ sellers that each hold an identical item and each the value of each seller drawn i.i.d.~from some distribution $F_S$.
There are $m$ buyers that each wish to obtain one of these items and their value is drawn i.i.d.~from another distribution $F_B$.
They consider a variant of the natural, prior-independent Trade Reduction mechanism \cite{McAfee92}, which they call Buyer Trade Reduction (BTR).
They show that when the two distributions are identical,\footnote{Note that no further assumptions are placed on this distribution, while similar results in one-sided markets make certain regularity assumption about the distribution.}
%when both sides of the market have values drawn i.i.d.~from a common distribution
BTR with one additional buyer can achieve welfare at least the best welfare achievable in the original market even without the BIC, IR, and BB constraints (such a benchmark is called the \emph{first best}). Note that the first best is exactly the welfare of the celebrated VCG mechanism, which is BIC and IR, but may violate the BB constraint.
% \aranyaknote{(don't need to add, just curious) Does a simple mechanism give an approx to first-best (or second best) in the identical distributions case?}
%as efficient as the \emph{optimal allocation} (i.e.~even ignoring BIC, IR, and BB considerations) before augmentation.
%They then consider the setting where the two sides of the markets may have different distributions but where each side of the market remains i.i.d.
%With no assumptions, they prove that no finite bound is possible, even in the setting of bilateral trade.
While this resolves the most basic case, it is rarely assumed that both distributions are identical.
For example, a passenger in ride-sharing applications most likely has higher value for obtaining transportation than the driver's cost for providing such transportation.
When there are no assumptions on the distributions, \citet{BabaioffGG20} prove that no finite bound is possible.
Despite this negative result, they prove that when the buyers' distribution first-order stochastically dominates\footnote{A distribution $D$ first-order stochastically dominates $D'$ if $\Pr_{x\sim D}[x\leq c]\leq \Pr_{x\sim D'}[x\leq c]$ for every $c$.} the sellers' distribution, $n(m + 4\sqrt{m})$ additional buyers are sufficient for BTR to have welfare at least the first-best welfare in the original market
%optimal allocation where %$m$ is the number of buyers, $n$ is the number of sellers, and 
when $m \geq n$.\footnote{Their result applies to the $m\leq n$ case using \emph{Seller Trade Reduction}.}

{An immediate question from Babaioff et al.'s result is whether the number of additional agents can be improved. Does a constant number of agents suffice for any number of buyers and sellers?} The main difficulty turns out to come from the mechanism recruiting only one side of the market. In fact, their paper shows that $\lfloor \log_2 m \rfloor$ buyers are necessary if only extra buyers are recruited, even when there is a single seller. However in many situations, %it is reasonable to assume that one 
the mechanism designer is able to recruit both buyers and sellers. For example, in ride-sharing applications, recruiting both sides is very much feasible -- more riders will use the platform with better marketing, advertisement, or deals, and more drivers will adopt the platform with better incentives and marketing towards them.
%(remove: there is an abundance of both passengers and drivers. More agents will start using the application if more advertisements are served.)
%, although the number sellers may be a constant fraction of the number of buyers.
In this paper, we allow recruiting from \emph{both} sides of the market. We show that with the Seller Trade Reduction (STR), a mechanism analogous to BTR, 
%which is very similar to BTR, with 
only $O(1)$ additional agents suffice.
%guarantees GFT at least the first-best GFT in the original market. See \Cref{thm:main_str} for the formal statement.
We give a formal definition of the mechanism in \Cref{subsec:results}.

To formally state our result, it is crucial to first discuss the measure of efficiency we adopt in this paper.  There are two main measures of efficiency in two-sided markets.
The first is the standard notion of \emph{welfare} in the literature, which is equal to the sum of the value of all buyers and sellers that hold the items in the final allocation.
The second is the \emph{gain from trade (GFT)} which is the welfare of the final allocation minus the total value of sellers.
At a high-level the GFT of a mechanism is a direct measure of the \emph{additional} value of a mechanism.
Note that when the set of sellers is fixed, maximizing welfare in a market where only the buyers are augmented (as in \cite{BabaioffGG20}) is identical to maximizing the GFT.
In other words, there is no need to make a distinction between welfare and GFT.
However, since we are interested in the problem where both sides of the market can be augmented, we focus on GFT as it is the more meaningful measure. As an extreme example, simply augmenting the market with additional sellers, and leaving them untraded, would increase the welfare while the GFT remains unchanged. It is not hard to see that our result implies that the welfare achieved by STR in the augmented market exceeds the first-best welfare in the original market (see \Cref{cor:main_str}).

\subsection{Our results and techniques}
\label{subsec:results}
We summarize prior results and our results in Table~\ref{table:results}.
Our main result is \Cref{thm:main_str} which states that if we use a simple and prior-independent mechanism, namely Seller Trade Reduction (STR), then augmenting both sides of the market by a constant number of participants has at least as much GFT as the optimal allocation before augmentation,
assuming that the buyers' distribution first-order stochastically dominates the sellers' distribution.

The STR mechanism was introduced by \cite{BabaioffGG20} and is a variant of the Trade Reduction mechanism \cite{McAfee92}. Given the buyer's bids $b^{(1)} \geq \ldots \geq b^{(m)}$ and the seller's bids $s^{(1)} \leq \ldots \leq s^{(n)}$, let $r = \max\{ i \leq \min\{m ,n\} \,:\, b^{(i)} \geq s^{(i)} \}$. The welfare-maximizing allocation (called first best, which we denote by OPT) trades the $r$ highest-value buyers with the $r$ lowest-value sellers. We refer to the value $r$ as the \emph{optimal trade size}. The STR mechanism works as follows.
For notation, let $s^{(n+1)} = \infty$.
If $b^{(r)} \geq s^{(r+1)}$, the mechanism offers a price of $s_{r+1}$ to the $r$ highest-value buyers with the $r$ lowest-value sellers, resulting in a matching of size $r$. Otherwise, the $r-1$ highest-value buyers trade with the $r-1$ lowest-value sellers. Each traded buyer pays $b^{(r)}$ while each traded seller receives $s^{(r)}$. In the latter case, we say that the last trade is \emph{reduced}.

\newcommand{\withincell}[1]{
\begin{tabular}{@{}c@{}}
    #1
\end{tabular}
}

\begin{table}[t]
    % \centering
    \centerline{
    \begin{tabular}{|c|c|c|c|}
    \hline 
    \multirow{2}{*}{Distribution Assumptions} & \multicolumn{2}{c|}{Upper Bound} & \multirow{2}{*}{Lower Bound} \\ 
    \cline{2-3}
    & Previous Work & This Work & \\
    \hline
    $F_B=F_S$ & \withincell{1 buyer \\ \cite[Theorem~1.1]{BabaioffGG20}} & -- & 1 agent (trivial) \\ 
    \hline
    $F_B$ FSD $F_S$ & \withincell{$n(m+4\sqrt{m})$ buyers \\ \cite[Theorem~1.10]{BabaioffGG20}} & \withincell{$O(1)$ agents \\ (\Cref{thm:main_str})} & \withincell{$\lfloor \log_2 m \rfloor$ buyers \\ \cite[Theorem~5.1]{BabaioffGG20}} \\  
    \hline
    $\Pr_{b\sim F_B, s\sim F_S}[b\geq s] = r$ & -- &
    \begin{tabular}{@{}c@{}} $O(\frac{\log(m/n)+\log(1/r)}{r})$ agents \\ (Theorem~\ref{thm:non_fsd}) \end{tabular}
     & \begin{tabular}{@{}c@{}}
     $\Omega(r^{-1/8})$ agents\\ (\Cref{thm:non_fsd_lb_intro})
     \end{tabular} \\
    \hline
    no assumption & -- & -- & \withincell{any finite number \\ \cite[Proposition~3.4]{BabaioffGG20}}\\
    \hline
    \end{tabular}
    }
    \caption{Summary of our main results. The upper bounds state the number of additional agents suffices for a prior-independent mechanism (BTR or STR) to achieve GFT at least the first best. The lower bounds state the number of additional agents necessary for any anonymous and deterministic mechanism. Results with ``buyer'' listed indicate that only buyers can be augmented to the market.}\label{table:results}
\end{table}


\begin{theorem}
\label{thm:main_str}
Consider the double auction with $m$ i.i.d.~buyers and $n$ i.i.d.~sellers. Suppose $m\geq n$ and the buyers' distribution $F_B$ first-order stochastically dominates the sellers' distribution $F_S$. Then there is a global constant integer $c>0$ 
such that 
the GFT of STR with $m+c$ buyers and $n+c$ sellers 
is at least the first-best GFT with $m$ buyers and $n$ sellers.
\end{theorem}
\begin{remark}\label{remark:mn_assumption}
While Theorem~\ref{thm:main_str} assumes that $m \geq n$, the result applies analogously to the case where $m\leq n$ using Buyer Trade Reduction, by negating the values/costs and swapping the role of buyers and sellers. See \cite[Proposition~A.1]{BabaioffGG20}.
%one can also handle the case where $m \leq n$ using Buyer Trade Reduction instead (see \cite[Proposition~A.1]{BabaioffGG20}).
\end{remark}

Since the welfare of any mechanism is the GFT plus the sum of the seller values, our results immediately apply to the welfare objective, as the sum of seller values in the augmented market is at least the one in the original market.

\begin{corollary}
\label{cor:main_str}
Consider the double auction with $m$ i.i.d. buyers and $n$ i.i.d. sellers. Suppose $m\geq n$ and the buyers' distribution $F_B$ first-order stochastically dominates the sellers' distribution $F_S$. Then there is a global constant integer $c>0$ 
such that 
the \emph{welfare} of STR with $m+c$ buyers and $n+c$ sellers 
is at least the welfare of the optimal allocation with $m$ buyers and $n$ sellers.
\end{corollary}

%\mingfei{Define the optimal trade size, first best in the following paragraph.}

Notice that STR loses no more than a single trade from the first-best allocation in the augmented market.
%Since STR loses no more than a single trade, 
Thus a natural (but erroneous) starting point to prove Theorem~\ref{thm:main_str} may be to (i) show that with only a constant number of new buyers and new sellers, at least one of the new buyers is eligible to trade with a new seller and (ii) show that if there is a trade between a new buyer and a new seller then the trade size must increase by $1$ and thus STR performs at least as well as OPT.
If the second statement were true then the proof should be relatively straightforward since the first statement happens with fairly high probability due to the stochastic dominance assumption. Unfortunately, the second statement is false and thus the first statement is not a sufficient condition for STR to outperform OPT. Indeed, consider the following example, which is also depicted in Figure~\ref{figure:str_lose_trade}.
Let $\eps > 0$.
There are $3$ original buyers with values $\oldb_1 = 3, \oldb_2 = 2+\eps, \oldb_3 = 2$ and $3$ original sellers all with value $\olds_1 = \olds_2 = \olds_3 = 1$.
The original optimal GFT is $4 + \eps$.
Now, suppose we add a new buyer with value $\newb = 2+3\eps$ and a new seller with value $\news = 2 + 2\eps$.
Note that $\newb$ and $\news$ are eligible to trade with each other.
The new optimal matching matches $\oldb_1, \newb, \oldb_2$ with $\olds_1, \olds_2, \olds_3$.
STR checks if $\news$ is able to price the buyers and the sellers; in this case it has higher value than $\oldb_2$.
Thus, STR removes $\oldb_2$ and $\olds_3$ (say) and matches only $\oldb_1, \newb$ with $\olds_1, \olds_2$ for a GFT of $3 + 3\eps$.
This is strictly worse than the original GFT if $\eps < 1/2$.
Note that a similar example could be possible even if there are multiple trades among the new agents.
\begin{figure}[ht]
\begin{center}
\resizebox{200pt}{!}{%
\input{figures/str_lose_trade.tex}
}
\end{center}
\caption{This figure illustrates an example where the the new agents can trade yet incorporating them with the original agents causes STR to lose a trade. In the figure, \textcolor{blue}{original agents} are depicted with \textcolor{blue}{blue circles} and \textcolor{red}{new agents} are depicted with \textcolor{red}{red squares}. The figure on the left depicts the original market and the figure on the right depicts the augmented market.}
\label{figure:str_lose_trade}
\end{figure}

The message in the previous paragraph is that having additional trades among the new agents is not sufficient to guarantee that the optimal trade size increases. We would like to find an event such that the optimal trade size increases, which is sufficient for STR to outperforms OPT.
Naively, we could simply consider the event where the optimal trade size does increase.
However, the difficulty is in being able to lower bound the gain of the expected GFT restricted to this event and compare that with the loss of the expected GFT when this does not happen.
In order to make the analysis more feasible, we consider more structured events that (i) make it possible to analyze the gain or loss in GFT and (ii) we can compare the probabilities of these events.

In order to make the argument formal, we utilize a coupling argument that was also used by \citet{BabaioffGG20}.
In particular, we first \emph{fix} a set of quantiles and then assign these quantiles uniformly at random to the new and original buyers and sellers.
However, the techniques in our paper and \citet{BabaioffGG20} are otherwise very different.
\citet{BabaioffGG20} first consider the single seller and $m$ buyers setting and proceed by showing that by adding a sufficient number of buyers it must be that (i) the GFT difference between the new and original optimal allocations is large and (ii) the GFT difference between the new optimal allocation and BTR is small.
The only way for this to be possible is that the GFT of BTR must be large compared to the original optimal allocation.
To handle the case with an arbitrary number of sellers, they show that they can reduce the problem to the single seller case but this reduction incurs a linear overhead (in the number of sellers).
In contrast, our argument directly compares the GFT difference between STR and OPT and show that this difference is net positive.

Finally, we consider general distributions that may not satisfy the FSD condition. Existing hardness results show that no finite bound applies to any pair of distributions even for the single seller case~\cite{BabaioffGG20}. Instead we prove a parameterized result using the parameter $r = \probs{b \sim F_B, s \sim F_S}{b \geq s} \in (0,1)$. Intuitively, $r$ indicates how much the buyer distribution overlap with the seller distribution.
\begin{theorem}
\label{thm:non_fsd}
Consider the double auction with $m$ i.i.d.~buyers and $n$ i.i.d.~sellers. Suppose $m\geq n$ and that $\probs{b \sim F_B, s \sim F_S}{b \geq s} = r$.
Then there exists $c = O((\log(m/n) + \log(1/r)) / r)$ such that
the GFT of STR with $m+c$ buyers and $n+c$ sellers 
is at least the first-best GFT with $m$ buyers and $n$ sellers.
\end{theorem}

When $m/n = O(1/r)$ (for example, if $m = n$) then \Cref{thm:non_fsd} implies an $O(\log(1/r) / r)$ upper bound. When $F_B$ FSD $F_S$, then the median of the buyer's value exceeds the median of the seller's value. This implies that $r=\prob{b \geq s} \geq 1/4$. However, in this case \Cref{thm:non_fsd} gives an upper bound of $O(\log(m/n))$ which does not fully match \Cref{thm:main_str}. {It remains an interesting open question whether the dependency on $m,n$ can be removed in \Cref{thm:non_fsd} so that the result generalizes the FSD case.}

The techniques used to prove \Cref{thm:non_fsd} differs from the techniques for \Cref{thm:main_str} in the following way.
In \Cref{thm:non_fsd} we prove that STR has GFT at least OPT for every fixed set of quantiles,
with the expectation only taken over the random assignment from the quantiles to the agents.
However this approach is unlikely to work in this general case since it is possible that we are unlucky with the realization of the quantiles.
Instead we bound the expected GFT difference over the randomness of the quantiles as well.

To complement \Cref{thm:non_fsd}, we also prove a lower bound that a polynomial dependency on $1/r$ is required, using the result in \cite{BabaioffGG20}.
A proof can be found in Appendix~\ref{subsec:non_fsd_lb}.
\begin{theorem}[{Adapted from \cite[Proposition~3.4]{BabaioffGG20}}]
\label{thm:non_fsd_lb_intro}
For any sufficiently small $r\in (0,1)$, there exists a double auction instance with $\Pr_{b\sim F_B, s\sim F_S}[b\geq s]=r$ such that: For any $c\leq \frac{1}{4}\cdot r^{-1/8}$ and any deterministic, prior-independent, BIC, IR, BB and anonymous mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than the first-best GFT on $m$ buyers and $n$ sellers.
\end{theorem}


\comment{
% does not imply that the optimal trade size increases.
% The issue in the previous example is that even though the new buyer and new seller could trade, including them with the original buyers and sellers causes the new buyer to ``steal'' an original trade.
% This means that the size of the optimal trade in the augmented market remains the same and STR could potentially have a trade size that is one smaller than this.
% which causes the size of optimal trade in the augmented market to remain the same and thus STR has one less trade.
%while causing us to lose a trade since we are using STR.
To get around this issue, it is helpful to find a more structured event that ensures 
% that when we do have a trade among a new buyer and a new seller,
that including new agents increases the trade size of the optimal matching, and so that it can offset the loss of GFT in the event where STR has a smaller trade size than OPT.
% Note that STR loses at most one trade and therefore the GFT of STR is at least that of OPT in this case.
% To ensure that STR is strictly better than OPT, we need to offset the loss of GFT in the event where STR has a smaller trade size than OPT.
\todo{We can mention here that there is a tension between defining high probability good events and being able to lower bound the condition mean of the gain of this event. E.g.~take $\cE_1$ to be the event where we increase the trade size by $2$. Hard to estimate.}
\todo{Actually, tension may not be super clear to the reader. We can say that if we define naive events then we cannot get a good understanding of the conditional mean. So we need to define more structured events.
}
For this reason, we consider an event that increases the trade size by at least two.
To make this formal, we construct a ``good'' event $\cE_1$ where STR outperforms
% While the previous paragraph suggests how we might come up with a way to obtain strictly more trades with STR than in OPT,
% one still needs to quantitatively bound the GFT when STR performs better than OPT and show that this offsets the loss of GFT when STR performs worse than OPT.
% A key insight in our proof is to craft a ``good'' event $\cE_1$ where STR outperforms
OPT by at least $C$ (in expectation) and a ``bad'' event $\cE_2$ where STR underperforms OPT by at most $C$ (in expectation).
For the good event $\cE_1$, one naive definition is to define it as the event that the optimal trade size increases by two. However, it is difficult to understand the structure of this event and provide a good quantitative lower bound on the conditional expectation of the increase in GFT.
Instead, we define a more structured event $\cE_1$ 

For the good event $\cE_1$, we ensure that (i) at least two new buyers have value which is greater than the value of some originally traded buyer and (ii) at least two new sellers have value which is less than the value of some originally traded seller.
As we show, this is sufficient for the optimal trade size to increase by two.
We then define the event $\cE_2$ such that it is a necessary condition for STR to have a smaller trade size than OPT.
An obvious choice is to define $\cE_2$ as $\overline{\cE_1}$.
When $n \approx m$, we can show that $\prob{\cE_1} \geq 1/2$.
Therefore, this definition of $\cE_2$ is sufficient for our purposes.
However, when $n \ll m$, $\prob{\cE_1} \ll 1/2$ and thus, $\overline{\cE_1}$ is too large of an event.
Roughly speaking, we choose $\cE_2$ so that all the new sellers have value which is larger than the lowest value originally traded buyer.

\chris{Mention the contention between probability and gain.}

When $n \approx m$, this is a fairly high probability event since 

In this case, we define $\cE_2$ as the event where the value of all the new sellers are among the top $2n$ agent values.
We show that outside of this event, STR performs at least as well OPT.
When $n \approx m$, this is a trivial event but when $n \ll m$, this event is very small.

However, we can make this event smaller by also enforcing that most 

The bad event $\cE_2$ is that all the new sellers have very high value.
We show that if even one seller does not have too large of a value then STR performs at 

Simultaneously, we will guarantee that $\prob{\cE_1} \geq \prob{\cE_2}$.



% \textcolor{red}{Comments below.}

% 1. Uber example
% 2. Welfare vs. GFT

% Mention that a technical difficulty is that it is \emph{not} sufficient that to just have additional possible trades.

% Condition 1: The intuition is that we get a new buyer and a new seller that is able to trade. Intuitively, this is sufficient. However, it turns out that this is \emph{not} sufficient.

% Condition 2: Even if we do gain one more trade, we have to be careful since it is not clear that this additional gain will recover the loss when we do lose the trade.

% Mention some roadblocks with the analysis of using trade reduction vs seller trade reduction.

% A few questions:
% - Could you do this with just augmenting the smaller side by a constant number?
% % - For $(m, \Theta(m))$ case in Babaioff, did they really need

% Intuition is that only one additional trade is needed as long as neither side is saturated.
% This is true for $(m, m)$ case and if this intuition is true then we ought to be able to only augment one side of the market.
% But even here, best upper bound is $O(m^2)$ due to Yannai.
}

==> zz_non_fsd_apr3.tex <==
%\section{$O(\log(m / rn) / r)$ upper bound for $r$ overlapping distributions}
\section{A Parameterized Upper Bound for General Distributions}
\label{sec:non_fsd}
In this section, we get rid of the stochastic dominance assumption and prove Theorem~\ref{thm:non_fsd}. It is known that no finite bound applies to any pair of distributions even at the single seller case~\cite{BabaioffGG20}. Instead we prove a parameterized upper bound on the parameter $r = \probs{b \sim F_B, s \sim F_S}{b \geq s} \in (0,1)$. %$r$ depends on both distributions and indicates
%we refer to this as the $r$-overlap setting.
% Our main result in this section is the following theorem.
% \begin{theorem}
%     \label{thm:non_fsd}
%     Suppose $m\geq n$ and let $r=\probs{b \sim F_B, s \sim F_S}{b \geq s}$.
%     %For every $m \geq n$, there exists $c = O(\log(m / rn) / r)$ such that
%     There exists $c = O(\frac{\log(m/n)+\log(1/r)}{r})$ such that
%     \[
%         \STR(m+c, n+c) \geq \OPT(m, n). 
%     \]
% \end{theorem}

%\chris{Moved remark to intro.}
% \begin{remark}\label{remark:non_fsd}
% Here are some remarks from \Cref{thm:non_fsd}:

% 1. When $\frac{m}{n}=O(1/r)$ (we notice that $n=m$ belongs to this case), then \Cref{thm:non_fsd} implies an $O(\frac{1}{r}\cdot \log(\frac{1}{r}))$ upper bound.

% 2. We notice that the assumption of $F_B$ FSD $F_S$ implies that $r\geq\frac{1}{4}$ as $b(\frac{1}{2})\geq s(\frac{1}{2})$. However, the upper bound from \Cref{thm:non_fsd} in this case is $O(\log(m/n))$, which does not fully match the result in \Cref{thm:str_main}.
% \end{remark}


In \Cref{sec:str}, we crucially made use of stochastic dominance in many parts of the proof, i.e.~$b(q) \geq s(q)$ for every $q$. While the stochastic dominance is no longer satisfied, the following lemma is useful to prove our result. It indicates that the trade is available as long as the buyer is at a high quantile and seller is at a low quantile. 
%the following observation suggests that we still have a property that has a similar flavor as stochastic dominance.
\begin{lemma}[{\cite[Lemma~3.1]{CaiGMZ21}}]
    \label{lemma:r_fsd}
    For any distribution $F_B$ and $F_S$, let $r=\probs{b \sim F_B, s \sim F_S}{b \geq s}$.
    Then $b(1-r/2) \geq s(r/2)$.
\end{lemma}
Unlike the previous section, we can no longer use an argument that fixes the quantiles a priori and then simply consider random assignments of these quantiles.
For example, we could unlucky and draw quantiles such that, in expectation over the random assignments, OPT has positive GFT while STR never trades (and thus, has GFT equal to $0$).
For this reason, we cannot condition on the realization of the quantiles and instead consider the follow process to assign quantiles.
% we draw quantiles slightly differently than in Section~\ref{sec:str} (although they are still uniform at random).
First, we draw $m$ quantiles $\qbo(1), \ldots, \qbo(m)$ uniformly at random from $[0, 1]$ ordered such that $\qbo(1) \geq \ldots \geq \qbo(m)$.
Similarly, we draw $c$ quantiles $\qbn(1), \ldots, \qbn(c)$ uniformly at random from $[0, 1]$ ordered such that $\qbn(1) \geq \ldots \geq \qbn(c)$.
We repeat this for the sellers except that we order the quantiles such that $\qso(1) \leq \ldots \qso(n)$ and $\qsn(1) \leq \ldots \leq \qsn(c)$.
Finally, we let $\qb(1) \geq \ldots \geq \qb(m+c)$ be all the buyer quantiles
and $\qs(1) \leq \ldots \leq \qs(n+c)$ be all the seller quantiles.
We also let $\Bq$ be a vector with all the quantiles.

We let $\Bold = \{\qbo(1), \ldots, \qbo(m)\}$, $\Bnew = \{\qbn(1), \ldots, \qbn(c)\}$, $\Sold = \{\qso(1), \ldots \qso(n)\}$ and $\Snew = \{\qsn(1), \ldots, \qsn(c)\}$.
We also let $Q = \Bold \cup \Bnew \cup \Sold \cup \Snew$ denote the set of all quantiles.
Let $p = r n / 100 m$.
Next, for $k \geq 1$, we define the intervals
\begin{equation}
    I_k = \left( 1 - kp, 1-(k-1)p \right]
    \quad\text{and}\quad
    J_k = \left[ (k-1)p, kp \right)
\end{equation}
We also define $I_{\leq k} = \cup_{\ell=1}^k I_{\ell}$ and $J_{\leq k} = \cup_{\ell=1}^k J_{\ell}$.
Note that, as in Section~\ref{sec:str}, $I_k$ correspond to high quantile, high value buyers and $J_k$ correspond to low quantile, low value buyers.

% The proof of Theorem~\ref{thm:non_fsd} follows fairly straightforwardly from the following two lemmas.
% \begin{restatable}{lemma}{lemmacontbign}
%     \label{lemma:cont_big_n}
%     Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
%     Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
%     Then
%     \[
%         \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
%     \]
% \end{restatable}

The remainder of this section is structured as follows.
Subsection~\ref{subsec:defining_events} defines the various events we utilize to prove Theorem~\ref{thm:non_fsd}.
Two of the events are nearly identical to the events used in Section~\ref{sec:str} but we require one additional event that shows that each interval
contains roughly the ``right'' number of agents.
Subsection~\ref{subsec:cont_prob} analyzes the increase of GFT by using STR in the augmented market compared with OPT in the original market.
Finally, in Subsection~\ref{subsec:proof_non_fsd}, we summarize the arguments and prove Theorem~\ref{thm:non_fsd}.

\subsection{Constructing the Events}
\label{subsec:defining_events}
In this section, we define and analyze the events that we utilize to prove Theorem~\ref{thm:non_fsd}.

\paragraph{The event $\cE_3$.}
Define the event $\cE_3$ as the event that
\begin{equation}
\label{eqn:contE3def}
\begin{aligned}
    \cE_3 = \{
    & |I_{\leq 2} \cap \Bold| \leq 4pm,
    |(1-r/2, 1] \cap \Bold| \geq r n / 4, \\
    & |J_{\leq 2} \cap \Sold| \leq 4pm,
    |[0, r/2) \cap \Sold| \geq r n / 4
    \}
\end{aligned}
\end{equation}
At a high-level, we should think of $\cE_3$ as the event that each interval contains roughly the right number of original buyers and original sellers.
We require the following fact which will be used repeatedly.
\begin{claim}
    \label{claim:non_fsd_orig_matched}
    Condition on event $\cE_3$.
    In the original first-best matching, every original buyer in $I_{\leq 2}$ is matched
    and every original seller in $J_{\leq 2}$ is matched.
    Furthermore, in the augmented first-best matching, every buyer in $I_{\leq 2}$ is matched and every seller in $J_{\leq 2}$ is matched.
\end{claim}
\begin{proof}
    First, we prove that every original buyer in $I_{\leq 2}$ is matched.
    Let $k = |I_{\leq 2} \cap \Bold|$ be the number of original buyers in $I_{\leq 2}$.
    Note that $k \leq 4pm = 4 r n / 100 < r n / 4$, where the first inequality is by definition of $\cE_3$ (see Eq.~\eqref{eqn:contE3def}).
    Using the definition of event $\cE_3$ again, since $|(1-r/2, 1] \cap \Bold| \geq r m / 4$ and $|[0, r/2) \cap \Sold| \geq r n / 4$, we must have $\qbo(k) \geq 1 - r/2$ and $\qso(k) \leq r / 2$.
    By Lemma~\ref{lemma:r_fsd}, $b(\qbo(k)) \geq b(1-r/2) \geq s(r/2) \geq s(\qso(k))$ and thus every original buyer in $I_{\leq 2}$ is matched.

    The proof for the sellers is similar.
    Let $t = |J_{\leq 2} \cap \Sold|$ be the number of original sellers in $J_{\leq 2}$.
    When $\cE_3$ happens, we have $t \leq 4pm = 4 r n / 100 < r n / 4$.
    Following the identical logic above, we conclude that $s(\qso(t)) \leq s(r/2)\leq b(1-r/2) \leq b(\qbo(t))$ and thus every original seller in $J_{\leq 2}$ is matched.
    This proves the first assertion.

    The proof for the second assertion is nearly identical and is omitted.
\end{proof}


The following lemma shows that $\cE_3$ happens with high probability.
\begin{lemma}
    \label{lemma:cont_probE3_bound}
    $\prob{\cE_3} \geq 1 - 4\exp\left( -rn/300 \right)$.
\end{lemma}
\begin{proof}
    Since $|I_{\leq 2} \cap \Bold|$ can be written as a sum of i.i.d.~random variables and $\expect{|I_{\leq2} \cap \Bold|} = 2pm$,
    an application of the Chernoff Bound (see Lemma~\ref{lemma:chernoff}) gives
    \[
        \prob{|J_{\leq 2} \cap \Sold| \geq 4pm}
        \leq
        \prob{|I_{\leq 2} \cap \Bold| \geq 4pm} 
        \leq \exp\left( - pm / 3 \right)=\exp(-rn/300).
    \]
    Next, $\expect{|[0, r/2) \cap \Sold|} = rn/2$.
    So
    \[
        \prob{|(1-r/2, 1] \cap \Bold| \leq rn/4}
        \leq \prob{|[0, r/2) \cap \Sold| \leq rn/4}
        \leq \exp\left( - rn / 24 \right).
    \]
    % Similarly,
    % \[
    %     \prob{|[0, r/2) \cap \Sold| \leq rn/4} = \exp\left( -r^2 n / 2 \right).
    % \]
    By union bound we conclude that $\prob{\neg\cE_3} \leq 4 \exp\left( - rn / 300 \right)$.
    %The lemma follows by taking a complement.
\end{proof}
%\mingfei{One minor thing I changed: use $\neg \cE$ for the complement instead of $\overline{\cE}$ as the line connects with the brackets in the prob, e.g. $\prob{\overline{\cE}}$. }
%\chris{Sounds good. We can change it everywhere to be consistent.}

The following lemma bounds the loss on the GFT when the event $\cE_3$ is not satisfied. We denote $q_B\sim I_1$ the random variable $q_B$ drawn uniformly at random from the interval $I_1$. Similarly for $q_S\sim J_1$.
\begin{lemma}\label{lemma:expectation_E3}
    We have that
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq 4m \cdot \exp\left(- rn / 300 \right) \cdot
        \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    In particular, for any $\eta\in (0,1)$, if $n \geq \frac{300 \log(4m / \eta)}{r}$ then
    \[
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}} \leq \eta \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
    We write
    \begin{align*}
        \expect{(\OPT(\Bq) - \STR(\Bq)) \cdot \ind{\Bq\not\in \cE_3}}
        & = \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}.
    \end{align*}
    Note that $\OPT(\Bq) - \STR(\Bq) \leq (\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qbo(j))\})_+$.
    \chrisnote{For the proof, we consider the following process to generate random uniform quantiles.
    First, for every agent, we assign them the label $1$ with probability $p$, the label $2$ with probability $p$, the label $3$ with probability $r/2 - 2p > 0$, and the label $4$ with the remaining probability. Note that the event $\neg \cE_3$ is defined via these labels. For example, the event that $|I_{\leq 2} \cap \Bold| \leq 4pm$ is the event that at most $4pm$ original buyers have the label $1$ or $2$.
    For the second step, we assign quantiles as follows.
    \begin{enumerate}[itemsep=0pt, topsep=0pt]
        \item Every buyer with label $1$ is assigned a uniform random quantile from $I_1$.
        \item Every buyer with label $2$ is assigned a uniform random quantile from $I_2$.
        \item Every buyer with label $3$ is assigned a uniform random quantile from $(1-r/2, 1] \setminus I_{\leq 2}$.
        \item Every buyer with label $4$ is assigned a uniform random quantile from $[0, 1-r/2]$.
    \end{enumerate}
    The sellers are assigned quantiles in an analogous manner. Note that each agent receives a uniformly random quantile.}
    
    \chrisnote{We claim that the random variable $\max_{i \in [m]}\{b(\qbo(i))\}$ is first-order stochastically dominated by the random variable $\max_{i \in [m]} \{b(\qb'(i))\}$ where $\qb'(1), \ldots, \qb'(m) \sim I_{1}$ uniformly at random. Indeed, fix any labelling as described above. If $k = 0$ then the stochastic-dominance is trivial. Otherwise, conditioned on $k\geq 1$ original buyers with the label $1$, we know that}
    \[
        \max_{i \in [m]} \{b(\qbo(i))\} \stackrel{d}{=} \max_{i \in [k]} \{b(\qb'(i)\} \stackrel{d}{\leq} \max_{i \in [m]}\{b(\qb'(i))\},
    \]
    \chrisnote{where we used $\stackrel{d}{=}$ to denote equal in distribution and $\stackrel{d}{\leq}$ to denote first-order stochastic dominance. As the stochastic dominance is true for every labelling, it follows that $\max_{i \in [m]} \{b(\qbo(i)\}$, conditioned on $\neg \cE_3$, is first-order stochastically dominated by $\max_{i \in [m]} \{b(\qb'(i))\}$.
    By an analogous argument, and since $m \geq n$, conditioned on $\neg \cE_3$, we can show that $-\min_{j \in [n]} \{s(\qso(j)\}$ is first-order stochastically dominated by $-\max_{j \in [m]} \{s(\qs'(j)\}$ where $\qs'(1), \ldots, \qs'(m) \sim J_{1}$ uniformly at random.}
    
    Thus, we have
    \begin{align*}
        \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3}
        & = \expectg{\max_{i \in [m]} \{b(\qbo(i))\} - \min_{j \in [n]} \{s(\qso(j))\} }{\neg \cE_3} \\
        & \leq \expect{\max_{i \in [m]} \{b(\qb'(i))\} - \min_{j \in [m]} \{s(\qs'(j))\} } \\
        & \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}
    \end{align*}
    % We observe that, conditioned on $\cE_3$, $\OPT(\Bq) - \STR(\Bq)$ is first-order stochastically dominated by the random variable $\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}$ where $\qb'(i) \sim I_1$ (resp.~$\qs'(j) \sim J_1$) i.i.d.~and uniformly at random.
    % Let $\Bq'$ denote these auxiliary quantiles.
    % We thus have
    % \[
    %     \expectg{\OPT(\Bq) - \STR(\Bq)}{\neg \cE_3} \leq
    %     \expects{\Bq'}{\max\{b(\qb'(i))\}_{i \in [m]} - \min\{s(\qs'(j))\}_{j \in [m]}}
    %     \leq m \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    % \]
    Combining the inequality with Lemma~\ref{lemma:cont_probE3_bound} completes the proof.
\end{proof}

It remains to lower bound the GFT difference $\STR(\Bq)-\OPT(\Bq)$ when $\cE_3$ is satisfied. Similar to \Cref{sec:str}, we construct the following two events.

\paragraph{The good event $\cE_1$.}
Define $\cE_1$ as
\[
    \cE_1 = \{ \Bq : |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_1 \cap \Snew| \geq 2, |J_2 \cap \Sold| \geq 1 \}.
\]
We prove that $\cE_1\cap \cE_3$ is a sufficient condition for $\STR(\Bq)\geq \STR(\Bq)$. Moreover, we prove a lower bound on the expected GFT increase conditioned on $\cE_1\cap \cE_3$.
%on the event $\cE_1 \cap \cE_3$, we can obtain a strong lower bound on the GFT increase.
\begin{lemma}
    \label{lemma:cont_E1_lb}
    For any $\Bq \in \cE_1\cap \cE_3$, $\STR(\Bq) \geq \OPT(\Bq)$.
    Moreover,
    \[
        \expectsg{\Bq}{\STR(\Bq) - \OPT(\Bq)}{\cE_1\cap \cE_3} \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
\end{lemma}
\begin{proof}
Let $T$ be the number of trades in the original first-best matching.
We prove in the following claim that when $\cE_1\cap \cE_3$ happens, there are at least $T + 2$ trades in the augmented first-best matching.
\begin{claim}
    Recall that $\qbn(2)$ is the quantile of the second-highest new buyer and $\qsn(2)$ is the quantile of the second-lowest new seller. For any $\Bq\in \cE_1$, $b(\qbn(2)) \geq b(\qb(T+2)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
\end{claim}
\begin{proof}
    Let $\qb' \in I_2 \cap \Bold$ be the index of any original buyer in $I_2$ (by definition of $\cE_1$ there is at least one).
    By Claim~\ref{claim:non_fsd_orig_matched}, we have $\qb' \geq \qbo(T)$ (the buyer corresponding to quantile $\qb'$ is matched).
    On the event $\cE_1$, we have $|I_1 \cap \Bnew| \geq 2$ and thus $\qbn(2) \geq \qb' \geq \qbo(T)$.
    Therefore, $\qbn(2) \geq \qb(T+2) \geq \qbo(T)$ as both the highest and second-highest new buyer have quantile no less than $\qbo(T)$.
    A similar argument shows that $\qsn(2) \leq \qs(T+2) \leq \qso(T)$.
    We conclude that $b(\qbn(2)) \geq b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+2)) \geq s(\qsn(2))$.
    Here the first inequality follows from the fact that there are $T$ trades in the original first-best matching.
\end{proof}
Recall that that $\STR(\Bq) \geq \sum_{t=1}^{T+1} b(\qb(t)) - s(\qs(t))$
and $\OPT(\Bq) = \sum_{t=1}^T b(\qbo(t)) - s(\qso(t))$.
Since $\{\qb(1), \ldots, \qb(T+1)\} \setminus \{\qbn(1)\}$ consists of the top $T$ buyer quantiles except the highest \emph{new} buyer quantile and $\{\qbo(1), \ldots, \qbo(T)\}$ consist only of the top $T$ \emph{original} buyer quantiles, we have $\sum_{t=1}^{T+1} b(\qb(t)) - b(\qbn(1)) \geq \sum_{t=1}^T \qbo(t)$.
By a similar argument, we have $\sum_{t=1}^{T+1} s(\qs(t)) - b(\qsn(1)) \leq \sum_{t=1}^T \qso(t)$,
whence $\STR(\Bq) - \OPT(\Bq) \geq b(\qbn(1)) - s(\qsn(1))$.

Finally, we check that $\expectg{b(q(\inew_1))}{\cE_1\cap \cE_3} \geq \expects{\qb \sim I_1}{b(\qb)}$ (and analogously for the seller).
Note that if $\qb \sim I_1$ uniformly at random then $\qbn(1)$, conditioned on $|I_1 \cap \Bnew| \geq 2$, FSD $\qb$.
In addition, since the random variables $\qbn(1)$ and $|I_1 \cap \Bnew|$ are independent of the events $\cE_3$ and the random variables $|I_2 \cap \Bold|$, $|J_1 \cap \Snew|$ and $|J_2 \cap \Sold|$, we have
\[
    \expectg{b(\qbn(1))}{\cE_1\cap \cE_3} = \expectg{b(\qbn(1))}{|I_1 \cap \Bnew| \geq 2} \geq \expects{\qb \sim I_1}{b(\qb)}.
\]
A similar argument gives that $\expectg{s(\qsn(1))}{\cE_1\cap \cE_3} \leq \expects{\qs \sim J_1}{s(\qs)}$.
\end{proof}

% \chris{For the following, I think we need one more condition which is that there are at least $n+c$ buyers in the interval $[0, 2n/m]$.}
\paragraph{The bad event $\cE_2$.}
We define the bad event
\[
    \cE_2 = \neg\cE_1 \cap (\{ \Snew \cap (r/2, 1] = \Snew \} \cup \{ |\Bold \cap (1-r/2, 1]| < n + c\})
\]
In other words, the event requires that: (1) $\cE_1$ does not happen; (2) either every new seller has quantile in $(r/2, 1]$, or there are at least $n+c$ old buyers with quantile in $(1-r/2, 1]$. 
%all the new sellers are in the top $\gamma$ quantiles.
\begin{lemma}
    \label{lemma:contNotE2Better}
    % Meant to be a version of Lemma~\ref{lemma:notE2_STR_gt_OPT}.
    For any $\Bq \in \cE_3\cap \neg\cE_2$, we have $\STR(\Bq) \geq \OPT(\Bq)$.
\end{lemma}
\begin{proof}
    If $\Bq \in \cE_3$ but $\Bq \in \cE_1$ then we know from Lemma~\ref{lemma:cont_E1_lb} that $\STR(\Bq) \geq \OPT(\Bq)$.
    It remains to check that if $\Bq \in \cE_3 \cap \{\Snew \cap (1-\gamma, 1] \neq \Snew\} \cap \{|\Bold \cap (1-r/2, 1]| \geq n+c\}$ then $\STR(\Bq) \geq \OPT(\Bq)$.
    Let $\OPT'(\Bq)$ be the first-best matching in the augmented market.
    Suppose that $\OPT(\Bq)$ has $T \leq n$ trades.
    We consider two cases, depending on the number of trades in $\OPT'(\Bq)$.

    \paragraph{Case 1: $\OPT'(\Bq)$ has $T+1$ trades.}
    In this case, $\STR(\Bq)$ trades the top $T$ highest value (original and new) buyers and the bottom $T$ lowest value (original and new) sellers (but it could trade more). In particular, $\STR(\Bq) \geq \OPT(\Bq)$.

    \paragraph{Case 2: $\OPT'(\Bq)$ has $T$ trades.}
    Here, we want to show that $\STR(\Bq) = \OPT'(\Bq)$.
    By definition of STR, it suffices to show that $b(q(T)) \geq s(q(T+1))$.
    We claim that $\qso(T) > r/2$.
    For the sake of contradiction, suppose that $\qso(T) \leq r/2$.
    Since $\Bq \in \{\Snew \cap (r/2, 1] \neq \Snew\}$, this implies that $\qsn(1) \leq r/2$.
    But this means $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} \leq r/2$.
    However, since $|\Bold \cap (1-r/2, 1]| \geq n+c$ and $T \leq n$, it must be that $\qb(T+1) \geq \qbo(T+1) \geq 1-r/2$.
    But then by Lemma~\ref{lemma:r_fsd}, we would have $b(\qb(T+1)) \geq s(\qs(T+1))$ contradicting that $\OPT'(\Bq)$ has $T$ trades.
    We thus conclude that $\qso(T) > r/2$.
    
    To finish the proof, we have
    \[
        b(\qb(T)) \geq b(\qbo(T)) \geq s(\qso(T)) \geq s(\qs(T+1)). 
    \]
    The first inequality is because $\qb(T) \geq \qbo(T)$.
    The second inequality follows from the fact that $\OPT$ has $T$ trades.
    The last inequality holds because $\qs(T+1) \leq \max\{\qsn(1), \qso(T)\} = \qso(T)$ since $\qsn(1) \leq r/2 < \qso(T)$.
\end{proof}

\begin{lemma}
\label{lemma:cont_bound_loss_E2}
We have $\expectsg{\Bq}{\OPT(\Bq) - \STR(\Bq)}{\cE_2\cap \cE_3} \leq \expects{\qb \sim I_1, \qs \sim J_1}{b(\qb) - s(\qs)}$.
\end{lemma}
\begin{proof}
    Let $\OPT'(\Bq)$ be the GFT of the first-best matching in the augmented market.
    Let $b^*(\Bq)$ (resp.~$s^*(\Bq)$) denote the lowest (resp.~highest) value among buyers (resp.~sellers) traded in the augmented first-best matching.
    Let $\cF$ be the event that there is no trade in the first-best matching in the augmented market and let $b^*(\Bq) = 0$ and $s^*(\Bq) = 0$ if no trade exists in $\OPT'(\Bq)$.
    By definition of the STR mechanism, we have $\OPT(\Bq) - \STR(\Bq) \leq \OPT'(\Bq) - \STR(\Bq)\leq (b^*(\Bq)-s^*(\Bq)) \cdot \ind{\cF}$.

    We will show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \leq \expects{q_B \sim I_1}{b(\qb)}$. An analogous argument can be used to show that $\expectg{s^*(\Bq) \ind{\cF}}{\cE_2\cap \cE_3} \geq \expects{\Bs \sim J_1}{s(\qs)}$.
    We consider three cases.
    
    \chrisnote{Note that for the proof, we will make use of the following two-stage process to sample $\Bq$, which we describe only for the buyers (the sellers' description is analogous).
    First, we assign original and new buyers with two labels.
    For the first label, we assign them a label in $\{1, \ldots, \lceil 1/p \rceil\}$ where label $\ell \in [\lceil 1/ p \rceil]$
    is assigned with probability equal $\mu(I_\ell \cap [0, 1])$. Here $\mu$ denotes the Lebesgue measure.
    For the second label, if the first label is $\ell$ then we assign the second label $1$ with probability $\mu(I_{\ell} \cap (1-r/2, 1]) / \mu(I_{\ell})$ and $0$ otherwise.
    Note that except for one label $\ell'$ all labels $\ell \neq \ell'$ result in second labels having probability either $1$ or $0$.
    In particular, the label $(1,0)$ occurs with probability $0$ since $I_1 \cap (1-r/2, 1] = I_1$.
    For the second-stage, if a buyer is assigned the label $(\ell, 1)$ then we assign it a uniform random quantile from $(1-r/2, 1] \cap I_{\ell}$ and if it is assigned the label $(\ell, 0)$ then we assign it a uniform random quantile from $[0, 1-r/2) \cap I_{\ell}$.
    Note that with this process, every buyer is assigned a uniform random quantile from $[0, 1]$.}
    
    \chrisnote{Given this process, it is straightforward to maps the events $\cE_2, \cE_3$ to description about labels.
    For example, the event $|I_{\leq 2} \cap \Bold| \leq 4pm$ is equivalent to the event that at most $4pm$ original buyers are assigned a first label of $1$ or $2$ and the event $|(1-r/2, 1] \cap \Bold| \geq rn/4$ is equivalent to the event at least $rn/4$ original buyers are assigned a second label of $1$.}

    \paragraph{Case 1: $|I_1 \cap \Bnew| \geq 1$.}
    Let $\cE' = \{ |I_1 \cap \Bnew| \geq 1 \}$. \chrisnote{This is equivalent to the event that at least one new buyer is assigned a first label of $1$ in the above two-stage sampling process.}
    % To sample $\Bq$ such that $\Bq \in \cE' \cap \cE_2 \cap \cE_3$, we can first sample a quantile $\qb \sim I_1$ for a new buyer and then sample the remainder of $\Bq$.
    Conditioned on $\cE_3$, by Claim~\ref{claim:non_fsd_orig_matched}, we know that every new buyer in $I_1$ is traded (because every buyer in $I_1$ is traded).
    Let $\cG_k$ be the event that there are exactly $k$ new buyers in $I_1$.
    On the event $\cG_k \cap \cE_3 \cap \cE_2$ (provided that this event is non-empty), $b^*(\Bq)\ind{\cF} = b^*(\Bq) \leq \min_{i\in[k]} b(q'(i))$, where $q'(1), \ldots, q'(k)$ are $k$ uniform random quantiles from $I_1$.
    Note that $\min_{i \in [k]} b'(q(i))$ is first-order stochastically dominated by $b(\qb)$ where $\qb \sim I_1$ uniformly at random.
    Thus, $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    This is true for every $k$ such that $\cE_2 \cap \cE_3 \cap \cE' \cap \cG_k \neq \emptyset$ so we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 2: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| \geq 1$.}
    This case is very similar to the above.
    Let $\cE'' = \{|I_1 \cap \Bnew| = 0, |I_1 \cap \Bold| \geq 1\}$.
    In this case, we define $\cG_k$ as the event that there are exactly $k$ \emph{original} buyers in $I_1$.
    Following an identical proof, we can show that $\expectg{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE'' \cap \cG_k} \leq \expects{\qb \sim I_1}{b(\qb)}$.
    Thus, we conclude that $\expect{b^*(\Bq) \ind{\cF}}{\cE_2 \cap \cE_3 \cap \cE''} \leq \expects{\qb \sim I_1}{b(\qb)}$.

    \paragraph{Case 3: $|I_1 \cap \Bnew| = 0$ and $|I_1 \cap \Bold| = 0$.}
    This case is fairly trivial.
    Let $\cE''' = \{I_1 \cap \Bnew = I_1 \cap \Bold = \emptyset\}$.
    Then $b^*(\Bq)\ind{\cF} \leq b(1-p)\ind{\cF} \leq \expects{\qb \sim I_1}{b(\qb)} \ind{\cF}$ either because there is no trade or every traded buyer has a quantile outside $I_1$.
    
    Combining the three cases above concludes the proof.
\end{proof}

\subsection{Comparing STR and OPT in different regimes}
\label{subsec:cont_prob}
Let $\alpha \in (0, 1)$ be a constant decided later. We split the analysis into the regime where $n \geq \alpha m$ and $n \leq \alpha m$.
\paragraph{Case 1: $n \geq \alpha m$.}
\begin{lemma}
    \label{lemma:contProbE1}
    $\prob{\cE_1} \geq 1 - 6c(1-p)^c$.
\end{lemma}
\begin{proof}
    We have
    \[
        \prob{|I_1 \cap \Bnew| \leq 1}
        = (1-p)^c + c(1-p)^{c-1} p
        = (1-p)^c \left[ 1 + cp/(1-p) \right]
        < 2c (1-p)^c
    \]
    The inequality uses that $p=\frac{rn}{100m}\leq\frac{1}{100}$. Thus $p(1-p) \leq 1/4$ and $1 + c/4 \leq c + c/4 < 2c$ since $c \geq 1$.
    Identical calculations give
    \[
        \prob{|J_1 \cap \Snew| \leq 1} < 2c(1-p)^c
    \]
    Next, we have $\prob{|I_2 \cap \Bold| = 0} \geq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq (1-p)^c$ since $n\geq c$.
    Taking a union bound gives that $\prob{\neg\cE_1} \leq 6c(1-p)^c$.
\end{proof}
\begin{lemma}
    \label{lemma:cont_big_n}
    Let $\alpha > 0$ and suppose that $n \geq \max\{ 300 \log(16m) / r, \alpha m\}$.
    Let $c \geq \frac{400 \log(2400 / r\alpha)}{r \alpha}$.
    Then
    \[
        \expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0. 
    \]
\end{lemma}
% \lemmacontbign*
\begin{proof}[Proof of Lemma~\ref{lemma:cont_big_n}]
    Note that $\cE_1$ and $\cE_2$ are disjoint, we have
    \begin{align}
        \expect{\STR(\Bq) - \OPT(\Bq)}
        & = \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1\cap\cE_3} \label{eq:contE1E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2\cap\cE_3} \label{eq:contE2E3} \\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \cdot \prob{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \label{eq:contNotE1NotE2E3}\\
        & + \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3} \label{eq:contE3}
    \end{align}
    For Eq.~\eqref{eq:contE1E3}, we use Lemma~\ref{lemma:cont_E1_lb}, Lemma~\ref{lemma:cont_probE3_bound}, and Lemma~\ref{lemma:contProbE1}, along with a union bound to get that
    \begin{multline*}
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_1 \cap \cE_3} \cdot \prob{\cE_1 \cap \cE_3} \\ \geq \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot \left( 1 - 6c(1-p)^c - 4 \exp(-rn/300) \right).
    \end{multline*}
    For Eq.~\eqref{eq:contE2E3}, we use Lemma~\ref{lemma:cont_bound_loss_E2}, Lemma~\ref{lemma:contProbE1}, and the fact that $\prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \prob{\neg\cE_1}$ to get
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\cE_2 \cap \cE_3} \cdot \prob{\cE_2 \cap \cE_3} \geq - \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)} \cdot 6c(1-p)^c
    \]
    For Eq.~\eqref{eq:contNotE1NotE2E3}, Lemma~\ref{lemma:contNotE2Better} gives
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_1 \cap \neg\cE_2 \cap \cE_3} \geq 0.
    \]
    Finally, for Eq.~\eqref{eq:contE3}, by \Cref{lemma:expectation_E3} we have
    \[
        \expectg{\STR(\Bq) - \OPT(\Bq)}{\neg\cE_3} \cdot \prob{\neg\cE_3}
        \geq - 4m \cdot \exp(-rn/300) \cdot \expects{\substack{\qb \sim I_1 \\ \qs \sim J_1}}{b(\qb) - s(\qs)}.
    \]
    Putting everything together, it suffices to check that
    \[
        1 - 6c(1-p)^c - 4\exp(-rn / 300) \geq 6c(1-p)^c + 4m \exp(-rn/300).
    \]
    %A sufficient condition is that 
    The above inequality holds if $12c(1-p)^c \leq 1/2$ and $8m\exp(-rn/300) \leq 1/2$.
    To prove $12c(1-p)^c \leq 1/2$, note that $p = rn/(100 m) \geq r \alpha / 100$ and thus by our choice of $c$, we have
    $c \geq 4\log(24/p) / p$.
    Therefore,
    \[
        12c(1-p)^c \leq 12ce^{-cp} = \frac{12cp e^{-cp}}{p} \leq \frac{12e^{-cp/2}}{p} \leq \frac{12e^{-\log(24/p)}}{p} = \frac{1}{2}.
    \]
    Note that in the second inequality, we used that $cp \geq 4$ and the numeric inequality $xe^{-x} \leq e^{-x/2}$ valid for $x \geq 4$ (see Claim~\ref{claim:xexp_lt_exp}).
    For the inequality $8m \exp(-rn / 300) \leq 1/2$, note that this follows from the assumption that $r \geq \frac{300 \log(16 m)}{r}$.
\end{proof}

\paragraph{Case 2: $n \leq \alpha m$.}
\begin{lemma}
    \label{lemma:cont_small_n_E1}
    Let $\alpha > 0$ and suppose that $n \leq \alpha m$ and $c \geq 2$.
    Then
    \[
        \prob{\cE_1} \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r\alpha}{100} \right)^{2c-4} p^6.
    \]
\end{lemma}
\begin{proof}
    Since $|I_1 \cap \Bnew|$ and $|J_1 \cap \Snew|$ are both distributed as $\Binom(p, c)$, we have that
    \[
        \prob{|J_1 \cap \Bnew| = 2} = \prob{|I_1 \cap \Bnew| = 2} = \binom{c}{2} (1-p)^{c-2} p^2 \geq \frac{c^2}{4} (1-r\alpha / 100)^{c-2} p^2
    \]
    where we used that $p = rn/100m \leq r\alpha / 100$ and $\binom{c}{2} = c(c-1) / 2 \geq c^2 / 4$ since $c \geq 2$.
    Next, since $|I_2 \cap \Bold|$ is distributed as $\Binom(p, m)$ and $|J_2 \cap \Sold|$ is distributed as $\Binom(p, n)$, we have
    \[
        \prob{|I_2 \cap \Bold| = 0} \leq \prob{|J_2 \cap \Sold| = 0} = (1-p)^n \leq 1-p.
    \]
    Therefore, $\prob{|I_2 \cap \Bold| \geq 1} \geq \prob{|J_2 \cap \Sold| \geq 1} \geq p$.
    Since the random variables $|I_1 \cap \Bnew|, |J_1 \cap \Snew|, |I_2 \cap \Bold|, |J_2 \cap \Sold|$ are all independent, the lemma follows by taking a product.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n_E2}
    Suppose that $n \leq mr / 8$.
    Then $\prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3)$.
\end{lemma}
\begin{proof}
    Recall that $\cE_2 \subset (\{\Snew \cap (r/2, 1] = \Snew\} \cup \{|\Bold \cap (1-r/2, 1]| < n+c\})$.
    Since $|\Snew \cap (r/2, 1]|$ is distributed as $\Binom(1-r/2, c)$ we have that
    \[
        \prob{\Snew \cap (r/2, 1] = \Snew} = (1-r/2)^c \leq \exp(-rc/2). 
    \]
    Next, since $\expect{|\Bold \cap (1-r/2, 1]|} = mr/2 \geq 4n$, the Chernoff bound gives (Lemma~\ref{lemma:chernoff})
    \[
        \prob{|\Bold \cap (1-r/2, 1]| < n+c}
        \leq \prob{|\Bold \cap (1-r/2, 1]| < 2n}
        \leq \exp(-n/3).
    \]
    Using a union bound proves the lemma.
\end{proof}
\begin{lemma}
    \label{lemma:cont_small_n}
    Suppose that $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100m / rn)}{r}$, $n \geq 150c + \frac{300}{r} \log(9m)$, and $n \leq mr/8$.
    Then $\expects{\Bq}{\STR(\Bq) - \OPT(\Bq)} \geq 0$.
\end{lemma}
\begin{proof}
    The proof is nearly identical to Lemma~\ref{lemma:cont_big_n} except that we replace the bounds on $\prob{\cE_1 \cap \cE_3}$ and $\prob{\cE_2 \cap \cE_3}$
    with Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_small_n_E2}, respectively.
    For the former, using Lemma~\ref{lemma:cont_small_n_E1} and Lemma~\ref{lemma:cont_probE3_bound}, where $\alpha = r/8$,
    \[
        \prob{\cE_1 \cap \cE_3}
        = 1 - \prob{\neg\cE_1 \cup \neg\cE_3}
        \geq 1 - \prob{\neg\cE_1} - \prob{\neg\cE_3}
        \geq \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c - 4} p^6 - 4\exp(-rn / 300).
    \]
    and for the latter, using Lemma~\ref{lemma:cont_small_n_E1}, we have
    \[
        \prob{\cE_2 \cap \cE_3} \leq \prob{\cE_2} \leq \exp(-rc / 2) + \exp(-n/3).
    \]
    Continuing as in Lemma~\ref{lemma:cont_big_n}, we now require that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 - 4\exp(-rn/ 300)
        \geq
        \exp(-rc/2) + \exp(-n/3) + 4m \exp(-rn / 300).
    \]
    Rearranging, a sufficient condition is that
    \[
        \frac{c^4}{16} \cdot \left( 1 - \frac{r \alpha}{100} \right)^{2c-4} p^6 \geq \exp(-rc / 2) + 9m \exp(-rn / 300).
    \]
    Using that $n \geq 150c + \frac{300}{r} \log(9m)$, one can verify that $9m \exp(-rn / 300) \leq \exp(-rc/2)$.
    Also, since $c \geq 2$, we have $c^4/16 \geq 1$.
    Rearranging further, it suffices to show that
    \[
        p^6 \geq \frac{2\exp(-rc/2)}{\left(1 - r\alpha/100 \right)^{2c-4}}.
    \]
    This latter inequality is true since
    \begin{align*}
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c-4}}
        & \leq
        \frac{2 \exp(-rc / 2)}{(1-r\alpha/100)^{2c}} \\
        & \leq 2\exp(-rc / 2 + 4rc\alpha / 100) \\
        & \leq 2\exp(-rc / 4) \\
        & \leq \left( \frac{rn}{100m} \right)^6 = p^6,
    \end{align*}
    where the second inequality used the numeric inequality $1/(1-x) \leq e^{2x}$ valid for $x \in [0, 1/4]$ (see Claim~\ref{claim:one_over_one_minus_x_lt_exp}),
    the third inequality used that $\alpha \leq 1$ and thus, $-rc/2 + 4rc\alpha / 100 \leq -rc / 4$,
    and the last inequality is because $c \geq \frac{4 \log(2)}{r} + \frac{24 \log(100 m / rn)}{r}$.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:non_fsd}}
\label{subsec:proof_non_fsd}
Finally, we prove Theorem~\ref{thm:non_fsd}.
\begin{proof}[Proof of Theorem~\ref{thm:non_fsd}]
    Let $\alpha = r/8$.
    We first ``pre-augment'' the market so that we can apply the results from the previous section.
    Let $m \geq n$ be the original number of buyers and sellers.
    First, we add $O(\log(1/r)/r)$ buyers to get $m' = m + O(\log(1/r)/r)$ buyers and so that $m' \geq 300 \log(16m') / r$.
    If $n \leq 300 \log(16m') / r$ we add $300 \log(16m') / r - n = O(\log(m/n) / r)$ buyers \emph{and} sellers get a total of $m''$ buyers $n''$ sellers.
    Note that $m'' \geq 300 \log(16m'') / r$ and $n'' \geq 300 \log(16m'') / r$.
    
    Next, choose
    \[
        c \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m''/rn'')}{r} \right\} = O(\log(m/rn) / r).
    \]
    Let $\Delta_N = 150c + \frac{300}{r} \log(16m'') - n'' \leq 150c$.
    If $\Delta_N > 0$ then it straightforward, albeit somewhat cumbersome, calculation to check that setting $m''' = m'' + 200\cdot C \cdot \Delta_N$, $n''' = n'' + 200\cdot C \cdot \Delta_N$ and $c''' = c + C\cdot \Delta_N$ for a large enough constant $C > 0$, we have
    \begin{itemize}
        \item $m''' \geq n''' \geq 150c + \frac{300}{r} \log(16m''')$;
        \item $c''' \geq \max\left\{\frac{400 \log(2400 r/\alpha)}{r \alpha}, \frac{4 \log(2)}{r} + \frac{24 \log(100m'''/rn''')}{r} \right\} = O(\log(m / rn) / r)$.
    \end{itemize}
    
    Finally, applying Lemma~\ref{lemma:cont_big_n} if $n''' \geq \alpha m'''$ and Lemma~\ref{lemma:cont_small_n} if $n''' \leq \alpha m'''$,
    we conclude that $\STR(m''' + c''',n''' + c''') \geq \OPT(m''',n''')$.
    Note that both $m'''+c''' - m$ and $n''' + c''' - n$ are $O(\log(m / rn) / r)$.
\end{proof}

\mingfeinote{
\subsection{Lower Bound}\label{subsec:non_fsd_lb}

We derive a lower bound on the number of additional agents with result of \cite{BabaioffGG20}.
%required for any deterministic, prior-independent, truthful, BB and anonymous mechanism.

\begin{lemma}\label{lem:bgg_lb}
\cite[Proposition~E.5]{BabaioffGG20} For any $\eps>0$ and any integer $m, n$, there exists a double auction instance with $m$ buyers, $n$ sellers, and distributions $F_B$, $F_S$ such that: (1) $\Pr_{b\sim F_B, s\sim F_S}[b\geq s]\geq \frac{\eps^2}{(m+n+2c)^8}$; (2) For any deterministic, prior-independent, BIC, IR, BB and anonymous\footnote{A mechanism is \emph{anonymous} if the mechanism treats each buyer and seller equally. In other words, swapping the identity of any two buyers (or sellers) will only result in their allocation and payment being swapped.} mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than $\eps$ times the first-best GFT on $m$ buyers and $n$ sellers.
\end{lemma}

\begin{corollary}\label{cor:non_fsd_lb}
For any sufficiently small $r\in (0,1)$, there exists a double auction instance with \\
$\Pr_{b\sim F_B, s\sim F_S}[b\geq s]=r$ such that: For any $c\leq \frac{1}{4}\cdot r^{-1/8}$ and any deterministic, prior-independent, BIC, IR, BB and anonymous mechanism $M$, the GFT of $M$ on $m+c$ buyers and $n+c$ sellers is smaller than the first-best GFT on $m$ buyers and $n$ sellers.
\end{corollary}
\begin{proof}
Applying \Cref{lem:bgg_lb} with any $n\leq m\leq \frac{1}{4}\cdot r^{-1/8}$, we have $\eps\leq \sqrt{r(m+n+2c)^8}\leq 1$. The proof is done by \Cref{lem:bgg_lb}.  
\end{proof}
}


==> zz_old_fsd_noniid_approx_oct22.tex <==
\section{Approximation and Augmentation for FSD but Non-i.i.d.~Distributions}
\label{sec:fsd_noniid_approx}
In this section, we consider the following setting.
Let us assume that we have $m$ buyers whose value distributions are given by $F_1, \ldots, F_m$ and $n$ sellers whose cost distributions are given by $G_1, \ldots, G_n$.

\begin{definition}
    We say that a market is $c$-dominant if there exists sets $B \subseteq [m]$ and $S \subseteq [n]$ such that $|B| = |S| = c$ and $F_i$ FSD $G_j$ for all $i \in B, j \in S$.
\end{definition}

\begin{theorem}
    \label{thm:fsd_noniid_approx}
    If a market is $c$-dominant then Trade Reduction obtains a $(1-??/c)$-approximation to the first-best GFT.
\end{theorem}

We require the following combinatorial lemma.
Here, we write $\binom{[n]}{\leq x} = \{ S \subseteq [n] \,:\, |S| \leq x\}$ and similarly for $\binom{[n]}{\geq x}$.
\begin{lemma}
    Suppose that $n \geq 650$ and let $k \leq \alpha n$ where $\alpha \leq 0.01$.
    There is a function $f \colon \binom{[n]}{\leq k} \to \binom{[n]}{\geq 2k}^n$ such that:
    \begin{enumerate}[itemsep=0pt, topsep=0pt]
        \item for all $S_1, S_2 \in \binom{[n]}{\leq k}$ and $i, j \in [n]$, if $(i, S_1) \neq (j, S_2)$ then $f_i(S_1) \neq f_j(S_2)$.
        \item for all $i \in [n]$ and $S \in \binom{[n]}{\leq k}$, $S \subset f_i(S)$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    We prove this using the probabilistic method.
    For each $i \in [n]$ and $S \in \binom{[n]}{\leq k}$, we define $f_i(S)$ to be the set obtained by taking the union of $S$ with a uniformly random subset of $[n] \setminus S$.
    \begin{claim}
        \label{claim:fsd_noniid_combinatorial1}
        With probability at least $1-n\cdot e^{-n/100}$, $|f_i(S)| \geq 2k$ for all $i, S$.
    \end{claim}
    \begin{proof}
        We can apply the Chernoff Bound (see \Cref{lemma:chernoff}) with $\mu = (n-k) / 2 \geq (1-\alpha)n / 2$ and $\delta = \frac{1-5\alpha}{1-\alpha}$ to get
        \begin{align*}
            \prob{|f_i(S)| \leq 2k}
            & \leq \prob{|f_i(S)| \leq 2\alpha n} \\
            & = \prob{|f_i(S) \leq \left(1- \frac{1-5\alpha}{1-\alpha}\right) \cdot \frac{(1-\alpha)n}{2}} \\
            & \leq \exp\left(-\frac{(1-5\alpha)^2}{12(1-\alpha)} \cdot n\right).
        \end{align*}
        By \Cref{fact:binom_bounds}, we have $|\binom{[n]}{\leq k}| \leq k(en/k)^k \leq n(e/\alpha)^{\alpha n}$.
        Applying the union bound, we have \textcolor{red}{(forgot to multiply below by $n$. Should be $n^2$.)}
        \begin{align*}
            \prob{\exists i \in [n], S \in \binom{[n]}{k} \text{ such that } |f_i(S)| \leq 2k}
            & \leq
            \exp\left(-\frac{(1-5\alpha)^2}{12(1-\alpha)} \cdot n\right) n \left( \frac{e}{\alpha} \right)^{\alpha n} \\
            & = n\cdot \exp\left(-n\left[\frac{(1-5\alpha)^2}{12(1-\alpha)} - \alpha \log(e/\alpha) \right] \right) \\
            & < n \cdot \exp(-n/100),
        \end{align*}
        where the last inequality uses \Cref{claim:fsd_noniid_numeric_inequality}.
    \end{proof}
    \begin{claim}
        \label{claim:fsd_noniid_combinatorial2}
        Fix any $i, j \in [n]$ and $S_1, S_2 \in \binom{[n]}{\leq k}$.
        If $(i, S_1) \neq (j, S_2)$ then $\prob{f_i(S_1) = f_j(S_2)} \leq 2^{-(n-2k)}$.
        Consequently
        \[
            \prob{\exists i, j \in [n], S_1, S_2 \in \binom{[n]}{\leq k} \text{ such that } f_i(S_1) = f_j(S_2)]}
            \leq
            n^2 \cdot 0.54^n.
        \]
    \end{claim}
    \begin{proof}
        Without loss of generality, we assume $S_1 \cup S_2 \subseteq [2k]$ (otherwise, we can rename the elements).
        Then $\prob{f_i(S_1) = f_j(S_2)} \leq \prob{f_i(S_1) \setminus [2k] = f_j(S_2) \setminus [2k]} = 2^{-(n-2k)} \leq 2^{-(1-2\alpha)n}$ since $f_i(S_1) \setminus [2k]$ and $f_j(S_2) \setminus [2k]$ is drawn uniformly and independently from $[n] \setminus [2k]$.
        Using \Cref{fact:binom_bounds} and a union bound, we have
        \begin{align*}
            \prob{\exists i, j \in [n], S_1, S_2 \in \binom{[n]}{\leq k} \text{ such that } f_i(S_1) = f_j(S_2)]}
            & \leq
            n^2(e/\alpha)^{\alpha n} 2^{-(1-2\alpha)n} \\
            & = n^2 2^{-n} (4e/\alpha)^{\alpha n} \\
            & < n^2 \cdot 0.54^n,
        \end{align*}
        where the last inequality uses \Cref{claim:fsd_noniid_numeric_inequality2}.
    \end{proof}
    Let $\cE_1$ be the event that for all $i \in [n]$ and $S \in \binom{[n]}{\leq k}$, we have $|f_i(S)| \geq 2k$ and
    $\cE_2$ be the event that for all $i, j \in [n]$ and $S_1, S_2 \in \binom{[n]}{\leq k}$, we have $f_i(S_1) \neq f_j(S_2)$ whenever $(i, S_1) \neq (j, S_2)$.
    By \Cref{claim:fsd_noniid_combinatorial1}, \Cref{claim:fsd_noniid_combinatorial2}, and a union bound we have that $\prob{\cE_1 \wedge \cE_2} \geq 1 - n\cdot e^{-n/100} - n^2 \cdot 0.54^n > 0$.
    Here, the last inequality uses \Cref{claim:fsd_noniid_numeric_inequality3}.
    We conclude that the event $\cE_1 \wedge \cE_2$ is non-empty and there exists a function $f \colon \binom{[n]}{\leq k} \to \binom{[n]}{\geq 2k}^n$ satisfying the conditions of the lemma.
\end{proof}

\begin{fact}[{\cite[Exercise~2.14]{boucheron2013concentration}}]
    \label{fact:binom_bounds}
    For all $n \geq 1$ and $1 \leq k \leq n$, we have $\sum_{j = 0}^k \binom{n}{k} \leq \left( \frac{en}{k} \right)^k$.
\end{fact}

\begin{claim}
    \label{claim:fsd_noniid_numeric_inequality}
    If $0 < \alpha \leq 0.01$ then $\frac{(1-5\alpha)^2}{12(1-\alpha)} - \alpha \log(e/\alpha) > 0.01$.
\end{claim}
\begin{proof}
    Let $f(\alpha) = \frac{(1-5\alpha)^2}{12(1-\alpha)} - \alpha \log(e/\alpha)$.
    Differentiating, we get
    \begin{align*}
        f'(\alpha)
        & = \frac{1}{12} \cdot \frac{-10(1-5\alpha)(1-\alpha) + (1-5\alpha)^2}{(1-\alpha)^2} + \log \alpha \\
        & = \frac{(1-5\alpha)(5\alpha - 9)}{12(1-\alpha)^2} + \log \alpha \\
        & = \frac{-25\alpha^2 + 50\alpha - 9}{12(1-\alpha)^2} + \log \alpha \\
        & = \frac{4}{3(1-\alpha)^2} - \frac{25}{12} + \log \alpha \\
        & \leq \frac{4}{3(1-0.01)^2} - \frac{25}{12} \approx -0.723,
    \end{align*}
    where the last inequality uses that $\alpha < 0.01$.
    In particular, $f$ is decreasing on $(0, 0.01]$ so for all $\alpha \in (0, 0.01]$, we have $f(\alpha) \geq f(0.01) \approx 0.0199$.
\end{proof}

\begin{claim}
    \label{claim:fsd_noniid_numeric_inequality2}
    If $0 < \alpha \leq 0.01$ then $(4e/\alpha)^\alpha < 1.08$.
\end{claim}
\begin{proof}
    Let $f(\alpha) = (4e/\alpha)^\alpha$.
    Then $f'(\alpha) = (4e/\alpha)^{\alpha} \log(4/\alpha)$.
    So $f$ is increasing on the interval $(0, 0.01]$ and thus, $f(\alpha) \leq f(0.01) \approx 1.072$.
\end{proof}
\begin{claim}
    \label{claim:fsd_noniid_numeric_inequality3}
    If $x \geq 650$ then $x\cdot \exp(-x/100) + x^2 \cdot 0.54^x < 1$.
\end{claim}
\begin{proof}
    Let $f(x) = x\cdot \exp(-x/100) + x^2 \cdot 0.54^x$.
    Then $f'(x) = \exp(-x/100) \cdot (1 - x/100) + 0.54^x \cdot (2 + x \log(0.54))$.
    Note that $f'(x) \leq 0$ provided $x \geq \max(100, -1/\log(0.54)) = 100$.
    Thus $f$ is non-decreasing on $[100, \infty)$.
    In particular, if $x \geq 650$ then $f(x) \geq f(650) \approx 0.977$.
\end{proof}

In what follows, we let 
\begin{lemma}
    Suppose that a market is $c$-dominant and without loss of generality, 
\end{lemma}

\textcolor{red}{(Chris: WIP below)}
\begin{lemma}
    There are functions $\alpha(\gamma) = \Theta(\gamma^2)$ and $N(\gamma) = \Theta(1/\gamma^2)$ such that the following holds.
    For any $\gamma \in (0, 1)$, if $n \geq N(\gamma)$ then there exists $T$ and a function $f \colon \binom{[n]}{\leq \alpha(\gamma) \cdot n} \to (2^{[n]})^T$ satisfying the following properties (where $\alpha = \alpha(\gamma)$.
    \begin{enumerate}[topsep=0pt, itemsep=0pt]
        \item For every $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$ we have $|f_t(S)| \geq \alpha n$.
        \item For every $t_1, t_2 \in [T]$ and $S_1, S_2 \in \binom{[n]}{\leq \alpha n}$, we have $f_{t_1}(S_1) \neq f_{t_2}(S_2)$ whenever $(t_1, S_1) \neq (t_2, S_2)$.
        \item For every $S \in \binom{[n]}{\leq \alpha n}$, we have $n \cdot \gamma^{|S|} (1-\gamma)^{n - |S|} \leq \sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|}$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    We consider the following probabilistic construction of $f$.
    For each $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$, we set $f_t(S)$ to the set which includes every element in $[n]$ with probability $\gamma$ (independently) union with $S$.
    We now split the proof into three claims which verify each requirement of the lemma.
    \begin{claim}
        \label{claim:combinatorial1}
        With probability at least $1 - (e/\alpha)^{\alpha n} e^{-n \gamma / 12}$, we have $|f_t(S)| \geq \gamma n / 2$ for all $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$.
    \end{claim}
    \begin{proof}
        By definition of $f_t(S)$, we have that $\expect{|f_t(S)|} \geq n \gamma$.
        Thus, a standard Chernoff bound (see \Cref{lemma:chernoff}) gives that $\prob{|f_t(S)| \leq n\gamma / 2} \leq e^{-n\gamma / 12}$. By \Cref{fact:binom_bounds}, we have $|\binom{[n]}{\leq \alpha n}| \leq (e/\alpha)^{\alpha n}$.
        The claim now follows by a union bound.
    \end{proof}

    \begin{claim}
        \label{claim:combinatorial2}
        With probability at least $1-T^2 (e/\alpha)^{2\alpha n} (\gamma^2 + (1-\gamma)^2)^{-n(1-2\alpha)}$, we have $f_{t_1}(S_1) \neq f_{t_2}(S_2)$ for all $t_1, t_2 \in [T]$ and $S_1, S_2 \in \binom{[n]}{\leq \alpha n}$ provided $(t_1, S_1) \neq (t_2, S_2)$.
    \end{claim}
    \begin{proof}
        We have that
        \[
            \prob{f_i(S_1) = f_j(S_2)} \leq  (\gamma^2 + (1-\gamma)^2)^{-n(1-2\alpha)}.
        \]
        Taking a union bound over all pairs of $(i,S_1)$ and $(j, S_2)$ gives that
        \begin{align*}
            \prob{\exists (i, S_1), (j, S_2) \text{ such that }f_i(S_1) = f_j(S_2)}
            \leq T^2 (e/\alpha)^{2\alpha n} (\gamma^2 + (1-\gamma)^2)^{-n(1-2\alpha)},
        \end{align*}
        where in the last inequality we used that $|\binom{[n]}{\leq \alpha n}| \leq (e/\alpha)^{\alpha n}$ (see \Cref{fact:binom_bounds}).
    \end{proof}
    \begin{claim}
        \label{claim:combinatorial3}
        Suppose that $T \geq 12n \left( \frac{1-\gamma}{\gamma^2 + (1-\gamma)^2} \right)^n$.
        Then with probability at least $1 - (e/\alpha)^{\alpha n} e^{-n}$, we have
        we have
        \[
            n \cdot \gamma^{|S|} (1-\gamma)^{n - |S|} \leq \sum_{t \in [T]} \gamma^{|f_t(S)|} (1-\gamma)^{n-|f_t(S)|}
        \]
        for every $t \in [T]$ and $S \in \binom{[n]}{\leq \alpha n}$.
    \end{claim}
    \begin{proof}
        For any fixed $T$, we have that
        \begin{align*}
            \expect{\gamma^{|f_t(S)|} \cdot (1-\gamma)^{n - |f_t(S)|}} 
            & = \gamma^{|S|} \expect{\gamma^{|f_t(S)|-|S|} \cdot (1-\gamma)^{(n-|S|) - (|f_t(S)|-|S|)}} \\
            & = \gamma^{|S|} \sum_{k=0}^{n-|S|} \gamma^k \cdot (1-\gamma)^{(n-|S|)-k} \prob{|f_t(S)| - |S| = k} \\
            & = \gamma^{|S|} \sum_{k=0}^{n-|S|} \binom{n-|S|}{k} \gamma^{2k} (1-\gamma)^{2(n-|S| - k)} \\
            & = \gamma^{|S|} \cdot (\gamma^2 + (1-\gamma)^2)^{n - |S|}.
        \end{align*}
        By a Chernoff bound (see \Cref{lemma:chernoff}), since $\gamma^{|f_t(S)|}(1-\gamma)^{n-|f_t(S)|} \in [0, (1-\gamma)^{n-|S|}]$, we have
        \[
            \sum_{t \in [T]} \gamma^{|f_t(S)|} \cdot (1-\gamma)^{n - |f_t(S)|}
            \leq \frac{1}{2} T \gamma^{|S|} \cdot (\gamma^2 + (1-\gamma)^2)^{n - |S|}
        \]
        with probability at most $\exp\left( -\frac{T(\gamma^2 + (1-\gamma)^2)^{n-|S|}}{12(1-\gamma)^{n-|S|}} \right)$.
        If $T \geq 2n \left( \frac{1-\gamma}{\gamma^2 + (1-\gamma)^2} \right)^n \geq 2n \left( \frac{1-\gamma}{\gamma^2 + (1-\gamma)^2} \right)^{n-|S|}$ (the second inequality uses $(1-\gamma) / (\gamma^2 + (1-\gamma)^2) \geq 1$ which is true when $\gamma \leq 1/2$) then we have
        \begin{equation}
            \label{eqn:combinatorial1}
            \sum_{t \in [T]} \gamma^{|f_t(S)|} \cdot (1-\gamma)^{n - |f_t(S)|} < n \cdot \gamma^{|S|} (1-\gamma)^{n-|S|}
        \end{equation}
        with probability at most $e^{-n}$.
        Taking a union bound over all $S$ shows that \Cref{eqn:combinatorial1} happens with probability at most $(e/\alpha)^{\alpha n} \exp(-n / 6)$.
    \end{proof}
    We take
    \[
        \alpha = \min\left\{\frac{\gamma / 24}{1 + 2\log(24 / \gamma)}, \frac{\log(1 + \gamma^2 / (1-\gamma)^2)}{8(1 + \log(1 + \gamma^2 / (1-\gamma)^2))}, \frac{\log(1 + \gamma^2 / (1-\gamma)^2)}{8 \log(1/(\gamma^2 + (1-\gamma)^2))} \right\} = \Theta(\gamma^2).
    \]
    With this, note that $(e/\alpha)^\alpha \leq \gamma / 24$, $(e/\alpha)^{2\alpha} \leq (1 + \gamma^2 / (1-\gamma)^2)^{1/4} = ((1-\gamma)^2 + \gamma^2) / (1-\gamma)^2)^{1/4}$, and $1/(\gamma^2 + (1-\gamma)^2)^{2\alpha} \leq ((1-\gamma)^2 + \gamma^2) / (1-\gamma)^2)^{1/4}$.
    We also take
    \[
        T = 12n \left( \frac{1-\gamma}{(\gamma^2 + (1-\gamma)^2)} \right)^n.
    \]
    Let $\cE_1, \cE_2, \cE_3$ correspond to the three conditions in the lemma.
    We show that if $n$ is sufficiently large (in particular, if $n \geq \Theta(1/\gamma^2)$) then we have $\prob{\cE_1, \cE_2, \cE_3} > 0$.

    By \Cref{claim:combinatorial1}, \Cref{claim:combinatorial2}, and \Cref{claim:combinatorial3}, we have $\prob{\cE_1} \geq 1 - e^{-n\gamma / 24}$,
    \begin{align*}
        \prob{\cE_2}
        & \geq
        1 - 144n^2 \left( \frac{1-\gamma}{\gamma^2 + (1-\gamma)^2} \right)^{2n} \cdot \left( \frac{(1-\gamma)^2 + \gamma^2}{(1-\gamma)^2} \right)^{n / 2} \cdot (\gamma^2 + (1-\gamma)^2)^{-n} \\
        & =
        1 - 144n^2 \left( \frac{(1-\gamma)^2}{\gamma^2 + (1-\gamma)^2} \right)^{n/2},
    \end{align*}
    and
    $\prob{\cE_3} \geq 1 - e^{-n(1-\gamma / 24)} \geq 1 - e^{-n\gamma / 24}$.
    By a union bound, we have that
    \[
        \prob{\cE_1, \cE_2, \cE_3}
        \geq 1 - 2e^{-n\gamma / 24} - 144n^2 \left( \frac{(1-\gamma)^2}{\gamma^2 + (1-\gamma)^2} \right)^{n/2}.
    \]
    Define $a = \frac{2 \log(576)}{\log((\gamma^2 + (1-\gamma)^2) / (1-\gamma)^2)}$ and $b = \frac{4}{\log((\gamma^2 + (1-\gamma)^2) / (1-\gamma)^2)}$. Note that $a, b = \Theta(1/\gamma^2)$.
    We now take
    \[
        n \geq \max\left\{ \frac{24 \log 8}{\gamma},  2\max\{a, 5(b+1)(1 + \log(b+1))\} \right\} = \Theta(1/\gamma^2).
    \]
    In this case, we have $2e^{-n\gamma / 24} \leq 1/4$.
    Further, some calculations (see \Cref{claim:log_ineq1}) gives that
    \begin{align*}
        n
        & \geq a + b \log n \\
        & = \frac{2 \log 576}{\log((\gamma^2 + (1-\gamma)^2) / (1-\gamma)^2)} + \frac{4 \log n}{\log((\gamma^2 + (1-\gamma)^2) / (1-\gamma)^2)},
    \end{align*}
    which, upon rearranging, is equivalent to
    \[
        144n^2 \left( \frac{(1-\gamma)^2}{\gamma^2 + (1-\gamma)^2} \right)^{n/2} \leq \frac{1}{4}.
    \]
    We conclude that $\prob{\cE_1, \cE_2, \cE_3} > 0$.
\end{proof}
%     Let us focus on the dominant terms for now (the ones with exponents of $n$). This amounts to
%     \begin{align*}
%         \frac{(1-\gamma)^2}{\gamma^2 + (1-\gamma)^2} \cdot \frac{1}{(\gamma^2 + (1-\gamma)^2)^{2\alpha}} \cdot \left( \frac{e}{\alpha} \right)^{2\alpha}.
%     \end{align*}
%     The second and third factors tend to $1$ as $\alpha \to 0$.
%     Thus, we can choose $\alpha$ such that the quantity above is $< 1$ provided $\gamma \in (0, 0.5)$ \textcolor{red}{(Chris: I believe it is also true for $\gamma = 0.5$. Will double check.)}
%     Thus, in the above probability, the base of the exponent terms is $< 1$ so we can take $n$ sufficiently large to prove the lemma.
% \end{proof}

\begin{claim}
    \label{claim:alpha_log_e_alpha}
    Fix $x \in (0, 1)$.
    Suppose that $0 <\alpha \leq \frac{x}{1 + 2\log(1/x)}$.
    Then $\alpha \log(e/\alpha) \leq x$.
    Equivalently, $(e/\alpha)^{\alpha} \leq e^x$.
\end{claim}
\begin{proof}
    First we check that $\frac{x}{1 + 2 \log(1/x)} < 1$ whence $\alpha < 1$.
    Let $f(x) = \frac{x}{1+2\log(1/x)}$.
    Then $f'(x) = \frac{2\log(1/x) + 3}{(1+2\log(1/x))^2} > 0$ when $x \in (0, 1)$.
    Thus, $f(x) \leq f(1) = 1$ when $x \in (0, 1)$.
    Now let $g(\alpha) = \alpha \log(e/\alpha)$.
    Then $g'(\alpha) = - \log(\alpha) > 0$ when $\alpha < 1$ so it suffices to check the claim only when $\alpha = \frac{x}{1 + 2\log(1/x)}$.
    In this case, we have
    \begin{align*}
        \alpha \log(e/\alpha)
        & = \frac{x}{1 + 2\log(1/x)} \left[1 + \log\left( \frac{1 + 2\log(1/x)}{x} \right) \right] \leq x \\
        & \leq \frac{x}{1 + 2\log(1/x)} \cdot [1 + 2\log(1/x)] = x,
    \end{align*}
    where the inequality is from \Cref{claim:alpha_log_e_alpha_aux}.
\end{proof}
\begin{claim}
    \label{claim:alpha_log_e_alpha_aux}
    If $x \in (0,1)$ then $\log((1+2\log(1/x))/x) \leq 1 + 2\log(1/x)$.
\end{claim}
\begin{proof}
    By exponentiating, the inequality is equivalent to $1 + 2 \log(1/x) \leq 1/x^3$.
    Taking $u = 1/x$ the inequality is equivalent to $1 + 2\log u \leq u^3$ for $u > 1$.
    Let $f(u) = u^3 - 2 \log u - 1$.
    Then $f(1) = 0$ and $f'(u) = 3u^2 - 2 / u > 0$ when $u \geq 1$.
    We conclude that $f(u) \geq 0$ for all $u \geq 1$.
\end{proof}

\begin{claim}
    \label{claim:log_ineq1}
    Let $a, b > 0$.
    If $x \geq 2 \max\{a, 5(b+1)(1 + \log(b+1))\}$ then $x \geq a + b\log x$.
    Equivalently, $e^x / x^b \geq e^a$.
\end{claim}
\begin{proof}
    We have $x - b\log x \geq x/2 \geq a$ where the first inequality follows from \Cref{claim:log_ineq2} and the second inequality is because $x \geq 2a$.
\end{proof}
\begin{claim}
    \label{claim:log_ineq2}
    Fix $b > 0$.
    If $x \geq 10(b+1)(1 + \log(b+1))$ then $x - b \log x \geq x / 2$.
\end{claim}
\begin{proof}
    The last inequality is equivalent to $x/2 - b \log x \geq 0$.
    Let $f(x) = x/2 - b\log x$.
    Note that $f'(x) = 1/2 - b / x$ so $f$ is increasing on $(2b, \infty)$.
    Thus it suffices to prove that $f(x) \geq 0$ when $x= 10(b+1)(1 + \log(b+1))$.
    Let
    \begin{align*}
        g(b)
        & = f(2(b+1)(1 + \log(b+1))) \\
        & = 5(b+1) + 5(b+1) \log(b+1) - b \log(2) - b \log(b+1) - b\log(1 + \log(b+1)).
    \end{align*}
    Some calculations give that
    \begin{align*}
        g'(b) & = 5 + 5(\log(b+1) + 1) - \log(2) - \frac{b}{b+1} - \log(b+1) \\
        & - \frac{b}{(b+1)(1 + \log(b+1))} - \log(1+\log(b+1)).
    \end{align*}
    Differentiating again gives
    \begin{align*}
        g''(b) & = \frac{5}{b+1} + \frac{1}{(b+1)^2} - \frac{1}{b+1} + \frac{b - \log(b+1) + 1}{(b+1)^2(1+\log(b+1))^2} - \frac{1}{(b+1)(1+\log(b+1))} \\
        & = \frac{4}{b+1} + \frac{1}{(b+1)^2} - \frac{(b+2) \log(b+1)}{(b+1)^2(1 + \log(b+1))^2} \\
        & = \frac{4(b+1)(1 + 2 \log(b+1) + \log^2(b+1)) - (b+2) \log(b+1)}{(b+1)^2(1 + \log(b+1))^2} + \frac{1}{(b+1)^2} > 0.
    \end{align*}
    Note that $g(0) = 5$ and $g'(0) = 10 - \log 2 > 0$ and $g'(b) > 0$ for all $b > 0$.
    We conclude that $g(b) \geq g(0) > 0$ for all $b > 0$.
\end{proof}

==> zz_str_mar30.tex <==
\section{Seller trade reduction}
\label{sec:str}
% \paragraph{Mechanism.}
% The seller trade reduction mechanism works as follows.
% Suppose there are $m$ buyers and $n$ sellers.
% We always assume that $m \geq n$. \todo{At some point, we should write down why the case $m \leq n$ is symmetric.}
% \mingfei{For the case of $m\leq n$, we can swap the role of buyers and sellers by considering the buyer distribution $C-F_S$ and seller distribution $C-F_B$ for some large $C$ (the distribution now has to be bounded though, any other thoughts?). We will need the buyer trade reduction mechanism for the $m\leq n$ case.}
% \chris{The Babaioff paper had some stuff about this. They say exactly the same thing except that they also mentioned that unboundedness doesn't cause any issues. I don't really understand why at the moment though. Can we convince ourselves that if $m \leq n$ then BTR would use a completely analogous proof? We could also say that.}
% Let $b_1 \geq \ldots \geq b_m \geq 0$ be the values of the buyers and $0 \leq s_1 \leq \ldots \leq s_n$ be the values of the sellers.
% For notation, we assume that $s_{n+1} = \infty$.
% Let $r = \max\{ i \leq \min(m, n) \,:\, b_i \geq s_i \}$.
% If $b_r \geq s_{r+1} \geq s_r$ then we offer a price of $s_{r+1}$ to the $r$ highest value buyers and the $r$ lowest value sellers.
% Otherwise, we offer a price of $b_r$ to the $(r-1)$ highest value buyers and a price of $s_r$ to the $(r-1)$ lowest value sellers.

% We let $\OPT(m, n)$ be the (random) GFT from the optimal mechanism when there are $m$ buyers and $n$ sellers.
% Similarly, we let $\STR(m, n)$ be the (random) GFT of the seller trade-reduction mechanism when there are $m$ buyers and $n$ sellers.

% \chris{Mention at some point that both $\STR(m,n)$ and $\OPT(m,n)$ are increasing in both coordinates. I think, as stated, we prove $\STR(m+c_1, n+c_2) \geq \OPT(m,n)$.}

In this section we prove our main result which is that STR with a constant number of additional agents extracts at least as much GFT as the optimal allocation with the original set of agents.
\begin{theorem}
    \label{thm:str_main}
    There is an absolute constant $c \geq 1$ such that $\STR(m+c,n+c) \geq \OPT(m,n)$.
\end{theorem}

\mingfei{The notations below will be used throughout the paper, we can move them to the prelim.}

The proof uses a coupling argument. We first present some notations necessary for the proof. For $q \in (0, 1)$, we let $b(q) = F_B^{-1}(q)$ and $s(q) = F_S^{-1}(q)$, where $F_B, F_S$ are the c.d.f.'s of the buyer and seller distribution respectively. For simplicity, we assume that $F_B, F_S$ are continuous so that their inverses are well-defined. In the proof we fix $m,n,c$. ($c$ will be decided in later proof.) We use $\STR, \OPT$ to denote $\STR(m+c, n+c), \OPT(m,n)$. Denote $N=m+n+2c$ the total number of quantiles in the augmented setting. Let $q_1, \ldots, q_N$ be $N$ uniform quantiles from $[0,1]$. We assume these quantiles are sorted so that $q_1 \geq \ldots \geq q_N$. Let $\Bq = (q_1, \ldots, q_N)$. For exposition purposes, we sometimes abuse the notations and use $q(i)$ to denote $q_i$. 

We then uniformly assign these quantiles to all agents in the augment setting, including all original (called ``old'') and augment (called ``new'') buyers and sellers.
%\chrisnote{
Formally, let $\pi \colon [N] \to \{\BO, \BN, \SO, \SN\}$ be a function that maps indices to old buyers, new buyers, old sellers, and new sellers, respectively. Let $\Pi_{n,m,c} = \{ \pi \,:\, |\pi^{-1}(\BO)| = m, |\pi^{-1}(\SO)| = n, |\pi^{-1}(\BN)| = |\pi^{-1}(\SN)| = c\}$ be the set of valid assignments. The assignment we choose is thus uniformly drawn from $\Pi_{n,m,c}$. Given an assignment $\pi$, we write $\Bold^{\pi} = \pi^{-1}(\BO)$ as the set of indices $i$ such that the quantile $q_i$ is assigned to an old buyer. Similarly, define $\Bnew^{\pi}$, $\Sold^{\pi}$, $\Snew^{\pi}$ as the sets for new buyers, old sellers and new sellers respectively. Let $i^{\pi}_1 \leq \ldots \leq i^{\pi}_{m+c}$ be the indices of all buyers (in an decreasing order of their quantiles and thus their values). Let $j^{\pi}_1 \geq \ldots \geq j^{\pi}_{m+c}$ be the indices of all sellers (in an increasing order of their quantiles and thus their values). 
%Similarly, let $i^{\pi, O}_1 \leq \ldots \leq i^{\pi, O}_{m}$ and $i^{\pi, N}_1 \leq \ldots \leq i^{\pi, N}_{m}$
We omit the superscript $\pi$ when the assignment is fixed and clear from context. 

%In the remainder of this section $\pi$ always refers to a uniformly random element from $\Pi_{m,n,c}$ and so we write $\Bold, \Bnew, \Sold, \Snew$ for the (random) set of old and new buyers and sellers.}
% Denote $\pi$ the random assignment. Define the (random) set $\Bold\subseteq [N]$ as the set of all indices $i$ such that the quantile $q_i$ is assigned to an old buyer. Similarly, define $\Bnew$, $\Sold$, $\Snew$ as the sets for new buyers, old sellers and new sellers respectively. They are all determined by the assignment $\pi$. 

Note that the agents' profile in the original and augmented setting are both determined by the quantiles $\Bq$ and the assignment $\pi$. For any fixed $(\Bq,\pi)$, we abuse the notation and denote $\STR(\Bq,\pi)$ the GFT of seller trade reduction at the current profile, in the augment setting. Similarly denote $\OPT(\Bq,\pi)$ the first-best GFT at the current profile, in the original setting. Thus $\STR = \bE_{\Bq,\pi}[\STR(\Bq,\pi)]$ and $\OPT = \bE_{\Bq,\pi}[\OPT(\Bq,\pi)]$.


%\chris{Mingfei: I modified this paragraph a bit. Can you take a look? If you agree, feel free to clean up the tex.}

%\mingfei{Agree with your comment. Rewrote the condition to make it clear and formal.}

The high-level idea of the proof is as follows.
%\modify{For the entire proof, we condition on the quantiles but \emph{not} the assignment of these quantiles to the agents.
%We then construct two events $\cE_1, \cE_2$ over the randomness of the assignment such that:}
For any fixed $\Bq$, we would like to construct two events $\cE_1$ and $\cE_2$ over the randomness of the assignment $\pi$ such that:
\begin{enumerate}
    \item $\cE_1$ is a sufficient condition for $\STR(\Bq, \pi)\geq\OPT(\Bq, \pi)$. Moreover, $\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_1]\geq C(\Bq)$ for some $C(\Bq)>0$. 
    \item $\cE_2$ is a necessary condition for $\OPT(\Bq, \pi)>\STR(\Bq, \pi)$. Moreover, $\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_2]\leq C(\Bq)$.
    \item $\Pr_{\pi}[\cE_1]\geq\Pr_{\pi}[\cE_2]$.
\end{enumerate}

%\modify{We note that the constant $C > 0$ that we choose is a function of the quantiles and the distributions $F_B, F_S$.}

The existence of both events immediately proves the theorem since
\begin{align*}
\STR-\OPT &= \bE_{\Bq, \pi}[\STR(\Bq,\pi)-\OPT(\Bq,\pi)] \\
&\geq \bE_{\Bq}[\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_1]\cdot \Pr[\cE_1]+\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_2]\cdot \Pr[\cE_2]]\geq 0
\end{align*}
Here the first inequality follows from Property 2: For any $\Bq$, $\STR(\Bq,\pi)\geq \OPT(\Bq,\pi)$ when $\cE_2$ does not happen and thus $\STR(\Bq,\pi) \geq \OPT(\Bq,\pi)$ on the event $\overline{\cE_1} \cap \overline{\cE_2}$.

%\chris{I think we only use the first two and last two buckets right?}
Before diving into technical details, we need one last bit of notation.
By adding a constant number of buyers and sellers, we assume that $m \geq n \geq 20$. Let $p=\left\lceil \frac{n}{10} \right\rceil \geq 2$. Define sets
\begin{align*}
I_1 = \left\{1, \ldots, p\right\}, \quad
& I_2 = \left\{ p + 1, \ldots, 2p\right\}, \\
J_1 = \{N-p+1, \ldots, N\}, \quad 
& J_2 = \{N-2p+1, N-p\}.
\end{align*}
%Here, we use $A - B$ to denote the Minkowski difference of two sets, i.e.~$A - B = \{a - b\,:\, a \in A, b \in B\}$.
In other words, $I_1$ denotes the first $p$ indices, $I_2$ denote the $p$ indices after $I_1$, $J_1$ denote the last $p$ indices, and $J_2$ denote the $p$ indices before $J_1$. It is straightforward to check that when $n\geq 20$, $I_1, I_2, J_1, J_2$ are all disjoint.
% and $|I_1| = |I_2| = |J_1| = |J_2| = p \geq 2$.
% \mingfei{Rewrote the set definition to make things simple. And I feel like we don't need a proof for the following claim since it's pretty straightforward.}

\begin{claim}
    $I_1, I_2, J_1, J_2$ are all disjoint.
    % In addition $|I_1| = |I_2| = |J_1| = |J_2| = p \geq 2$.
\end{claim}
% \begin{proof}
%     Clearly, $I_1, I_2$ are disjoint and $J_1, J_2$ are also disjoint.
%     Next, note that the largest index is $I_2$ is $2\lceil n / 10 \rceil$ and the smallest index in $J_2$ is $m + n + 2c + 1 - 2\lceil n / 10 \rceil$.
%     Thus, to check disjointness, we just need to check $2 \lceil n / 10 \rceil < m + n + 2c + 1 - 2\lceil n / 10 \rceil$.
%     This is true since $4\lceil n / 10 \rceil \leq 4n / 10 + 4 \leq 6n / 10 \leq m + 2n + 2c + 1$.
%     For the last inequality, we used that since $n \geq 20$, we have $4 \leq 2n/10$.
%     This proves the first assertion.
%     The second assertion is trivial given $n \geq 20$.
% \end{proof}

% To construct both events, we divide the $M=m+n+2c$ quantiles into $K$ buckets of size $\frac{n}{10}$, $K=\frac{10(m+n+2c)}{n}$.  For $k \in [K]$, define $I_k = \{M\cdot \frac{k-1}{K} + 1, \ldots, \cdot \frac{k}{K}\}$. \mingfeinote{Need to round the bucket size, indexes etc.}

\paragraph{The good event $\cE_1$.}
Define event $\cE_1$ as the set of assignments $\pi$ such that all of the properties below are satisfied:
\begin{itemize}[itemsep=0pt, topsep=0pt]
    \item $|I_1 \cap \Bnew^{\pi}| \geq 2$, i.e.~at least $2$ new buyers are in $I_1$;
    \item $|I_2 \cap \Bold^{\pi}| \geq 1$, i.e.~at least $1$ old buyer is in $I_2$;
    \item $|J_1 \cap \Snew^{\pi}| \geq 2$, i.e.~at least $2$ new sellers are in $J_1$;
    \item $|J_2 \cap \Sold^{\pi}| \geq 1$, i.e.~at least $1$ old sellers is in $J_2$.   
\end{itemize}
\chrisnote{Let us first describe the intuition for this event. We show in Claim~\ref{claim:all_I2J2_trades} that every original buyer in $I_2$ and every original seller in $J_2$ participates in a trade in the original first-best matching. The requirement that $|I_2 \cap \Bold^{\pi}| \geq 1$ and $|J_2 \cap \Sold^{\pi}| \geq 1$ ensures that the original first-best matching has at least one buyer trading from $I_2$ and one seller trading from $J_2$. Conditioned on this, we can show that a \emph{sufficient} condition to augment the optimal trade size by is to have a new buyer and seller pair in $I_1$ and $J_1$, respectively. By ensuring that $|I_1 \cap \Bnew^{\pi}| \geq 2$ and $|J_1 \cap \Snew^{\pi}| \geq 2$, we can guarantee that the first-best matching increases by $2$ and thus, STR has at least one more trade than the original first-best matching. As an added bonus, defining the events as above allows us to prove a lower bound on the increase by GFT by using STR.}
Formally, we prove the following lemma.
\begin{lemma}
\label{lemma:E1}
Fix any $\Bq$.
We have that $\STR(\Bq, \pi)\geq\OPT(\Bq, \pi)$ for all $\pi\in \cE_1$. Moreover, $\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_1]\geq \expects{i, j}{b(q_i) - s(q_j)}$ where $i \sim I_1, j \sim J_1$ uniformly at random.
\end{lemma}
%\begin{proof}
%Let $\pi$ be any assignment in event $\cE_1$. Let $T$ be the number of trades in $\OPT$ in the original setting. 
%We condition on event $\cE_1$ and suppose that the original setting has $T$ trades. 

\begin{claim}
    \label{claim:all_I2J2_trades}
    In the original first-best matching, every original buyer in $I_1\cup I_2$ is matched and every original seller in $J_1\cup J_2$ is matched. Similarly, in the augmented first-best matching, every buyer in $I_1\cup I_2$ is matched and every seller in $J_1\cup J_2$ is matched.
\end{claim}
\begin{proof}
    For the first statement, we prove only that every original buyer in $I_1\cup I_2$ is matched. The proof for the sellers is analogous.
    
%    Let $\iold_{b, 1} < \ldots < \iold_{b, m}$ be the indices of the $m$ original buyers
%    and $\jold_{s, 1} > \ldots > \jold_{s, n}$ be the indices of the $m$ original sellers.
%    Similarly, let $\inew_{b, 1} < \ldots < \inew_{b, c}$ be the indices of the $c$ new buyers
%    and $\jnew_{s,1} > \ldots > \jnew_{s, c}$ be the indices of the $c$ new sellers.
%    We also let $i_{b, 1} < \ldots < i_{b, m+c}$ be the indices of all $m+c$ buyers
%    and $j_{s, 1} < \ldots < j_{s, n+c}$ be the indices of all $m+c$ sellers.
    
    Let $k = |(I_1 \cup I_2) \cap \Bold^{\pi}|$ be the number of original buyers in $I_1 \cup I_2$.
    Note that $k \leq 2\cdot \lceil n / 10 \rceil$.
    We prove that there are at least $k$ original sellers outside of $I_1 \cup I_2$, i.e.~$|\Sold^{\pi} \cap ([N] \setminus (I_1 \cup I_2))| \geq k$.
    Indeed, we have
    \begin{align*}
        |\Sold^{\pi} \cap ([N] \setminus (I_1 \cup I_2))|
        & =
        \underbrace{|\Sold^{\pi} \cap [N]|}_{=n} - |\Sold^{\pi} \cap (I_1 \cup I_2)|\\
        &\geq n - 2\left\lceil \frac{n}{10} \right\rceil
        \geq \frac{8n}{10} - 2
        \geq \frac{2n}{10} + 2 \\
        & \geq 2\left\lceil \frac{n}{10} \right\rceil \geq k,
    \end{align*}
    where in the third inequality we use $n \geq 20$.
    Recall that $\iold_k$ is the index of the $k$-th highest original buyer and $\jold_k$ is the index of the $k$-th lowest original seller. The above argument immediately implies that $q(\iold_k)\geq q(\jold_k)$ and thus $b(q(\iold_k))\geq s(q(\jold_k))$ since $F_B$ FSD $F_S$. Thus there are at least $k$ trades in the original first-best matching, which implies that every original buyer in $I_1\cup I_2$ is matched.
    
    The second statement follows from a similar argument. Let $k = |(I_1 \cup I_2) \cap (\Bold^{\pi} \cup \Bnew^{\pi})|$ be the number of buyers in $I_1 \cup I_2$. Note that $k \leq 2\cdot \lceil n / 10 \rceil$.
    We prove that there are at least $k$ sellers outside of $I_1 \cup I_2$, i.e.~$|(\Sold^{\pi}\cup \Snew^{\pi}) \cap ([N] \setminus (I_1 \cup I_2))| \geq k$.
    Indeed, we have
    \begin{align*}
        |(\Sold^{\pi}\cup \Snew^{\pi}) \cap ([N] \setminus (I_1 \cup I_2))|
        & =
        \underbrace{|(\Sold^{\pi}\cup \Snew^{\pi}) \cap [N]|}_{=n+c} - |(\Sold^{\pi}\cup \Snew^{\pi}) \cap (I_1 \cup I_2)|\\
        &\geq n + c - 2\left\lceil \frac{n}{10} \right\rceil
        \geq \frac{8n}{10} + c - 2
        \geq \frac{2n}{10} + 2 \\
        & \geq 2\left\lceil \frac{n}{10} \right\rceil \geq k,
    \end{align*}
    where in the third inequality we use $n \geq 20$.
    Since $F_B$ FSD $F_S$, every buyer in $I_1\cup I_2$ has value no less than the cost of every seller outside of $I_1\cup I_2$. Thus there are at least $k$ trades in the augment first-best matching, which implies that every buyer in $I_1\cup I_2$ is matched.
\end{proof}
% \chris{Currently, we use $i_b$, $j_s$ to denote buyer and seller indices. We can drop the $b$ and $s$. WDYT?}
% \mingfei{Sounds good.}

\begin{prevproof}{Lemma}{lemma:E1}
Let $\pi$ be any assignment in event $\cE_1$. Let $T$ be the number of trades in the original first-best matching. We prove in the following claim that there are at least $T+2$ trades in the augmented first-best matching. An immediate consequence of this is that STR must have at least $T + 1$ trades.

\begin{claim}\label{claim:two_more_trades}
    \label{claim:T_plus_2_trades_v2}
    Recall that $\inew_{2}$ is the index of the second-highest new buyer and $\jnew_{2}$ is the index of the second-lowest new seller. 
    Then 
    $b(q(\inew_{2}))\geq b(q(i_{T+2})) \geq s(q(j_{T+2}))\geq s(q(\jnew_{2}))$. Thus there are at least $T+2$ trades in the augmented first-best matching.
\end{claim}
\begin{proof}
    Let $i'\in I_2 \cap \Bold$ be the index of any original buyer in $I_2$ (by definition of $\cE_1$ there is at least one). By Claim~\ref{claim:all_I2J2_trades}, $i'$ is matched in the original first-best matching and thus $q(i') \geq q(\iold_{T})$. By the property of $\cE_1$ that $|I_1 \cap \Bnew| \geq 2$, we have $q(\inew_{2}) \geq q(i')\geq q(\iold_{T})$ since $\inew_2\in I_1$ while $i'\in I_2$.
    Therefore, $q(\inew_2)\geq q(i_{T+2}) \geq q(\iold_{T})$ as both the highest and second-highest new buyer have quantile no less than $q(\iold_{T})$. A similar argument shows that $q(\jnew_2)\leq q(j_{T+2}) \leq q(\jold_{T})$.
    We conclude that $b(q(\inew_{2}))\geq b(q(i_{T+2})) \geq b(q(\iold_{T})) \geq s(q(\jold_{T})) \geq s(q(j_{T+2}))\geq s(q(\jnew_{2}))$.
    Here the third inequality follows from the fact that there are $T$ trades in the original first-best matching.
\end{proof}

\Cref{claim:two_more_trades} shows that STR trades the $T+1$ highest buyers and the $T+1$ lowest sellers (it may trade more).
Therefore, $\STR(\Bq, \pi)\geq \sum_{t=1}^{T+1}[b(q(i_t))-s(q(j_t))]$. On the other hand, OPT trades the $T$ highest original buyers with the $T$ lowest original sellers and thus, $\OPT(\Bq, \pi)=\sum_{t=1}^{T}[b(q(\iold_t))-s(q(\jold_t))]$.

We claim that $\sum_{t=1}^{T+1}b(q(i_t))-\sum_{t=1}^{T}b(q(\iold_t))\geq b(q(\inew_1))$. This is because by \Cref{claim:two_more_trades}, buyers $\inew_1$ and $\inew_2$ are among the top $T+2$ highest-value buyers. So $\inew_1$ must be in the top $T+1$ highest-value buyers, which is contributed in the first term.
\chrisnote{Note that $\{i_1, \ldots, i_{T+1}\} \setminus \{\inew_1\}$ correspond to the $T$ highest value buyers excluding $\inew_1$ and $\{\iold_1 \ldots, \iold_T\}$ correspond to the top $T$ highest value \emph{original} buyers.
Thus, we conclude that $\sum_{t=1}^{T+1} b(q(i_t)) - b(q(\inew_1)) \geq \sum_{t=1}^T b(q(\iold_t))$.}
% $\sum_{t=1}^{T+1}b(q(i_t))-b(q(\inew_1))$ is the sum of values for the top $T$ buyers excluding $\inew_1$ (a new buyer), which is at least the sum of values for the top $T$ old buyers.
By a similar argument, we have $\sum_{t=1}^{T+1}s(q(j_t))-\sum_{t=1}^{T}s(q(\jold_t))\leq s(q(\jnew_1))$.
Thus
$$\STR(\Bq, \pi)-\OPT(\Bq, \pi)\geq b(q(\inew_1))-s(q(\jnew_1)) \geq 0$$

It remains to lower bound the expected difference between $\STR(\Bq, \pi)$ and $\OPT(\Bq, \pi)$ conditioned on the event $\cE_1$. 
%For any integer $k, \ell\in \{2, \ldots, p=\lceil n/10\rceil\}$, define event $\cF_{k, \ell}$ as the set of assignments such that there are $k$ (and $\ell$) new buyers (and sellers) in $I_1$. 
From the above inequality, $\STR(\Bq, \pi)-\OPT(\Bq, \pi)$ is lower bounded by the value of the highest new buyer subtracting the cost of the lowest new seller. We need the following definition.

\begin{definition}
For any event $\cE$ over an assignment $\pi$, $\cE$ is \emph{swappable} in a set $S$ if: For every $\pi\in \cE$, the assignment $\pi'$ obtained by swapping the label for any two indices in $S$ is also in $\cE$. %Similarly, an event $\cE$ is \emph{seller-swappable} in $J_1$ if for every $\pi\in \cE$, the assignment $\pi'$ obtained by swapping the label for any two sellers in $J_1$ is also in $\cE$.
\chrisnote{In other words, for every $\pi \in \cE$ and every $i', i'' \in S$, if $\pi'(i') = \pi(i'')$, $\pi'(i'') = \pi(i')$, and $\pi'(i) = \pi(i)$ for $i \notin \{i', i''\}$ then $\pi' \in \cE$.}
\end{definition}
\chris{Can you check the note above? Is that correct?}

\begin{lemma}\label{lem:E1_swappable}
$\cE_1$ is swappable in $I_1$ and it is swappable in $J_1$.
\end{lemma}

\begin{proof}
The lemma directly follows from the fact that swapping the label for any two indices in $I_1$ (or $J_1$) will not change the value of $|I_1 \cap \Bnew^{\pi}|$, $|I_2 \cap \Bold^{\pi}|$, $|J_1 \cap \Snew^{\pi}|$, $|J_2 \cap \Sold^{\pi}|$.
\end{proof}

Consider the following process that generates a random assignment $\pi$ from $\cE_1$: 
%that obtains a uniformly random assignment $\pi$ from $\cE_1$:
% \chris{I really like this. :)}
\begin{enumerate}
    \item Choose an index $i$ uniformly at random from $I_1$ and assign it to the ``New Buyer'' label. Choose an index $j$ uniformly at random from $J_1$ and assign it to the ``New Seller'' label.
    %\item Randomly choose an index from the rest indices in $I_1$ and assign it to the ``New Buyer'' label. Randomly choose an index from the rest indices in $J_1$ and assign it to the ``New Seller'' label.
    %\item Randomly choose an index from $I_2$ and assign it to the ``Old Buyer'' label. 
    %Randomly choose an index from $J_2$ and assign it to the ``Old Seller'' label.     
    %\item Randomly assign the remaining indices.
    \item Denote $\Pi_{i, j}$ the set of valid assignments
    in set $\cE_1$ such that $i$ is assigned to the ``New Buyer'' label and $j$ is assigned to the ``New Seller'' label. Draw an assignment $\pi$ uniformly at random from $\Pi_{i, j}$ and assign the indices accordingly.    
\end{enumerate}

By \Cref{lem:E1_swappable}, we have that $|\Pi_{i', j'}|=|\Pi_{i'', j''}|$ for any indices $i',i''\in I_1, j', j''\in J_1$: For any assignment in $\Pi_{i', j'}$, we can swap the label between indices $i', i''$ and swap between $j, j''$. This generates an assignment in $\Pi_{i'', j''}$ and vice versa. Moreover, for any valid assignment $\pi$, the number of ``New Buyer'' (or ``New Seller'') labels is $c$.
\chrisnote{Hence, for every valid assignment $\pi$, $|\{ i \in I_1, j \in J_1 \,:\, \pi \in \Pi_{i,j}\}| = c^2$.}
% So $\pi$ is in $c^2$ (a fixed number) different $\Pi_{i', j'}$s.
Thus the above random process chooses the assignment $\pi$ uniformly at random from $\cE_1$.

For any realization of the above process, the value of the highest new buyer is at least $b(q_{i})$ and the cost of the lowest new seller is at most $s(q_{j})$. Thus the difference is at least $b(q_{i})-s(q_{j})$.   
Taking expectation over the random process, we have
$$\bE_{\pi}[\STR(\Bq, \pi) - \OPT(\Bq, \pi)|\cE_1]\geq \expects{i, j}{b(q_{i}) - s(q_{j})}$$ where $i \sim I_1, j \sim J_1$ uniformly at random according to Step 1 of the process.
%\textcolor{red}{To be completed!}
\end{prevproof}

\paragraph{The bad event $\cE_2$.}
Next, we define the bad event $\cE_2$ as $\overline{\cE_1} \cap \{\pi\in \Pi_{n,m,c}\mid\Snew^{\pi} \subseteq [2n+2c]\}$.
In other words, event $\cE_2$ requires that (i) $\cE_1$ does not happen and (ii) all new sellers are in the top $2n+2c$ quantiles.
Lemma~\ref{lemma:notE2_STR_gt_OPT} shows that $\cE_2$ is a \emph{necessary} condition for $\OPT$ to obtain (strictly) more GFT than $\STR$.
Next, in Lemma~\ref{lemma: bound_loss_E2}, we bound the loss in GFT when $\cE_2$ does happen.
\begin{lemma}
    \label{lemma:notE2_STR_gt_OPT}
    Fix any $\Bq$, we have $\STR(\Bq, \pi) \geq \OPT(\Bq, \pi)$ for all $\pi\in \overline{\cE_2}$.
\end{lemma}
\begin{proof}
    We know from Lemma~\ref{lemma:E1} that on the event $\cE_1$, we have $\STR(\Bq, \pi) \geq \OPT(\Bq, \pi)$.
    Hence it suffices to show the inequality on the event $\cE'=\{\pi\in \Pi_{n,m,c}\mid\Snew^{\pi} \cap [2n+2c]\not=\Snew^{\pi}\}$. %Let $\OPT' = \OPT(m+c, n+c)$ be the optimal matching even with the augmented buyers and sellers.
    Let $\OPT'$ be the first-best matching in the augment market. For any $\pi\in \cE'$, we consider two cases based on the number of trades in $\OPT'$ compared with $\OPT$. Suppose $\OPT$ has $T$ trades. Note that the number of trades in $\OPT'$ is least $T$. 
    \paragraph{Case 1: $\OPT'$ has at least $T+1$ trades.}
    %Suppose $\OPT$ has $T$ trades. Then $\OPT'$ has at least $T+1$ trades.
    %In which case, 
    Now in $\STR$ at least the top $T$ (old and new) buyers and bottom $T$ (old and new) sellers trade.
    The GFT from this is larger than the GFT from $\OPT$ which trades the top $T$ old buyers and the bottom $T$ old sellers.

    \paragraph{Case 2: $\OPT'$ also has $T$ trades.}
    In this case, our goal is to show that $\STR$ has the exact same $T$ trades as $\OPT'$. Thus the GFT of $\STR$ is the same as the GFT of $\OPT'$, which is at least the GFT of $\OPT$.   
    %More precisely, suppose that $T \leq n$ is the number of trades in $\OPT'$ (and $\OPT$).
    By definition of STR, it suffices to show that $b(q(i_{T})) \geq s(q(j_{T+1}))$, i.e. the $T$-th highest buyer value is least the $(T+1)$-th lowest seller cost.
    %\begin{equation}
    %    \label{eqn:bT_gt_qT+1}
    %    b(q(i_{T})) \geq s(q(j_{T+1})) \geq s(q(j_{s,T})).
    %\end{equation}
    %The second inequality is true by definition so we only prove the first inequality.

    First, we claim that $i_{n+c} \leq 2n+2c$. Indeed, there are $n+c$ sellers in the augment market. Thus, the $(n+c)$-th highest-value buyer must have index at most $2n+2c$.

    Next, recall that $\jold_{T}$ is the index of the $T$-th lowest-value seller.
    We claim that $\jold_{T} \leq 2n+2c$.
    For the sake of contradiction, suppose $\jold_{T} > 2n+2c$. Recall that $\jnew_{1}$ is the index of the lowest-value new seller.
    Since $\pi\in \cE'$, i.e. not all new sellers are in the top $2n+2c$ quantiles, we have $\jnew_{1}>2n+2c$.
    Thus, $j_{T+1} \geq %\max
    \mingfeinote{\min}\{\jold_{T}, \jnew_{1}\} > 2n+2c \geq i_{n+c} \geq i_{T+1}$. Thus $q(i_{T+1})>q(j_{T+1})$ and $b(q(i_{T+1}))>s(q(j_{T+1}))$. This implies that $\OPT'$ has at least $T + 1$ trades, a contradiction.
    
    To finish the proof, we have
    \[
        b(q(i_{T}))
        \geq b(q(\iold_{T}))
        \geq s(q(\jold_{T}))
        \geq s(q(j_{T+1})).
    \]
    The first inequality uses $i_T\leq \iold_T$. The second inequality follows from the fact that $\OPT$ has $T$ trades. The last inequality holds because: $\jold_{T}\leq 2n+2c<\jnew_{1}$, we have $j_{T+1} \geq \min\{\jold_{T}, \jnew_{1}\} = \jold_{T}$.
    
    We conclude that $\STR$ has the exact same $T$ trades as $\OPT'$.
\end{proof}

\begin{lemma}\label{lemma: bound_loss_E2}
  %  $\expectg{\OPT - \STR}{\cE_2} \leq \expects{i, j}{b(q(i)) - s(q(j))}$ where $i \sim I_1, j \sim J_1$ uniformly at random.
For any $\Bq$, we have $\bE_{\pi}[\OPT(\Bq, \pi) - \STR(\Bq, \pi)|\cE_2]\leq \expects{i, j}{b(q_i) - s(q_j)}$ where $i \sim I_1, j \sim J_1$ uniformly at random.
\end{lemma}

\begin{proof}
For every $(\Bq, \pi)$ denote $\OPT'$ the GFT of the first-best matching in the augment market. We clearly have $\OPT(\Bq, \pi)\leq \OPT'(\Bq, \pi)$. For each $(\Bq, \pi)$, denote $b^*(\Bq,\pi)$ (and $s^*(\Bq, \pi)$) the lowest value among buyers (the largest cost among sellers) traded in the augment first-best matching. Let $b^*(\Bq,\pi)=s^*(\Bq, \pi)=0$ if there is no trade. Then by definition of the $\STR$ mechanism, $\OPT(\Bq, \pi) - \STR(\Bq, \pi)\leq \OPT'(\Bq, \pi)-\STR(\Bq, \pi)\leq b^*(\Bq, \pi)-s^*(\Bq,\pi)$. 

%To bound the expected difference $b^*(\Bq, \pi)-s^*(\Bq,\pi)$ conditioned on $\cE_2$, we need the following definition.

We consider $\bE[b^*(\Bq, \pi)|\cE_2]$, the expected lowest value among buyers traded in the augment first-best matching, conditioned on $\cE_2$. Let $\cE'$ be the event such that at least one new buyer is in $I_1$, i.e. $|I_1\cap \Bnew^{\pi}|\geq 1$. The following lemma is similar to \Cref{lem:E1_swappable}, which immediately follows from the definition of $\cE'$ and $\cE_2$.

\begin{lemma}\label{lem:swappable}
$\cE'\cap\cE_2$ is swappable in $I_1$. Moreover, it is swappable in $J_1$.
\end{lemma}

\begin{proof}
Let $\pi$ be any assignment in $\cE'\cap\cE_2=\cE'\cap\overline{\cE_1}\cap \{\hat{\pi}\in \Pi_{n,m,c}\mid\Snew^{\hat{\pi}} \subseteq [2n+2c]\}$ and $\pi'$ be the assignment obtained by swapping any two labels in $I_1$ (or $J_1$). We notice that swapping the label for any two indices in $I_1$ (or $J_1$) will not change the value of $|I_1 \cap \Bnew^{\pi}|$, $|I_2 \cap \Bold^{\pi}|$, $|J_1 \cap \Snew^{\pi}|$, $|J_2 \cap \Sold^{\pi}|$. Thus the new assignment $\pi'$ is also in $\cE'\cap\overline{\cE_1}$. Moreover, since $I_1\subseteq [2n+2c]$, $\Snew^{\pi} \subseteq [2n+2c]$ implies that $\Snew^{\pi'} \subseteq [2n+2c]$. Thus $\pi\in \{\hat{\pi}\in \Pi_{n,m,c}\mid\Snew^{\hat{\pi}} \subseteq [2n+2c]\}$.
\end{proof}

Back to the proof of \Cref{lemma: bound_loss_E2}. Consider the following random process of choosing an assignment $\pi$:

\begin{enumerate}
    \item Choose an index $i$ uniformly at random from $I_1$ and assign it to the ``New Buyer'' label.
    \item Denote $\Pi_{i}$ the set of valid assignments %$\pi_{-i} \colon [N]\backslash \{i\} \to \{\BO, \BN, \SO, \SN\}$ 
    in set $\cE'\cap \cE_2$ such that $i$ is assigned to the ``New Buyer'' label. Draw an assignment $\pi$ uniformly at random from $\Pi_{i}$ and assign the indices accordingly.
\end{enumerate}

By \Cref{lem:swappable}, we have that $|\Pi_{i'}|=|\Pi_{i''}|$ for any indices $i',i''\in I_1$: For any assignment in $\Pi_{i'}$, we can swap the label for index $i'$ and index $i''$ and generate an assignment in $\Pi_{i''}$ and vice versa. Moreover, for any valid assignment $\pi$, the number of ``New Buyer'' labels is $c$. So $\pi$ is in $c$ (a fixed number) different $\Pi_{i'}$s. Thus the above random process chooses the assignment $\pi$ uniformly random from $\cE'\cap \cE_2$.

For any realization of the above process, we notice that by \Cref{claim:all_I2J2_trades}, the new buyer with index $i$ trades in the augmented first-best matching. Thus $b^*(\Bq, \pi)$, the lowest value among buyers traded in the augmented first-best matching, is upper bounded by $b(q(i))$. Thus $\bE_{\pi}[b^*(\Bq, \pi)|\cE'\cap\cE_2]\leq \bE_i[b(q(i))]$, where $i$ draws from $I_1$ uniformly at random.

Let $\cE''$ be the event such that no new buyer is in $I_1$ and at least one old buyer is in $I_1$, i.e. $|I_1\cap \Bold^{\pi}|\geq 1$ and $|I_1\cap \Bnew^{\pi}|=0$. One can easily verify that $\cE''\cap \cE_2$ is also swappable in $I_1$. And using a similar argument (by assigning index $i$ to the ``Old Buyer'' label in the random process), we have $\bE_{\pi}[b^*(\Bq, \pi)|\cE''\cap\cE_2]\leq \bE_i[b(q(i))]$, where $i$ draws from $I_1$ uniformly at random.

Let $\cE'''=\overline{\cE'\cup \cE''}$ be the event such that no buyer is in $I_1$. Then for any $\pi\in \cE'''$, $b^*(\Bq, \pi)\leq b(q(\lceil n/10\rceil))$, the buyer value from the lowest quantile in $I_1$. Thus $\bE_{\pi}[b^*(\Bq, \pi)|\cE'''\cap\cE_2]\leq b(q(\lceil n/10\rceil))\leq \bE_i[b(q(i))]$, where $i$ draws from $I_1$ uniformly at random.

Summarizing the three inequalities above, we have that $\bE_{\pi}[b^*(\Bq, \pi)|\cE_2]\leq \bE_i[b(q(i))]$, where $i$ draws from $I_1$ uniformly at random. Without an analogous argument, we have that $\bE_{\pi}[s^*(\Bq, \pi)|\cE_2]\geq \bE_j[s(q(j))]$, where $j$ draws from $J_1$ uniformly at random. Therefore,
$$\bE_{\pi}[\OPT(\Bq, \pi) - \STR(\Bq, \pi)|\cE_2]\leq \bE_{\pi}[b^*(\Bq, \pi) - s^*(\Bq, \pi)|\cE_2]\leq  \expects{i, j}{b(q_i) - s(q_j)},$$
where $i \sim I_1, j \sim J_1$ uniformly at random.
\end{proof}


To complete the proof, it remains to prove that $\prob{\cE_1} \geq \prob{\cE_2}$.
\begin{lemma}
    \label{lemma:probE1_gt_probE2}
    Fix $c \geq 20000$ and suppose that $m \geq n + 2c$ and $n \geq c$.
    Then $\prob{\cE_1} \geq \prob{\cE_2}$.
\end{lemma}
We devote Subsection~\ref{subsec:proof_probE1_gt_probE2} to the proof of Lemma~\ref{lemma:probE1_gt_probE2}.

\subsection{Proof of Lemma~\ref{lemma:probE1_gt_probE2}}
\label{subsec:proof_probE1_gt_probE2}
Before we prove Lemma~\ref{lemma:probE1_gt_probE2}, we give some high-level intuition.
Recall that the ``good event'' $\cE_1$ is that the following four statements hold:
\begin{itemize}
    \item $|I_1 \cap \Bnew^{\pi}| \geq 2$;
    \item $|I_2 \cap \Bold^{\pi}| \geq 1$;
    \item $|J_2 \cap \Sold^{\pi}| \geq 1$; and
    \item $|J_1 \cap \Snew^{\pi}| \geq 2$.
\end{itemize}
Recall that $|I_1| = |I_2| = |J_1| = |J_2| = p = \left\lceil \frac{n}{10} \right\rceil$.
For intuition, we consider two extremes.
First, suppose that $n = m$, i.e.~there are an equal number of buyers and sellers.
Assuming that $m \gg c$, we would have $|I_1| / (2m + 2c) \approx 1/20$.
In other words, if we took a random new buyer and assigned it a uniformly random index from $[N]$
then with probability about $1/20$, it would land in $I_1$.
Since there are $c$ new buyers, we would expect that $\expect{|I_1 \cap \Bnew^{\pi}|} \sim c / 20 \geq 2$ provided that $c \geq 40$.
Moreover, if $c$ is a sufficiently large constant then Hoeffding's Inequality suggests that we should have $|I_1 \cap \Bnew^{\pi}| \geq 2$ %with very high probability.
\mingfeinote{with probability at least $1-\eps$ for some sufficiently small constant $\eps>0$.}
Similarly, we would have $|I_2 \cap \Bold^{\pi}| \geq 1$, $|J_2 \cap \Sold^{\pi}| \geq 1$, and $|J_1 \cap \Snew^{\pi}| \geq 2$ %with high probability.
\mingfeinote{with probability at least $1-\eps$}. By union bound the good event $\cE_1$ happens %with high probability, it must be that 
with probability at least $1-4\eps$ while the bad event $\cE_2 \subseteq \overline{\cE_1}$ happens with probability \mingfeinote{at most $4\eps$}.
This proves Lemma~\ref{lemma:probE1_gt_probE2} when $m \approx n$.

Now, let us consider the other extreme where $n \ll m$.
In this case $|I_1| / N \sim n / m$.
%A very rough lower bound for 
The probability of event $\cE_1$ is roughly $(n/m)^6$
(the first and last requirement hold with probability $(n/m)^2$ each and the second and third requirement hold with probability $(n/m)$ each). A formal statement can be found in (ADD LEMMA). On the other hand, the bad event $\cE_2$ is contained in the event that all the new sellers are in the top $2n+2c$ quantiles.
The probability that a new seller receives a uniform index and lands in $[2n+2c]$ is $\frac{2n+2c}{m+n+2c} = O(\frac{n}{m})$. Thus, the probability that all the new sellers land in $[2n+2c]$ is $O((n / m)^c)$. Thus, for sufficiently large constant $c$, we would expect $\prob{\cE_2} \leq \prob{\cE_1}$.

More formally, we have the following two lemmas which together prove %that when %$m, n, c$ are sufficiently large,
%we always have $\prob{\cE_1} \geq \prob{\cE_2}$ and completes the proof of Theorem~\ref{thm:str_main}.
\Cref{lemma:probE1_gt_probE2}.

\begin{lemma}
    \label{lemma:large_n_case}
    If $c \geq 150$, $m \geq 2c$, $n \geq c$, and $n \geq \frac{40}{c} \log(12 c) \cdot m$ then $\prob{\cE_1} \geq 1/2 \geq \prob{\cE_2}$.
\end{lemma}
\begin{lemma}
    \label{lemma:small_n_case}
    If $c \geq 20000$, $m \geq c$,
    and $n \leq \frac{40}{c} \log(12c) \cdot m$.
    Then $\prob{\cE_1} \geq \prob{\cE_2}$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:probE1_gt_probE2}]
    Immediate from Lemma~\ref{lemma:large_n_case} and Lemma~\ref{lemma:small_n_case}.
\end{proof}

\subsubsection{Proof of Lemma~\ref{lemma:large_n_case}}
The main ingredient to prove Lemma~\ref{lemma:large_n_case} is the following lemma which shows that if $n = \Theta(m)$ then the probability that event $\cE_1$ does \emph{not} happen decays exponentially quickly in $c$.
\begin{lemma}
    \label{lemma:E1_prob_lb}
    If $m \geq n \geq c$ then
    $\prob{\cE_1} \geq 1 - 6c \cdot \exp\left( -\frac{cn}{10(m+n+2c)} \right)$.
\end{lemma}

Given this lemma, the proof of Lemma~\ref{lemma:large_n_case} is straightforward.
\begin{proof}[Proof of Lemma~\ref{lemma:large_n_case}]
    Since $\prob{\cE_2} \leq \prob{\overline{\cE_1}} = 1 - \prob{\cE_1}$, we only need to to prove that $\prob{\overline{\cE_1}} \leq 1/2$.
    By Lemma~\ref{lemma:E1_prob_lb}, we need to check that
    \begin{equation}
        \label{eqn:big_n_sufficient}
        6c \cdot \exp\left( - \frac{cn}{10(m+n+2c)} \right) \leq \frac{1}{2}. 
    \end{equation}
    Rearranging, this is equivalent to $n\left(1 - \frac{10}{c} \log(12c)\right) \geq \frac{10}{c} \log(12c)(m+2c)$.
    Indeed,
    \[
        n\left(1 - \frac{10}{c} \log(12c)\right) \geq \frac{n}{2} \geq \frac{20}{c} \log(12c) m \geq \frac{10}{c} \log(12c)(m+2c)
    \]
    where the first inequality uses Claim~\ref{claim:c_ineq}, the second inequality uses the assumption on $n$, and the last inequality uses that $2m = m + m \geq m + 2c$.
\end{proof}

We now prove Lemma~\ref{lemma:E1_prob_lb}.
\begin{proof}[Proof of Lemma~\ref{lemma:E1_prob_lb}]
Recall that $p=\lceil n/10\rceil$. First, we have
\[
    \Pr_{\pi}[|I_1 \cap \Bnew^{\pi}| = 0]
    = \frac{\binom{m+n+c}{p}}{\binom{m+n+2c}{p}}.
\]
To see this, one can think of the following alternative way of choosing the assignment: The agents (including buyers and sellers) are named as $1,2,\ldots, m+n+2c$. Agents $1,2,\ldots, m$ are old buyers; Agents $m+1,m+2,\ldots, m+n$ are old sellers; Agents $m+n+1,\ldots m+n+c$ are new buyers; Agents $m+n+c+1,\ldots m+n+2c$ are new sellers. We choose $p$ agents and assign them the ``In $I_1$'' label. 
%The numerator is the number of ways to assign $p$ indices to the $m+n+c$ quantiles which are \emph{not} a new buyer.
The numerator is the number of ways to choose $p$ agents from the set of ``not new buyers'' (and assign them the label). The denominator is the number of ways to choose $p$ agents from all $m+n+2c$ agents (and assign them the label).
%to any of the $m+n+2c$ buyers and sellers.
Similarly, we have
\[
    \Pr_{\pi}[|I_1 \cap \Bnew^{\pi}| = 1]
    = \frac{\binom{c}{1}\cdot \binom{m+n+c}{p - 1}}{\binom{m+n+2c}{p}}.
\]
The same argument can be applied for $|J_1 \cap \Snew^{\pi}|$.
In other words,
\[
    \Pr_{\pi}[|I_1 \cap \Bnew^{\pi}| \leq 1] = \Pr_{\pi}[|J_1 \cap \Snew^{\pi}| \leq 1]
    = \frac{\binom{m+n+c}{p} + c \cdot \binom{m+n+c}{p - 1}}{\binom{m+n+2c}{p}}.
\]
Next, we have
\[
    \Pr_{\pi}[|I_2 \cap \Bold^{\pi}| = 0]
    = \frac{\binom{n+2c}{p}}{\binom{m+n+2c}{p}}
\]
and
\[
    \Pr_{\pi}[|J_2 \cap \Sold^{\pi}| = 0]
    = \frac{\binom{m+2c}{p}}{\binom{m+n+2c}{p}}.
\]
Here we notice that the numerators in the two equations above are the number of ways to choose $p$ agents from the set excluding the $m$ old buyers (or $n$ old sellers), and assign them the ``In $I_2$ (or $J_2$)'' label. By union bound, we have
\begin{align*}
    \prob{\overline{\cE_1}}
    & \leq \frac{2\binom{m+n+c}{p} + 2c\cdot\binom{m+n+c}{p - 1} + \binom{n+2c}{p} + \binom{m+2c}{p} }{\binom{m+n+2c}{p}} \\
    & \leq \frac{6c \binom{m+n+c}{\lceil n / 10 \rceil}}{\binom{m+n+2c}{\lceil n / 10 \rceil}} \\
    & = 6c
        \cdot \frac{(m+n+c)!}{\lceil n / 10 \rceil! \cdot (m + n + c - \lceil n /10 \rceil)!}
        \cdot \frac{\lceil n / 10 \rceil! \cdot (m+n+2c - \lceil n / 10 \rceil)!}{(m+n+2c)!} \\
    & = 6c \prod_{i=1}^c \frac{m+n+c-\lceil n / 10 \rceil + i}{m+n+c+i} \\
    & = 6c \prod_{i=1}^c \left(1 - \frac{\lceil n / 10 \rceil}{m+n+c+i} \right) \\
    & \leq 6c\cdot \exp\left(-\sum_{i=1}^c \frac{n/10}{m+n+c+i}\right)
    \leq 6c \cdot \exp\left( - \frac{cn}{10(m+n+2c)} \right)
\end{align*}
In the second inequality, we used that (i) $p=\lceil n / 10 \rceil$, (ii) $\binom{m+n+c}{\lceil n / 10 \rceil - 1} \leq \binom{m+n+c}{\lceil n / 10 \rceil}$ since $\lceil n / 10 \rceil<\frac{1}{2}(m+n+c)$, (iii) $n + 2c\leq m+2c \leq m+n+c$ since $m \geq n \geq c$. The second-last inequality follows from $1-x\leq \exp(-x)$ for all $x>0$.
\end{proof}

%\begin{claim}
%    \label{claim:c_ineq}
%    If $c \geq 150$ then $\frac{10}{c} \log(12c) \leq 1/2$.
%\end{claim}
%\begin{proof}
%    Let $f(c) = \frac{10}{c} \log(12c)$.
%    One can check that $f(150) < 1/2$.
%    Moreover, $f'(c) = -\frac{10}{c^2} (\log(12c) - 1) > 0$ since $\log(12c) < \log(e) = 1$.
%\end{proof}

\subsubsection{Proof of Lemma~\ref{lemma:small_n_case}}
To prove Lemma~\ref{lemma:small_n_case}, we require two lemmas.
The first lemma is another lower bound on $\prob{\cE_1}$ which is tighter than Lemma~\ref{lemma:E1_prob_lb} when $n \ll m$ (the latter uses a union bound which becomes too loose in this setting).
The second lemma upper bounds $\prob{\cE_2}$ by upper bounding the probability that all new sellers are in the top $2n+2c$ quantiles.
In contrast, the previous subsection upper bounded $\prob{\cE_2}$ by simply saying that $\prob{\cE_2} \leq 1 - \prob{\cE_1}$.
However, since $\prob{\cE_1}$ is also small for small $n$. This latter upper bound is far too weak.

\begin{lemma}
    \label{lemma:small_n_E1}
    Let $\alpha > 0$ (possibly depending on $c$). Suppose that (i) $c \geq 2$, (ii) $m \geq n + 2c \geq n + c + 2$ and (iii) $n \leq \frac{10 \alpha m}{c} - 1$.
    Then
    \[
        \prob{\cE_1} \geq
        \frac{1}{40} \left( \frac{c}{120} \right)^4 \cdot \left(1 - \frac{10\alpha}{c} \right)^{2c} \cdot \frac{n^6}{m^6}.
    \]
\end{lemma}
The proof of Lemma~\ref{lemma:small_n_E1} is somewhat lengthy so we relegate it to Subsection~\ref{subsubsec:small_n_E1}.

\begin{lemma}
    \label{lemma:small_n_E2}
    %Suppose that $n \leq m / 6$.
    %Then $\prob{\cE_2} \leq (8n / m)^c$.
    {Suppose that $n \leq m / 4$.
    Then $\prob{\cE_2} \leq (4n / m)^c$.}
\end{lemma}
\begin{proof}
We have
\begin{align*}
    \Pr_{\pi}[\Snew^{\pi} \subseteq [2n + 2c]]
    & =
    \frac{\binom{m+n+c}{2n+c}}{\binom{m+n+2c}{2n+2c}} \\
    & = \frac{(m+n+c)!}{(2n+c)!(m-n)!} \cdot \frac{(2n+2c)!(m-n)!}{(m+n+2c)!} \\
    & = \prod_{i=1}^c \frac{2n+c+i}%{m-n-c+i} \\
    {m+n+c+i}
    %& \leq \frac{(4n)^c}{(m/2)^c} \\
    \leq \left( \frac{4n}{m} \right)^c
\end{align*}
In the first equality, the denominator is the number of ways to choose $2n+2c$ agents from all $m+n+2c$ agents (and assign them the ``In $[2n+2c]$'' label). When all $c$ new sellers are assigned the ``In $[2n+2c]$'' label, the numerator is the number of ways to choose another $2n+c$ agents from the rest $m+n+c$ agents (and assign them the label).
The inequality follows from $2n+c+i \leq 2n + 2c \leq 4n$ %and $m-n-c+i \geq m-n-2c \geq m-3n \geq m/2$ provided $n \leq m / 6$.
and $m+n+c+i\geq m$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:small_n_case}]
    Since $m \geq c \geq \frac{c}{40 \log(12c)}$ and $n \leq \frac{40}{c} \log(12c) \cdot m \leq m / 4$,
    it is straightforward to verify that $n \leq \frac{10 \alpha m}{c} - 1$ with $\alpha = 8 \log(12c)$.
    Thus, we have
    \begin{align*}
        \frac{\prob{\cE_2}}{\prob{\cE_1}}
        & \leq \frac{40 \left( \frac{120}{c} \right)^4}{\left( 1 - 10\alpha / c\right)^{2c}} \cdot 4^c \cdot \left( \frac{n}{m} \right)^{c-6} \\
        & \leq \frac{40 \left( \frac{120}{c} \right)^4}{\left( 1 - 10\alpha / c\right)^{2c}} \cdot 4^c \cdot \left( \frac{10\alpha}{c} \right)^{c-6} \\
        & \leq \frac{40 \left( \frac{120}{c} \right)^4}{\left( 1 - 10\alpha / c\right)^{2c}} \cdot 4^6 \cdot \left( \frac{40\alpha}{c} \right)^{c-6} \\
        & \leq 40 \left( \frac{120}{c} \right)^4 \cdot 16^6 \cdot \left( \frac{160\alpha}{c} \right)^{c-6} \\
        & \leq 9000 \cdot \left( \frac{160 \alpha}{c} \right)^{c-6} \\
        & \leq 9000 \cdot 0.8^{c-6} \\
        & < 1.
    \end{align*}
    In the fourth inequality, we used that $1 - 10\alpha / c = 1 - 80 \log(12c) / c \geq 1/2$ for $c \geq 2000$.
    In the sixth inequality, we used that $1280 \log(12c) / c \leq 0.8$ for $c \geq 20000$.
\end{proof}


\subsubsection{Proof of Lemma~\ref{lemma:small_n_E1}}
\label{subsubsec:small_n_E1}
\begin{claim}
    \label{claim:independence_lb}
    $\prob{\cE_1} \geq \prob{|I_1 \cap \Bnew \geq 2} \cdot \prob{|I_2 \cap \Bold| \geq 1} \cdot \prob{|J_2 \cap \Sold| \geq 1} \cdot \prob{|J_1 \cap \Snew| \geq 2}$.
\end{claim}
\begin{proof}
    Recall that
    \[
        \cE_1 = \{ |I_1 \cap \Bnew| \geq 2, |I_2 \cap \Bold| \geq 1, |J_2 \cap \Sold| \geq 1, |J_1 \cap \Snew| \geq 2 \}.
    \]
    We first check that
    \[
        \prob{|I_1 \cap \Bnew| \geq 2 \mid |I_2 \cap \Bold| \geq 1, |J_2 \cap \Sold| \geq 1, |J_1 \cap \Snew| \geq 2}
        \geq \prob{|I_1 \cap \Bnew| \geq 2}.
    \]
    Let $\cE_{1,1} = \{ |I_2 \cap \Bold| \geq 1, |J_2 \cap \Sold| \geq 1, |J_1 \cap \Snew \geq 2 \}$
    and $\cF = \{ \exists X \subseteq [N] \setminus I_1, |X| = 4, X \cap \Bnew = \emptyset \}$.
    Note that $\cE_{1,1} \subseteq \cF$ and that the random variable $|I_1 \cap \Bnew|$ is independent of $\cE_{1,1}$ given $\cF$.
    Thus,
    \[
        \probg{|I_1 \cap \Bnew| \geq 2}{\cE_{1,1}} 
        = \probg{|I_1 \cap \Bnew| \geq 2}{\cE_{1,1} \wedge \cF}
        = \probg{|I_1 \cap \Bnew| \geq 2}{\cF}
        \geq \prob{|I_1 \cap \Bnew| \geq 2},
    \]
    where the last inequality is by Claim~\ref{claim:prob_condition_lb}.
    % Note that the LHS is a conditional probability of $|I_1 \cap \Bnew| \geq 2$ conditioned on $|I_2 \cap \Bold| \geq 1, |J_2 \cap \Sold| \geq 1, |J_1 \cap \Snew| \geq 2$. To compute the probability on the left, we can first remove $4$ quantiles from $I_2 \cup J_2 \cup J_1$.
    % Then the LHS is the probability that at least $2$ out of $c$ quantiles chosen uniformly at random from the remaining $m+n+2c-4$ quantiles are in $I_1$.
    % On the other hand, the RHS probability is the probability that at least $2$ out of $c$ quantiles chosen uniformly at random from all $m+n+2c$ quantiles are in $I_1$.
    % In particular, the former probability is larger than the latter probability.
    % Thus, we conclude that
    % \[
    %     \prob{\cE_1} \geq \prob{|I_1 \cap \Bnew| \geq 2} \cdot \prob{|I_2 \cap \Bold| \geq 1, |J_2 \cap \Sold| \geq 1, |J_1 \cap \Bold| \geq 2}.
    % \]
    Continuing this argument gives the claim.
\end{proof}



\begin{claim}
    \label{claim:small_n_I1_J1_lb}
    Let $\alpha > 0$. Suppose that (i) $c \geq 2$, (ii) $m \geq n + c + 2$ and (iii) $n \leq \frac{10 \alpha m}{c} - 1$.
    Then
    \[
        \prob{|I_1 \cap \Bnew| \geq 2} = \prob{|J_1 \cap \Snew| \geq 2} \geq \frac{c^2}{12800} \cdot \frac{n^2}{m^2} \cdot \left( 1 - \frac{10\alpha}{c} \right)^c.
    \]
\end{claim}
\begin{proof}
    We compute a lower bound on $\prob{|I_1 \cap \Bnew| = 2}$.
    We have that
    \begin{align*}
        \prob{|I_1 \cap \Bnew| = 2}
        & = \frac{\binom{c}{2} \cdot \binom{m+n+c}{\lceil n / 10 \rceil - 2}}{\binom{m+n+2c}{\lceil n / 10 \rceil}} \\
        & = \binom{c}{2} \cdot \frac{(m+n+c)!}{(m+n+2c)!} \cdot \frac{\lceil n / 10 \rceil! (m+n+2c - \lceil n / 10 \rceil)!}{(\lceil n / 10 \rceil - 2)!(m+n+c - \lceil n / 10 \rceil + 2)!} \\
        & \geq \frac{(c-1)^2}{2} \cdot \frac{\left( \frac{n}{10} - 1 \right)^2}{(m+n+c+2)^2} \cdot \prod_{i=3}^c \frac{m+n+c-\lceil n / 10 \rceil + i}{m+n+c+i} \\
        & \geq \frac{(c-1)^2}{2} \cdot \frac{\left( \frac{n}{10} - 1 \right)^2}{(m+n+c+2)^2} \cdot \left( 1 - \frac{\lceil n / 10 \rceil}{m+n+c} \right)^{c-2} \\
        & \geq \frac{(c-1)^2}{2} \cdot \frac{\left( \frac{n}{10} - 1 \right)^2}{(m+n+c+2)^2} \cdot \left( 1 - \frac{10\alpha m / c}{m+n+c} \right)^{c-2} \\
        & \geq \frac{(c-1)^2}{2} \cdot \frac{\left( \frac{n}{10} - 1 \right)^2}{(m+n+c+2)^2} \cdot \left( 1 - \frac{10\alpha}{c} \right)^c \\
        & \geq \frac{c^2}{8} \cdot \frac{(n/20)^2}{(2m)^2} \cdot \left( 1 - \frac{10\alpha}{c} \right)^c \\
        & = \frac{c^2}{12800} \cdot \frac{n^2}{m^2} \cdot \left( 1 - \frac{10\alpha}{c} \right)^c.
    \end{align*}
    In the third inequality, we used that $\lceil n / 10 \rceil < n/10 + 1 \leq 10\alpha m / c$ since $n \leq 10\alpha m / c - 1$.
    In the fourth inequality, we used the trivial inequality $m + n + c \geq m$.
    Finally, in the fifth inequality, we used that $c-1 \geq c/2$, $n/10 - 1 \geq n / 20$ and $m+n+c+2 \leq 2m$.
\end{proof}

\begin{claim}
    \label{claim:small_n_I2_J2_lb}
    If $m \geq n + 2c$ then $\prob{|I_2 \cap \Bold| \geq 1} \geq \prob{|J_2 \cap \Sold| \geq 1} \geq \frac{n}{20m}$.
\end{claim}
\begin{proof}
    The first inequality is because $m \geq n$ so we prove only the second inequality.
    We have that
    \begin{align*}
        \prob{|J_2 \cap \Sold| = 0}
        & = \frac{\binom{m+2c}{\lceil n / 10 \rceil}}{\binom{m+n+2c}{\lceil n / 10 \rceil}} \\
        & = \frac{(m+2c)!}{(m+n+2c)!} \cdot \frac{(m+n+2c-\lceil n / 10 \rceil)!}{m+2c-\lceil n / 10 \rceil)!} \\
        & = \prod_{i=1}^n \frac{m+2c+i-\lceil n / 10 \rceil}{m+2c+i} \\
        & = \prod_{i=1}^n \left( 1 - \frac{\lceil n / 10 \rceil}{m+2c+i} \right) \\
        & \leq \prod_{i=1}^n \left( 1 - \frac{n}{10(m+n+2c)} \right) \\
        & \leq 1 - \frac{n}{10(m+n+2c)}
    \end{align*}
    In the first inequality, we used that $\lceil n / 10 \rceil \geq n / 10$ and $m=2c+i \leq m+n+2c$ for all $i \in [n]$.
    Thus, $\prob{|I_2 \cap \Bold| \geq 1} \geq \frac{n}{10(m+n+2c)} \geq \frac{n}{20m}$, where the final inequality is because $n+2c \leq m$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:small_n_E1}]
    Follows directly by combining Claim~\ref{claim:independence_lb}, Claim~\ref{claim:small_n_I1_J1_lb}, and Claim~\ref{claim:small_n_I2_J2_lb}.
\end{proof}

%\chris{Following claim appears a few times albeit with different constants.}
\begin{claim}\label{claim:c_ineq}
    If $c \geq 2000$ then $\frac{80 \log(12c)}{c} \leq 1/2$. If $c \geq 150$ then $\frac{10}{c} \log(12c) \leq 1/2$.
    If $c \geq 20000$ then $\frac{1280\log(12c)}{c} \leq 0.8$.
\end{claim}
\begin{proof}
    Let $f(c) = \frac{80}{c} \log(12c)$.
    One can check that $f(2000) < 1/2$.
    Moreover, $f'(c) = -\frac{80}{c^2} (\log(12c) - 1) < 0$ since $\log(12c) > \log(e) = 1$. Other statements are similar.
\end{proof}

The proof of the following claim can be found in Appendix~\ref{app:prob_condition_lb}.
\begin{claim}
    \label{claim:prob_condition_lb}
    Let $N \geq 1, c \geq 1$ be integers.
    Fix sets $I \subseteq [N]$ and $K \subseteq [N] \setminus I$.
    Let $X$ be a uniformly random subset of $[N]$ such that $|X| = c$.
    Then for every $r \geq 0$,
    \[
        \probg{|X \cap I| \geq r}{X \cap K = \emptyset} \geq \prob{|X \cap I| \geq r}.
    \]
\end{claim}

